Factorization and Normalization, Essentially

Lambda-calculi come with no fixed evaluation strategy. Different strategies may then be considered, and it is important that they satisfy some abstract rewriting property, such as factorization or normalization theorems. In this paper we provide simple proof techniques for these theorems. Our starting point is a revisitation of Takahashi's technique to prove factorization for head reduction. Our technique is both simpler and more powerful, as it works in cases where Takahishi's does not. We then pair factorization with two other abstract properties, defining \emph{essential systems}, and show that normalization follows. Concretely, we apply the technique to four case studies, two classic ones, head and the leftmost-outermost reductions, and two less classic ones, non-deterministic weak call-by-value and least-level reductions.

==> 05_-_Abstract_Normalisation.tex <==
% !TEX root = main.tex
\section{Abstract Normalisation}
\label{sect:abstract-rewriting}


==> 07_-_Stratified_CbV.tex <==
% !TEX root = mainCbV.tex
\renewcommand{\toat}[1]{\xrightarrow[\betav:#1]{}}
\newcommand{\tobat}[1]{\xrightarrow[\beta:#1]{}}

\renewcommand{\tmp}{ p}

\label{sect:stratified-cbn}
\newcommand{\sth}{\text{ s.t. }}

\section{Preliminary Lemmas}
Notation: $p\to^*q$ indicates a finite sequence from $p$ to $q$.

The lemmas below are elementary properties of $\tob$ (resp. $\tobv$) 

\begin{lemma}\label{l:basicCbN} If $\tm\tob\tms$ by a step which is \emph{not} a $\beta$-redex then  $s$ is an abstraction (resp. an application) \emph{if and only if so} is $\tm$:
	\begin{enumerate}
	%	\item $\tms$ is not a variable
		\item  $\tms=\la x s'$ iff $\tm=\la x t'$ with  $t'\tob s'$
		\item $\tms=pq$ iff $\tm = rs$ with  ($\tmr\tob p$ and $\tms= q$) or ($\tmr= p$ and $\tms\tob q$). 
	\end{enumerate}
	So if  $\tms=pq$ and $\tm = rs$, then    $p$ is an abstraction iff $r$ is.
\end{lemma}


\begin{lemma}\label{l:basicCbV} If $\tm\tobv\tms$ by a step which is \emph{not} a $\betav$-redex  
	 then  $s$ is an abstraction (resp. an application) \emph{if and only if so} is $\tm$:
	\begin{enumerate}
	%	\item $\tms$ is not a variable
		\item $\tms=\la x s'$ iff $\tm=\la x t'$, with  $t'\tobv s'$
		\item $\tms=pq$ iff $\tm = rs$, with  ($\tmr\tobv p$ and $\tms= q$) or ($\tmr= p$ and $\tms\tobv q$). 
	\end{enumerate}
	So  if  $\tms=pq$ and $\tm = rs$, then $p$ is an abstraction iff $r$ is; $q$ is a value iff $s$ is.
\end{lemma}

\section{Least-Level Normalization  in CbV}
With the obvious CbV definitions of depth of the $\betav$ step $\toat{k}$ and of least-level of a term $\deg t$,
given surface factorization, we obtain normalization. 

 \CF{Per fare \textbf{induzione sulle forme normali}, non c'e' bisogno di avere una  speciale grammatica delle forme normali. }\\

We have proved \emph{surface factorization} :
\begin{theorem}[Weak \cbv factorization]
	\label{thm:weak-fact0}
	If $\tm \tobv^* \tmtwo$ then $\tm\toat{0}^* \tms \toat{>0}^* \tmu$.
\end{theorem}

\emph{Least-Level Normalization}  follows:
\begin{theorem}[CBV Normalization]
	if $\tm \tobv^* r$ with $r$  $\tobv$-normal, then $\tm\toll^*  \tmr$.
	
\end{theorem}

\begin{proof}	By induction on the term $r$.
	From $\tm \tobv^* r$, 
	by  \refthm{weak-fact0}, we have that \begin{center}
		$\tm\toat{0}^* u  \toat{>0}^* r$.
	\end{center}

	Cases:


\begin{enumerate}
	\item $r=x$. Then  $u=x$, and trivially  $\tm\toat{0}^* r$.
	\item $r=\l x.r'$. Then $u=\l x. u'$, hence  $u' \tobv^*  r'$, where  $ r' $ is $\tobv$-normal, and we use the \ih to obtain $u'\toll^* r'$, hence 
	$\tm\toat{0}^* u=\l x. u' \toll^* \l x.r'=r $.
	\item $r=r_pr_q$.  The sequence $u  \toat{>0}^* r$ never use a $\betav$-rule (since all steps have depth $>0$) therefore 
	(by \reflemma{basicCbV}) $u=pq$, with $p\tobv^* r_p$ and $q\tobv^* r_q$. Since  $r=r_pr_q$ is normal, both $r_p$ and $r_q$ are $\tobv$-normal.
	% By \reflem{l:basicCbV}, no term in 
	
	\begin{itemize}
		
	
		
		\item By \ih,
		$p \toll^*  r_p$ and $q \toll^* r_q$. 
		
		\item 
		% Observe that   since  $r=r_pr_q$ is normal, then $r_p$ is not an abstraction (and by \reflemma{basicCbV}, no term in $p\tobv^* r_p$) and  $r_q$ is not a value (and by \reflemma{basicCbV}, no term in $q\tobv^* r_q$). 
		 
		 We  \emph{merge}  the steps in 	$p   \toll^* r_p$ and 
		 $q\toll^* r_q$ in increasing order, so to  conclude that $pq\toll^* r_pr_q$, hence 	$\tm\toat{0}^* u= pq\toll^* r_pr_q=r$. 
		
	\end{itemize}

	
\end{enumerate}
		In all cases, we have proved the claim.
\end{proof}

\newpage

\section{Least-Level Normalization  in CbN}



  \CF{Supponiamo di aver dimostrato surface factorization per CbN...}
\begin{theorem}[Surface \cbn factorization]
	\label{thm:cbn-fact0}
	If $\tm \tob^* \tmtwo$ then $\tm\tobat{0}^* \tms \tobat{>0}^* \tmu$.
\end{theorem}

Least-Level Normalization follows.

\begin{theorem}[CBN Normalization]
	if $\tm \tob^* r$ with $r$  $\tob$-normal, then $\tm\toll^*  \tmr$.
	
\end{theorem}

\begin{proof}	By induction on the term $r$.
	From $\tm \tob^* r$, 
	by  \refthm{weak-fact0}, we have that \begin{center}
		$\tm\tobat{0}^* u  \tobat{>0}^* r$.
	\end{center}
	
	Cases:
	
	
	\begin{enumerate}
		\item $r=x$. Then  $u=x$, and trivially  $\tm\tobat{0}^* r$.
		\item $r=\l x.r'$. Then $u=\l x. u'$, hence  $u' \tob^*  r'$, where  $ r' $ is $\tob$-normal, and we use the \ih to obtain $u'\toll^* r'$, hence 
		$\tm\tobat{0}^* u=\l x. u' \toll^* \l x.r'=r $.
		\item $r=r_pr_q$.  The sequence $u  \tobat{>0}^* r$ never use a $\beta$-rule, therefore (by \reflemma{basicCbN}), $u=pq$, with $p\tob^* r_p$ and $q\tob^* r_q$. 
		Since $r=r_pr_q$ is normal, then  both  $r_p$ and $r_q$ are $\tob$-normal. 
		
		\begin{itemize}
			
			
			\item By \ih,
			$p \toll^*  r_p$ and $q \toll^* r_q$. 
			
			\item %Since $r=r_pr_q$ is normal, $ r_p$ is not an abstraction (and by \reflemma{basicCbV} no term in the sequence $p\tob^* r_p$). 
			
			  We   \emph{merge}  the steps of	$p   \toll^* r_p$ and 
			$q\toll^* r_q$ in increasing order, so to  conclude that $pq\toll^* r_pr_q$, hence 	$\tm\tobat{0}^* u= pq\toll^* r_pr_q=r$
			
		\end{itemize}
		
		
	\end{enumerate}
	In all cases, we have proved the claim.
\end{proof}

\newpage

\section{Left-Most Normalization in CbN}



\begin{theorem}[Head  factorization]
	\label{thm:cbn-fact0}
	If $\tm \tob^* \tmtwo$ then $\tm\toh^* \tms \tonoth^* \tmu$.
\end{theorem}

\begin{theorem}[CBN Normalization]
	if $\tm \tob^* r$ with $r$  $\tob$-normal, then $\tm\tolo^*  \tmr$.
	
\end{theorem}

\begin{proof}	By induction on the term $r$.
	From $\tm \tob^* r$, 
	by Head Factorization, we have that 
	\begin{center}
		$\tm\toh^* u  \tonoth^* r$.
	\end{center}
	
	Cases:
	
	
	\begin{enumerate}
		\item $r=x$. Then  $u=x$, and trivially  $\tm\toh^* r$.
		\item $r=\l x.r'$. Then $u=\l x. u'$, hence  $u' \tob^*  r'$, where  $ r' $ is $\tob$-normal, and we use the \ih to obtain $u'\tolo^* r'$, hence 
		$\tm\toh^* u=\l x. u' \tolo^* \l x.r'=r $.
		\item $r=r_pr_q$.  The sequence $u  \tonoth^* r$ never use a $\beta$-rule, therefore, $u=pq$, with $p\tob^* r_p$ and $q\tob^* r_q$. Observe that (i) $r_p$ and $r_q$ are $\tob$-normal and (ii) $r_p$ is not an abstraction  (because $r_pr_q$ is normal). 
		
		\begin{itemize}
			
			
			\item By \ih,
			$p \tolo^*  r_p$ and $q \tolo^* r_q$. 
			
			\item Because of  (ii) and \reflemma{basicCbN},  no term in the sequence 	$p   \tolo p_1 \tolo  \dots \tolo r_p$ is an abstraction. Hence  $pq \tolo p_1q\tolo \dots    \tolo r_pq$.    Since $r_p$ is normal and not an abstraction, from  $q \tolo^* r_q$  we also have $r_pq \tolo^* r_pr_q$.
		\end{itemize}
		
		
	\end{enumerate}
	In all cases, we have proved the claim.
\end{proof}





\end{document}

\section{Factorization by Level in CbV}
With the obvious CbV definitions of depth of the $\betav$ step $\toat{k}$ and of least-level of a term $\deg t$,
given surface factorization, we obtain factorization by level by induction.

\begin{theorem}[Weak \cbv factorization]
	\label{thm:weak-fact0}
	If $\tm \tobv^* \tmtwo$ then $\tm\toat{0}^* \tms \toat{>0}^* \tmu$.
\end{theorem}

\begin{theorem}[CBV \emph{\ll factorization}]
 if $\tm \tobv^* r$ then $\tm\toe^* \cdot \toi^* \tmr$.

\end{theorem}

\begin{proof}From $\tm \tobv^* r$, 
by  \refthm{weak-fact0}, we have that \begin{center}
	$\tm\toat{0}^* u  \toat{>0}^* r$.
\end{center}
We observe that the sequence $u  \toat{>0}^* r$ has the  property \#: no step  in the sequence  is a $\beta$-rule.
We   prove by induction on $r$ the following statement, from which the claim follows by taking $k=\deg r$

\begin{center}
	\emph{	
	If 	$ u  \tobv^* r $ and \# holds, then $u \toe^* \cdot \toat{>k}^* r$, for each $k\leq \deg r $, }
\end{center}



	We procede by cases. 

\begin{enumerate}
	\item $r=x$. Trivial
	\item $r=\l x.q$ 	Then $u=\l x. p$, hence  $p \tobv^*  q$, and we use the \ih.
	\item $r=r_pr_q$.  Because of \#, \ie the sequence never use a $\beta$-rule, therefore, $u=pq$, with $p\tobv^* r_p$ and $q\tobv^* r_q$.
	
\begin{itemize}
	\item 	Observe that by def. of $\deg r$, if  $k\leq \deg r $ then $k\leq \deg{ r_p}$ and $k \leq \deg {r_q}$. 
	
	\item 	By  \refthm{weak-fact0}, $p \toat{0}^* p' {\toat {>0}}^* r_p$ and $q \toat{0}^* q' {\toat {>0}}^* r_q$
	
	\item By \ih,
		$p' \toe^* p'' {\toat {>k}}^* r_p$ and $q' \tobv^* q'' {\toat {>k}}^* r_q$. 
	
	\item 	By merging 	$p \toat{0}^*p'  \toe^* p''$ and 
		$q \toat{0}^* q'\tobv^* q''$ in increasing order, we conclude that $pq\toe^* p''q''$.
		
		\item We also have 
		 $  p''q'' \toat {>k} r_pq'' \toat {>k} r_pr_q$.
\end{itemize}
Hence we have proved the statement.

%	\item $N=!S$. Then $U= !P$, hence  $P\parredb S$, and we use the \ih.
%	\item $N=ST$. Therefore,  $U=PQ$,  $P\parredb S$ and $Q\parredb T$.  By def., if  $k\leq \deg N $ then $k\leq \deg S$ and $k \leq \deg T$. 
%	
%	By \ih,
%	$P \eredb^* P'  \parredb  \at {>k} S$ and $Q \eredb^* Q'  \parredb \at {>k} T$. We conclude that $PQ\eredb^* P'Q'$
%	and $  P'Q' \parredb \at {>k} ST$
\end{enumerate}

\end{proof}




\SLV{}{
\begin{lemma} 	If $M\parredb N$ then $M\eredb^* \cdot  \iparredb N$
	
	
\end{lemma}

\begin{proof}By Lemma \ref{lem:split0}, we have that $M\sred^* U \dparred N$.
	We   prove by induction on $N$ the following, from which the claim follows by taking $k=\deg N$
	
	
	\begin{center}
		\emph{	For each $k\leq \deg N$, 
			$U\eredb^* \cdot  \parredb \at {>k} N$}
	\end{center}
	
	We procede by cases. 
	
	\begin{enumerate}
		\item $N=x$. ok
		\item $N=\lam x.S$ Then $U=\lam x. P$, hence  $P\parredb S$, and we use the \ih.
		\item $N=!S$. Then $U= !P$, hence  $P\parredb S$, and we use the \ih.
		\item $N=ST$. Therefore,  $U=PQ$,  $P\parredb S$ and $Q\parredb T$.  By def., if  $k\leq \deg N $ then $k\leq \deg S$ and $k \leq \deg T$. 
		
		By \ih,
		$P \eredb^* P'  \parredb  \at {>k} S$ and $Q \eredb^* Q'  \parredb \at {>k} T$. We conclude that $PQ\eredb^* P'Q'$
		and $  P'Q' \parredb \at {>k} ST$
	\end{enumerate}
	
\end{proof}
}

%Note that if $\tm \tob \tmtwo$ then either $\tm \tostrat \tmtwo$ or $\tm \tonotstrat \tmtwo$ .


% \paragraph{A normalizing strategy for $\tob$.}
% We prove that $(\Lambda, \{\tost,\tonst \})$ is a \emph{complete \external system.} 
% The  crucial properties of are the following.
% \begin{lemma}\label{l:st_basics}
% 
% \begin{enumerate}
% 	\item  $\tm$ is $\tob$-normal iff $\tm$ is $\tost$-normal.
% 	\item  If $\tm \tonst \tms$ then $\Deg \tm = \Deg \tms$.
% 			\NoteProof{lappendix:perpetuity-strat}
% 	\item The $\tost$-step has uniform termination.		
% \end{enumerate}
% \end{lemma}
%  \emph{Completeness} is Point 1. above, which is  immediate: if $\tm$ has any reduction, there exists one of minimal depth. \emph{Persistence} is immediate consequence of Point 2. above,  together with 
% \refprop{deg}. Clearly,  $\Deg \tm \not= \infty$. Since  $\tonst$-step does not change the minimal depth of the term, it means that a reduction is still available from $\tms$. \emph{Uniform termination} is obtained 
% by the standard technique to show that $\tost$ satisfies a diamond-like property. 
% Finally,\emph{ terminal factorization} follows from $\tost$-factorization (\refth{norm_st}) which we prove with  our standard technique
% \cf{(as we discuss in the next paragraph)}.
% With all these elements, \refprop{parallelsplit-gives-fact} gives us a proof that
% \begin{theorem}[Normalizing strategy]
% 	$\tost$ is a normalizing strategy for $\tob$
% \end{theorem}
% 
% 
% 
% \paragraph{\Stratified Factorization.} 
% 
% 
% 
% We prove  that  $(\Lambda, \{ \tost, \tonst \})$ is a \macrostep\ system, with $\partob,\partonst$ as \macrostep s.
% Observe that 
% $\tob \,\subseteq\, \partob\subseteq\, \tob^*$ and $\tonotstrat \,\subseteq\, \partonotstrat \,\subseteq\, \tonotstrat^*$, as required by \refdef{macrostep}. %Observe also that  $\tostratind{k} \,\subseteq\, \partostratind{k}$.
%  As usual, we  prove the merge and split properties.
% 
% 
% \begin{theorem}\label{th:norm_st}$\tob$ satisfies $\tost$-factorization: $\tob^* ~\subseteq~ \tost^*\tonst^*$
% \end{theorem}
% 
% 
% 
% \newcounter{prop:i-e-merge-strat}
% \addtocounter{prop:i-e-merge-strat}{\value{proposition}}
%\begin{proposition}[Merge]
%	\label{prop:i-e-merge-strat}
%	\NoteProof{propappendix:i-e-merge-strat}
%%	\begin{enumerate}
%%		\item\label{p:i-e-merge-strat-ind} If $\tm \partostratind{k}\tmtwo \tostratind{m} \tmthree$ with \mbox{$n > m$}, then $\tm \partob \tmthree$.% and $\tm \tostratind{m} \tmfour$ for some term $\tmfour$.
%%		\item\label{p:i-e-merge-strat-notstrat} If $\tm \partonotstrat \tmtwo \tostrat \tmthree$, then $\tm \partob \tmthree$.
%%	\end{enumerate}
%\label{p:i-e-merge-strat-notstrat} If $\tm \partonotstrat \tmtwo \tostrat \tmthree$, then $\tm \partob \tmthree$.
%\end{proposition}
%
%\RED{\newcounter{prop:quant-out-in-split-strat}
%\addtocounter{prop:quant-out-in-split-strat}{\value{proposition}}
%\begin{proposition}[Indexed Split]
%	\label{prop:quant-out-in-split-strat}
%	\NoteProof{propappendix:quant-out-in-split-strat}
%	If $\tm \partobind n \tmtwo$ then either $\tm \partonotstrat\tmtwo$ or $n>0$ and there exists $\tmthree$ such that $\tm \tostrat \tmthree \partobindlong {n-1} \tmtwo$.
%\end{proposition}}
%
%\begin{corollary}[Split]
%	If $\tm \partob \tmtwo$ then there exists $\tmthree$ such that $\tm \tost^* \tmthree \partonoth\tmtwo$.
%\end{corollary}


%
%
%A key-property of $\tostrat$ is \emph{persistence}. We show  $\partonotstrat$ does not increase the degree of a term, \ie if $\tm \partonotstrat \tmtwo$ then a (residual of a) $\beta$-redex of minimal depth in $\tm$ is still present in $\tmtwo$ with the same depth.
%
%\newcounter{l:perpetuity-strat}
%\addtocounter{l:perpetuity-strat}{\value{lemma}}
%\begin{lemma}[Persistence]
%	\label{l:perpetuity-strat}
%	\NoteProof{lappendix:perpetuity-strat}
%	\begin{enumerate}
%		\item If $\tm \parto \tmtwo$ then $\Deg{\tmtwo} \geq \Deg{\tm}$. 
%		\item 	If $\tm \partonotstrat \tmtwo$ then $\Deg{\tmtwo} = \Deg{\tm}$. 
%	\end{enumerate}
%\end{lemma}


==> proofs/proofs-abstrac-rew.tex <==
\subsection{Omitted proofs  of \refsect{abstract-rewriting} (Factorization and Normalization, Abstractly)}

\begin{theorem}[Essential normalization]	
Let $\rewsys$ be an  \external system. If $\tm \to^* \tmtwo$ and $\tmtwo$ is a $\toe$-normal form then $\tm$ is strongly $\toe$-normalizing. 	
\end{theorem}


\begin{proof}
	Assume $\tm \to^* \tmu$ with $\tmu$  $\toe$-normal. Then:
	\begin{enumerate}
		
		\item  \emph{Terminal factorization} implies  $\tm \toe^*\tms \toi^* \tmu$.
		\item Let us show that $\tms$ is $\toe$-normal: if it is not then $\tms$ a straightforward induction on the length of $\tms \toi^*\tmu$ iterating \emph{persistence} gives that $\tmu \toe \tmfive$ for some $\tmfive$, against the hypothesis that $\tmu$ it is $\toe$-normal. Absurd.	We have then proved that that $\tms$ is $\toe$-normal.
	
	
	\item By the previous point $\tm$ is weakly $\toe$-normalizing. By \emph{uniform termination}, $\toe$ is strongly normalizing. \qedhere
	\end{enumerate}
\end{proof}


==> proofs/proofs-headBIS.tex <==
% !TEX root = ../main.tex
\subsection{Omitted proofs  of \refsect{lambda} ($\l$-calculus)}

\setcounter{lemmaAppendix}{\value{l:partobind-subs}}
\begin{lemmaAppendix}[Substitutivity of $\partobind n$]
	\label{lappendix:partobind-subs} % \reflemmap{tob-subs}{ind-par}
	\NoteState{l:partobind-subs}
If $\tm \partobind n \tm'$ and $\tmtwo \partobind m \tmtwo'$ then $\tm \isub\var\tmtwo \partobind {n + \sizep{\tm'}\var\cdot m} \tm' \isub\var{\tmtwo'}$.
\end{lemmaAppendix}

\begin{proof}
By induction on $\tm \partobind n \tm'$. Cases:
\begin{itemize}
	\item \emph{Variable}: two sub-cases
	\begin{itemize}
	\item $\tm = \var$: then $\tm = \var \partobind 0 \var = \tm'$ then $\tm \isub\var\tmtwo = \var\isub\var\tmtwo = \tmtwo \partobind m \tmtwo' = \var \isub\var{\tmtwo'} = \tm' \isub\var{\tmtwo'}$ that satisfies the statement because $n + \sizep{\tm'}\var\cdot m = 0+1\cdot m = m$. 
	 \item $\tm = \vartwo$: then $\tm = \vartwo \partobind 0 \vartwo = \tm'$ then $\tm \isub\var\tmtwo = \vartwo\isub\var\tmtwo = \vartwo \partobind 0 \vartwo = \vartwo \isub\var{\tmtwo'} = \tm' \isub\var{\tmtwo'}$ that satisfies the statement because $n + \sizep{\tm'}\var\cdot m = n +0\cdot m=n$.
	 \end{itemize}
	
	\item \emph{Abstraction}, \ie $\tm = \la{\vartwo}{\tmthree} \partobind{n} \la{\vartwo}{\tmthree'} = \tm'$ because $\tmthree \partobind{n} \tmthree'$; we can suppose without loss of generality that $\vartwo \neq \var$, hence $\sizep{\tmthree'}{\var} = \sizep{\tm'}{\var}$ and $\tm\isub{\var}{\tmtwo} = \la{\vartwo}(\tmthree\isub{\var}{\tmtwo})$ and $\tm'\isub{\var}{\tmtwo'} = \la{\vartwo}(\tmthree'\isub{\var}{\tmtwo'})$.
		By \ih, $\tmthree\isub{\var}{\tmtwo} \partobindlong{n +  \sizep{\tmthree'}{\var} \cdot m} \tmthree'\isub{\var}{\tmtwo'}$, thus
		\begin{align*}
		\AxiomC{$\tmthree\isub{\var}{\tmtwo} \partobindlong{n +  \sizep{\tmthree'}{\var} \cdot m} \tmthree'\isub{\var}{\tmtwo'}$}
		%%\RightLabel{$\parRew{\l}$}
		\UnaryInfC{$\tm\isub{\var}{\tmtwo} = \la {\vartwo}\tmthree\isub{\var}{\tmtwo} \partobindlong{n +  \sizep{\tm'}{\var} \cdot m} \la{\vartwo}\tmthree'\isub{\var}{\tmtwo'} = \tm'\isub{\var}{\tmtwo'}$}
		\DisplayProof\,.
		\end{align*}		


	
	\item \emph{Application}, \ie	
	\[\AxiomC{$\tmthree \partobind {n_\tmthree} \tmthree'$}
	\AxiomC{$\tmfour \partobind {n_\tmfour} \tmfour'$}
	%\RightLabel{$\parRew{@}$}
	\BinaryInfC{$\tm = \tmthree \tmfour \partobindlong {n_\tmthree + n_\tmfour} \tmthree' \tmfour'= \tm'$}
	\DisplayProof\]
	with $n = n_\tmthree + n_\tmfour$. By \ih, $\tmthree\isub\var\tmtwo \partobindlong {n_\tmthree +\sizep{\tmthree'}\var \cdot m} \tmthree'\isub\var{\tmtwo'}$ and $\tmfour\isub\var\tmtwo \partobindlong {n_\tmfour +\sizep{\tmfour'}\var \cdot m} \tmfour'\isub\var{\tmtwo'}$. Then 
	\[\AxiomC{$\tmthree\isub\var\tmtwo \partobindlong {n_\tmthree +\sizep{\tmthree'}\var \cdot m} \tmthree'\isub\var{\tmtwo'}$}
	\AxiomC{$\tmfour\isub\var\tmtwo \partobindlong {n_\tmfour +\sizep{\tmfour'}\var \cdot m} \tmfour'\isub\var{\tmtwo'}$}
	%\RightLabel{$\parRew{@}$}
	\BinaryInfC{$\tm\isub\var\tmtwo = \tmthree\isub\var\tmtwo \tmfour\isub\var\tmtwo \partobindlong {n_\tmthree +\sizep{\tmthree'}\var \cdot m +n_\tmfour +\sizep{\tmfour'}\var \cdot m} \tmthree'\isub\var{\tmtwo'} \tmfour'\isub\var{\tmtwo'}= \tm'\isub\var{\tmtwo'}$}
	\DisplayProof\]
that proves the statement because $$n_\tmthree +\sizep{\tmthree'}\var \cdot m +n_\tmfour +\sizep{\tmfour'}\var \cdot m = n + (\sizep{\tmthree'}\var + \sizep{\tmfour'}\var)\cdot m = n + \sizep{\tm'}\var \cdot m$$

\item $\beta$, \ie
	\[\AxiomC{$\tmthree \partobind {n_\tmthree} \tmthree'$}
	\AxiomC{$\tmfour \partobind {n_\tmfour} \tmfour'$}
%\RightLabel{$\parRew{\beta}$}
\BinaryInfC{$\tm = (\la\vartwo \tmthree)\tmfour \partobindlong {n_\tmthree + \sizep{\tmthree'}\vartwo \cdot n_\tmfour +1} \tmthree'\isub \vartwo {\tmfour'} = \tm'$}
\DisplayProof\]
with $n = n_\tmthree + \sizep{\tmthree'}\vartwo \cdot n_\tmfour +1$. We can assume without loss of generality that $\vartwo\neq \var$,
		hence $\sizep{\tm'}{\var} = \sizep{\tmthree'\isub\vartwo {\tmfour'}}\var = \sizep{\tmthree'}{\var} + \sizep{\tmthree'}{\vartwo}\cdot\sizep{\tmfour'}{\var} $ and $\tm\isub\var\tmtwo = (\la\vartwo\tmthree\isub\var\tmtwo) (\tmfour\isub\var\tmtwo)$ and $\tm'\isub\var{\tmtwo'} = \tmthree'\isub\var{\tmtwo'} \isub\vartwo{\tmfour'\isub\var{\tmtwo'}}$.
		
		By \ih, $\tmthree\isub\var\tmtwo \partobindlong {n_\tmthree +\sizep{\tmthree'}\var \cdot m} \tmthree'\isub\var{\tmtwo'}$ and $\tmfour\isub\var\tmtwo \partobindlong {n_\tmfour +\sizep{\tmfour'}\var \cdot m} \tmfour'\isub\var{\tmtwo'}$. Then 
	\[\AxiomC{$\tmthree\isub\var\tmtwo \partobindlong {n_\tmthree +\sizep{\tmthree'}\var \cdot m} \tmthree'\isub\var{\tmtwo'}$}
	\AxiomC{$\tmfour\isub\var\tmtwo \partobindlong {n_\tmfour +\sizep{\tmfour'}\var \cdot m} \tmfour'\isub\var{\tmtwo'}$}
	%\RightLabel{$\parRew{\beta}$}
	\BinaryInfC{$\tm\isub\var\tmtwo = (\la\vartwo\tmthree\isub\var\tmtwo) (\tmfour\isub\var\tmtwo) \partobindlong {n_\tmthree +\sizep{\tmthree'}\var \cdot m +\sizep{\tmthree'}\vartwo\cdot(n_\tmfour +\sizep{\tmfour'}\var \cdot m)+1} \tmthree'\isub\var{\tmtwo'} \isub\vartwo{\tmfour'\isub\var{\tmtwo'}}= \tm'\isub\var{\tmtwo'}$}
\DisplayProof\]

The number on the $\parto$ arrow satisfies
$$n_\tmthree +\sizep{\tmthree'}\var \cdot m +\sizep{\tmthree'}\vartwo\cdot(n_\tmfour +\sizep{\tmfour'}\var \cdot m)+1 
=
\underbrace{n_\tmthree + \sizep{\tmthree'}\vartwo\cdot n_\tmfour + 1}_n + \underbrace{\sizep{\tmthree'}\var \cdot m + \sizep{\tmthree'}\vartwo\cdot \sizep{\tmfour'}\var \cdot m}_{\sizep{\tm'}\var\cdot m}$$
\end{itemize}
\end{proof}

\subsection{Omitted proofs  of \refsect{head} (head)}

\setcounter{propositionAppendix}{\value{prop:quant-out-in-split}}
\begin{propositionAppendix}[Head macro-step system]
	\label{propappendix:quant-out-in-split}
	\NoteState{prop:quant-out-in-split}
	\hfill
	\begin{enumerate}
		\item\label{p:quant-out-in-split-merge} \emph{Merge}: if $\tm \partonoth\cdot \toh \tmthree$ then $\tm \partob \tmthree$.
		\item\label{p:quant-out-in-split-indexed} \emph{Indexed split}: if $\tm \partobind n \tmtwo$ then $\tm \partonoth\tmtwo$, or $n>0$ and $\tm \toh \cdot \partobind {n-1} \tmtwo$.
		
		\item\label{p:quant-out-in-split-split} \emph{Split}: if $\tm \partob \tmtwo$ then $\tm \toh^* \cdot \partonoth\tmtwo$.
	\end{enumerate}
	that is, $(\Lambda, \{ \toh, \tonoth \})$ is a \macrostep\ system with respect to $\partob,\partonoth$.
\end{propositionAppendix}

\begin{proof}
	\refpoints{quant-out-in-split-indexed}{quant-out-in-split-split} are already proved on p.~\pageref{prop:quant-out-in-split}.
	We prove \refpoint{quant-out-in-split-merge} by induction on the definition of $\tm \partonoth \tmtwo$.
	Cases:
	\begin{itemize}
		\item \emph{Variable}: $\tm = \var \partonoth \var = \tmtwo$. 
		Then, there is no $\tmthree$ such that $\tmtwo \toh \tmthree$.
		
		\item \emph{Abstraction}: $\tm = \la \var\tm' \partonoth  \la \var \tmtwo' = \tmtwo$ because $\tm' \partonoth \tmtwo'$.
		According to the definition of $\tmtwo \toh \tmthree$, necessarily $\tmthree = \la{\var}{\tmthree'}$ with $\tmtwo' \toh \tmthree'$.
		By \ih applied to $\tm'$, we have $\tm' \partob \tmthree'$ and hence:
		\begin{align*}
			\AxiomC{$\tm' \partob \tmthree'$}
			\UnaryInfC{$\tm = \la{\var}{\tm'} \partob \la{\var}{\tmthree'} = \tmthree$}
			\DisplayProof
			\,.
		\end{align*}
	
		\item \emph{Application}:
		\begin{align}
		\label{eq:app}
		\AxiomC{$\tmfour \partonoth \tmfour'$}
		\AxiomC{$\tmfive \partob \tmfive'$}
		\BinaryInfC{$\tm = \tmfour\tmfive \partonoth \tmfour'\tmfive' = \tmtwo$}
		\DisplayProof
		\end{align}	
		Sub-cases:
		\begin{enumerate}
			\item $\tmtwo = \tmfour'\tmfive' \toh \tmfour''\tmfive' = \tmthree$ with $\tmfour' \toh \tmfour''$; 
			by \ih applied to $\tmfour \partonoth \tmfour' \toh \tmfour''$, we have $\tmfour \partob \tmfour''$, and so (as $\partonoth \,\subseteq\, \partob$)
			\begin{align*}
			\AxiomC{$\tmfour \partob \tmfour''$}
			\AxiomC{$\tmfive \partob \tmfive'$}
			\BinaryInfC{$\tm = \tmfour\tmfive \partob \tmfour''\tmfive' = \tmthree$}
			\DisplayProof\,;
			\end{align*}
			
			\item $\tmtwo = (\la{\var}\tmsix')\tmfive' \toh \tmsix'\isub{\var}{\tmfive'} = \tmthree$, which means that $\tmfour' = \la{\var}{\tmsix'}$ in \eqref{eq:app}.
			According to the definition of $\tmfour \partonoth \tmfour'$, necessarily $\tmfour = \la{\var}{\tmsix}$ with $\tmsix \partonoth \tmsix'$.
			Thus, (as $\partonoth \,\subseteq\, \partob$)
			\begin{align*}
			\AxiomC{$\tmq\partob \tmq'$}
			\AxiomC{$\tmfive \partob \tmfive'$}
			\BinaryInfC{$\tm =  (\la {\var} \tmsix) \tmfive \partob  \tmq'\isub{\var}{\tmfive'} = \tmthree$}
			\DisplayProof
			\,.
			\end{align*}
		\end{enumerate}
		\item \emph{$\beta$-redex}:
		\begin{align*}
			\AxiomC{$\tmfour \partob \tmfour'$}
			\AxiomC{$\tmfive \partob \tmfive'$}
			\BinaryInfC{$\tm = (\la\var \tmfour) \tmfive \partonoth (\la\var \tmfour') \tmfive' = \tmtwo$}
			\DisplayProof
		\end{align*}
		According to the definition of $\tmtwo \toh \tmthree$, we have $\tmthree = \tmfour'\isub{\var}{\tmfive'}$.
		Hence,
		\begin{align*}
			\AxiomC{$\tmfour \partob \tmfour'$}
			\AxiomC{$\tmfive \partob \tmfive'$}
			\BinaryInfC{$\tm = (\la\var \tmfour) \tmfive \partob \tmfour'\isub{\var}{\tmfive'} = \tmthree$}
			\DisplayProof
		\end{align*}
		\qedhere
	\end{itemize}
\end{proof}

\begin{proposition}[Head essential system]
\begin{enumerate}
 \item \emph{Persistence}: if $\tm \toh \tmtwo$ and $\tm \tonoth \tmthree$ then $\tmthree \toh \tmfour$ for some $\tmfour$.
 \item \emph{Determinism}: if $\tm \toh \tmtwo_1$ and $\tm\toh \tmtwo_2$ then $\tmtwo_1 = \tmtwo_2$.
\end{enumerate}
Then, $(\Lambda, \set{ \tow, \tonotw})$ is an essential system.
\end{proposition}

\begin{proof}
\begin{enumerate}
 \item \emph{Persistence}: by induction on $\tm \toh \tmtwo$. Cases:
 \begin{itemize}
  \item \emph{Root step}, \ie $\tm = (\la\var \tmfive) \tmsix \toh \tmfive\isub\var\tmsix = \tmtwo$. Sub-cases:
  \begin{itemize}
    \item \emph{$\tonoth$ in the left sub-term}: $\tm = (\la\var \tmfive) \tmsix \tonoth (\la\var \tmfive') \tmsix=\tmthree$ because $\tmfive \tob \tmfive'$ or $\tmfive \tonoth \tmfive'$. In both cases $\tmthree = (\la\var \tmfive') \tmsix \toh \tmfive'\isub\var\tmsix =:\tmfour$.
    
    \item \emph{$\tonoth$ in the right sub-term}: $\tm = (\la\var \tmfive) \tmsix \tonoth (\la\var \tmfive) \tmsix'=\tmthree$ because $\tmsix \tob \tmsix'$. Then $\tmthree = (\la\var \tmfive) \tmsix' \toh \tmfive\isub\var{\tmsix'} =:\tmfour$.    
  \end{itemize}
  \item \emph{Application}: \ie $\tm = \tmfive \tmsix \toh \tmfive'\tmsix = \tmtwo$ with $\tmfive \toh \tmfive'$ and $\tmfive$ not an abstraction. Sub-cases:
  \begin{itemize}
    \item \emph{$\tonoth$ in the left sub-term}: $\tm = \tmfive \tmsix \tonoth \tmfive'' \tmsix=\tmthree$ because $\tmfive \tonoth \tmfive''$. By \ih, $\tmfive'' \toh \tmfour'$ for some $\tmfour'$. Then $\tmthree = \tmfive'' \tmsix \toh \tmfour'\tmsix =:\tmfour$.
    
    \item \emph{$\tonoth$ in the right sub-term}: $\tm = \tmfive \tmsix \tonoth \tmfive \tmsix'=\tmthree$ because $\tmsix \tob \tmsix'$. Then $\tmthree = \tmfive \tmsix' \toh \tmfive'\tmsix' =:\tmfour$.   
  \end{itemize}
  \item \emph{Abstraction}: \ie $\tm = \la\var \tmfive \toh \tmfive' = \tmtwo$. Then $\tm = \la\var \tmfive \tonoth \la\var\tmfive'' = \tmthree$ for some $\tmfive''$ with $\tmfive \tonoth \tmfive''$. By \ih, $\tmfive'' \toh \tmfour'$ for some $\tmfour'$. Then $\tmthree = \la\var\tmfive'' \toh \la\var\tmfour'$.
 \end{itemize}

 \item \emph{Determinism}: \ben{to do}.
\end{enumerate}
 
\end{proof}

\begin{proof} By induction on $\tm$. 
	We show   that for each possible case  of $\tm$, persistence holds, and only one reduction applies (\emph{determinism}). 
		\begin{itemize}
			\item $\tm = (\la\var \tmfive)$. Only the  \emph{root step} applies. Since $\tm \tonoth \tmthree$ we have 
			\begin{itemize}
				\item either  $ (\la\var \tmfive) \tmsix \tonoth (\la\var \tmfive') \tmsix=\tmthree$. %The  \emph{root step} still applies to $\tmthree$.
				
				\item or $  (\la\var \tmfive) \tmsix \tonoth (\la\var \tmfive) \tmsix'=\tmthree$. 
			\end{itemize}
		In both cases,  the  \emph{root step}  applies to $\tmthree$.
		
			\item  $\tm = \tmfive \tmsix $ with $\tmfive$ not an abstraction. Only rule 2. applies, and  $\tmfive \toh \tmfive'$.
			Since $\tm \tonoth \tmthree$ we have 
			\begin{itemize}
				\item either  $  \tmfive \tmsix \tonoth  \tmfive' \tmsix=\tmthree$, where $\tmfive'$ is not an abstraction
				
				\item or $  \tmfive \tmsix \tonoth  \tmfive \tmsix'=\tmthree$, where $\tmfive$ is not an abstraction.
			\end{itemize}
					In both cases, rule 2.  applies to $\tmthree$.
			
			 
		
			\item  $\tm = \la\var \tmfive $. Only rule 3. applies, with a premiss $\tmfive \toh \tmfive'$. We also have 
			  $\tm = \la\var \tmfive \tonoth \la\var\tmfive''$, which gives  $\tmfive \tonoth \tmfive''$. By \ih, $\tmfive'' \toh \tmfour'$ for some $\tmfour'$. Then rule 3. applies to  $\tmthree = \la\var\tmfive''$.
		\end{itemize}
		
	
	
\end{proof}


==> proofs/proofs-stratified-cbn-degree.tex <==
% !TEX root = ../main.tex
\subsection{Omitted proofs and lemmas of \refsect{stratified-cbn}}




\setcounter{lemmaAppendix}{\value{l:perpetuity-strat}}
\begin{lemmaAppendix}[Persistence]
\label{lappendix:perpetuity-strat}
\NoteState{l:perpetuity-strat}
	If $\tm \partonotstrat \tmtwo$ then $\Deg{\tmtwo} \leq \Deg{\tm}$. 
\end{lemmaAppendix}

\begin{proof}
	By hypothesis, $\tm \partostratind{n} \tmtwo$ for some $n > \Deg{\tm}$.
	We prove that $\Deg{\tmtwo} \leq \Deg{\tm}$ by induction on the definition of $\tm \partostratind{n} \tmtwo$.
	Cases:
	\begin{itemize}
		\item \emph{Variable}: $\tm = \var \partostratind{\infty} \var = \tmtwo$. 
		Then, $\Deg{\tm} = \infty = \Deg{\tmtwo}$.
		
		\item \emph{Abstraction}: $\tm = \la \var\tm' \partostratind{n}  \la \var \tmtwo' = \tmtwo$ because $\tm' \partostratind{n} \tmtwo'$.
		As $n > \Deg{\tm} = \Deg{\tm'}$, then $\Deg{\tmtwo} = \Deg{\tmtwo'} \leq \Deg{\tm'} = \Deg{\tm}$ by \ih
		
		\item \emph{Application}:
		\begin{align*}
		\AxiomC{$\tm_0 \partostratind{n_0} \tmtwo_0$}	
		\AxiomC{$\tm_1 \partostratind{n_1} \tmtwo_1$}
		\BinaryInfC{$\tm = \tm_0 \tm_1 \partostratind{n} \tmtwo_0 \tmtwo_1 = \tmtwo$}
		\DisplayProof 
		\end{align*}
		where $n = \min\{n_0,n_1+1\}$.
		According to the definition of $\Deg{\tm}$, there are the following sub-cases:
		\begin{enumerate}
			\item $\Deg{\tm} = \Deg{\tm_0} \leq \Deg{\tm_1} + 1$ and $\tm_0$ is not an abstraction; 
			%here it is important to take the min in the for the index application case of the definition of \partostratind{n}
			by \ih applied to $\tm_0$ (since $\Deg{\tm_0} = \Deg{\tm} < n \leq n_0$), we have $\Deg{\tmtwo_0} \leq \Deg{\tm_0}$, and so (as $\Deg{\tm_0} \leq \Deg{\tm_1} + 1$) $\Deg{\tmtwo} = \min \{\Deg{\tmtwo_0}, \Deg{\tmtwo_1} + 1\} \leq \min\{\Deg{\tm_0}, \Deg{\tm_1} + 1\} = \Deg{\tm}$.
			
			\item $\Deg{\tm} = \Deg{\tm_1} + 1 \leq \Deg{\tm_0}$ and $\tm_0$ is not an abstraction; 
			%here it is important to take the min in the for the index application case of the definition of \partostratind{n}
			by \ih applied to $\tm_1$ (since $\Deg{\tm_1} + 1 = \Deg{\tm} < n \leq n_1+1$ and hence $\Deg{\tm_1} < n_1$), we have $\Deg{\tmtwo_1} \leq \Deg{\tm_1}$, and so (as $\Deg{\tm_1} + 1 \leq \Deg{\tm_0}$) $\Deg{\tmtwo} = \min \{\Deg{\tmtwo_0}, \Deg{\tmtwo_1} + 1\} \leq \min\{\Deg{\tm_0}, \Deg{\tm_1} + 1\} = \Deg{\tm}$.
			
			\item $\Deg{\tm} = 0$ and $\tm_0$ is an abstraction. 
			According to the definition of $\tm \partostratind{n} \tmtwo$, since $n > 0$, we have
				\begin{align*}
				\AxiomC{$\tm_0 \partostratind{n_0} \tmtwo_0$}
				\UnaryInfC{$\la{\var}\tm_0 \partostratind{n_0} \la{\var}\tmtwo_0$}
				\AxiomC{$\tm_1 \partostratind{n_1} \tmtwo_1$}
				\BinaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \partostratind{n} (\la{\var}{\tmtwo_0})\tmtwo_1 = \tmtwo$}
				\DisplayProof
				\end{align*}
				where $n = \min\{n_0, n_1+1\}$; therefore $\Deg{\tmtwo} = 0 = \Deg{\tm}$.
		\end{enumerate}
		
		\item \emph{$\beta$-step}: 
		\begin{align*}
		\AxiomC{}
		\UnaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \partostratind{0} \tm_0 \isub{\var}{\tm_1} = \tmtwo$}
		\DisplayProof
		\end{align*}
		where $0 = n > \Deg{\tm}$, which is impossible.
		\qedhere
	\end{itemize}
\end{proof}

%\begin{lemma}[Decomposition of parallel $n$-depth $\beta$-steps]
%	\label{l:decomp-strat}
%%	Let $\tm \partostratind{n} \tmtwo$ with $n \neq \infty$.
%%	\begin{enumerate}
%%		\item \label{p:decomp-strat-ind} Then, $\tm \tostratind{n} \tmthree \partostratind{j} \tmtwo$ for some term $\tmthree$ and some $j \geq n$ (possibly $j = \infty$).	
%%		
%%		\item\label{p:decomp-strat-notstrat} If moreover $\tm \partonotstrat \tmtwo$, then $n > 0 $ and $\tm \tostratind{k} \tmfour$ for some $\tmfour$ and some $k < n$.
%%	\end{enumerate}
%	If $\tm \partostratind{n} \tmtwo$ with $n \neq \infty$, then $\tm \tostratind{n} \tmthree \partostratind{j} \tmtwo$ for some term $\tmthree$ and some $j \geq n$ (possibly $j = \infty$).	
%\end{lemma}
%
%\begin{proof}
%	By induction on the definition of $\tm \partostratind{n} \tmtwo$. 
%		Cases:
%		\begin{itemize}
%			\item \emph{Variable}: $\tm = \var \partostratind{\infty} \var = \tmtwo$. 
%			This is impossible because $n \neq \infty$ by hypothesis.
%			
%			\item \emph{Abstraction}: $\tm = \la \var\tm' \partostratind{n}  \la \var \tmtwo' = \tmtwo$ because $\tm' \partostratind{n} \tmtwo'$. 
%			By \ih, $\tm' \tostratind{n} \tmthree' \partostratind{j} \tmtwo'$ for some term $\tmthree'$ and some $j \geq n$ (possibly $j = \infty$), so 
%			\begin{align*}
%			\AxiomC{$\tm' \tostratind{n} \tmthree'$}
%			\UnaryInfC{$\tm = \la{\var}{\tm'} \tostratind{n} \la{\var}{\tmthree'} = \tmthree$}
%			\DisplayProof
%			\qquad
%			\text{and}
%			\qquad
%			\AxiomC{$\tmthree' \partostratind{j} \tmtwo'$}
%			\UnaryInfC{$\tmthree = \la{\var}{\tmthree'} \partostratind{j} \la{\var}{\tmtwo'} = \tmtwo$}
%			\DisplayProof\,.
%			\end{align*}
%			
%			\item \emph{Application}:
%			\begin{align*}
%			\AxiomC{$\tm_0 \partostratind{n_0} \tmtwo_0$}	
%			\AxiomC{$\tm_1 \partostratind{n_1} \tmtwo_1$}
%			\BinaryInfC{$\tm = \tm_0 \tm_1 \partostratind{n} \tmtwo_0 \tmtwo_1 = \tmtwo$}
%			\DisplayProof 
%			\end{align*}
%			where $n = \min\{n_0,n_1+1\}$.
%			By \ih, $\tm_0 \tostratind{n_0} \tmthree_0 \partostratind{j_0} \tmthree_0$ and $\tm_1 \tostratind{n_1} \tmthree_1 \partostratind{j_1} \tmthree_1$ for some terms $\tmthree_0, \tmthree_1$ and some $j_0 \geq n_0$, $j_1 \geq n_1$ (possibly $j_0,j_1 = \infty$).
%			There are two possibilities:
%			\begin{enumerate}
%				\item $n = n_0$; then, $n_0 \leq n_1+1$ and 
%				\begin{align*}
%				\AxiomC{$\tm_0 \tostratind{n} \tmthree_0$}
%				\UnaryInfC{$\tm = \tm_0\tm_1 \tostratind{n} \tmthree_0\tm_1 = \tmthree$}
%				\DisplayProof
%				\qquad
%				\text{and}
%				\qquad
%				\AxiomC{$\tmthree_0 \partostratind{j_0} \tmtwo_0$}
%				\AxiomC{$\tm_1 \partostratind{n_1} \tmtwo_1$}
%				\BinaryInfC{$\tmthree = \tmthree_0\tm_1 \partostratind{j} \tmtwo_0\tmtwo_1 = \tmtwo$}
%				\DisplayProof
%				\end{align*}
%				where $j = \min\{j_0, n_1+1\} \geq n_0 = n$; 
%				\item $n = n_1+1$; then, $n_1 + 1 \leq n_0$ and  
%				\begin{align*}
%					\AxiomC{$\tm_1 \tostratind{n} \tmthree_1$}
%					\UnaryInfC{$\tm = \tm_0\tm_1 \tostratind{n} \tm_0\tmthree_1 = \tmthree$}
%					\DisplayProof
%					\qquad
%					\text{and}
%					\qquad
%					\AxiomC{$\tmthree_0 \partostratind{n_0} \tmtwo_0$}
%					\AxiomC{$\tm_1 \partostratind{j_1} \tmtwo_1$}
%					\BinaryInfC{$\tmthree = \tm_0\tmthree_1 \partostratind{j} \tmtwo_0\tmtwo_1 = \tmtwo$}
%					\DisplayProof
%				\end{align*}
%				where $j = \min\{n_0, j_1+1\} \geq n_1+1 = n$.
%			\end{enumerate}
%		
%			\item \emph{$\beta$-step}: 
%			\begin{align*}
%				\AxiomC{}
%				\UnaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \partostratind{0} \tm_0 \isub{\var}{\tm_1} = \tmtwo$}
%				\DisplayProof
%			\end{align*}
%			Let $\tmthree = \tmtwo$: then $\tmthree \partostratind{\infty} \tmtwo$ and
%			\begin{align*}
%				\AxiomC{}
%				\UnaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \tostratind{0} \tm_0 \isub{\var}{\tm_1} = \tmthree$}
%				\DisplayProof\,.
%			\end{align*}
%			\qedhere
%		\end{itemize}
%\end{proof}


%\setcounter{propositionAppendix}{\value{prop:i-e-merge-strat}}
\begin{propositionAppendix}[Internal-external merge]
	\label{propappendix:i-e-merge-strat}
	\NoteState{prop:i-e-merge-strat}
	\begin{enumerate}
		\item If $\tm \partostratind{n}\tmtwo \tostratind{m} \tmthree$ with $n > m$, then $\tm \partob \tmthree$. %and $\tm \tostratind{m} \tmfour$ for some term $\tmfour$.
		\item If $\tm \partonotstrat \tmtwo \tostrat \tmthree$, then $\tm \partob \tmthree$.
	\end{enumerate}
\end{propositionAppendix}

\begin{proof}\hfill
%	\begin{enumerate}
%		\item By induction on the definition of $\tm \partostratind{n} \tmtwo$.
%	Cases:
%		\begin{itemize}
%		\item \emph{Variable}: $\tm = \var \partostratind{\infty} \var = \tmtwo$. 
%		Then, there is no $\tmthree$ such that $\tmtwo \tostratind{m} \tmthree$ for any $m \in \nat$.
%		
%		\item \emph{Abstraction}: $\tm = \la \var\tm' \partostratind{n}  \la \var \tmtwo' = \tmtwo$ because $\tm' \partostratind{n} \tmtwo'$. 
%		According to the definition of $\tmtwo \tostratind{m} \tmthree$, by necessity $\tmthree = \la{\var}{\tmthree'}$ with $\tmtwo' \tostratind{m} \tmthree'$.
%		By \ih, $\tm' \partobv \tmthree'$ and $\tm' \tostratind{m} \tmfour'$ for some term $\tmfour'$, thus 
%		\begin{align*}
%			\AxiomC{$\tm' \partobv \tmthree'$}
%			\UnaryInfC{$\tm = \la{\var}{\tm'} \partobv \la{\var}{\tmthree'} = \tmthree$}
%			\DisplayProof
%			\qquad
%			\text{and}
%			\qquad
%			\AxiomC{$\tm' \tostratind{m} \tmfour'$}
%			\UnaryInfC{$\tm = \la{\var}{\tm'} \tostratind{m} \la{\var}{\tmfour'} = \tmfour$}
%			\DisplayProof\,.
%		\end{align*}
%		
%		\item \emph{Application}:
%		\begin{align*}
%			\AxiomC{$\tm_0 \partostratind{n_0} \tmtwo_0$}	
%			\AxiomC{$\tm_1 \partostratind{n_1} \tmtwo_1$}
%			\BinaryInfC{$\tm = \tm_0 \tm_1 \partostratind{n} \tmtwo_0 \tmtwo_1 = \tmtwo$}
%			\DisplayProof 
%		\end{align*}
%		where $n = \min\{n_0,n_1+1\}$.
%		According to the definition of $\tmtwo \tostratind{m} \tmthree$, there are the following sub-cases:
%		\begin{enumerate}
%			\item $\tmtwo = \tmtwo_0\tmtwo_1 \tostratind{m} \tmthree_0\tmtwo_1 = \tmthree$ with $\tmtwo_0 \tostratind{m} \tmthree_0$; 
%			since $m < n \leq n_0$, %here it is important to take the min in the for the index application case of the definition of \partostratind{n}
%			by \ih applied to $\tm_0 \partostratind{n_0} \tmtwo_0 \tostratind{m} \tmthree_0$, we have $\tm_0 \partobv \tmthree_0$ and $\tm_0 \tostratind{m} \tmfour_0$ for some term $\tmfour_0$, and so (as $\partostratind{n_1} \,\subseteq\, \partobv$)
%			\begin{align*}
%			\AxiomC{$\tm_0 \partobv \tmthree_0$}
%			\AxiomC{$\tm_1 \partobv \tmtwo_1$}
%			\BinaryInfC{$\tm = \tm_0\tm_1 \partobv \tmthree_0\tmtwo_1 = \tmthree$}
%			\DisplayProof
%			\qquad
%			\text{and}
%			\qquad
%			\AxiomC{$\tm_0 \tostratind{m} \tmfour_0$}
%			\UnaryInfC{$\tm = \tm_0\tm_1 \tostratind{m} \tmfour_0\tm_1 = \tmfour$}
%			\DisplayProof
%			\,;
%			\end{align*}
%			\item $\tmtwo = \tmtwo_0\tmtwo_1 \tostratind{m} \tmthree_0\tmtwo_1 = \tmthree$ with $\tmtwo_1 \tostratind{m-1} \tmthree_1$; 
%			since $m-1 < n-1 \leq n_1$,
%			by \ih applied to $\tm_1 \partostratind{n_1} \tmtwo_1 \tostratind{m-1} \tmthree_1$, we have $\tm_1 \partobv \tmthree_1$ and $\tm_1 \tostratind{m-1} \tmfour_1$ for some term $\tmfour_1$, and so (as $\tm_0 \partostratind{n_0} \,\subseteq\, \partobv$)
%			\begin{align*}
%			\AxiomC{$\tm_0 \partobv \tmtwo_0$}
%			\AxiomC{$\tm_1 \partobv \tmthree_1$}
%			\BinaryInfC{$\tm = \tm_0\tm_1 \partobv \tmtwo_0\tmthree_1 = \tmthree$}
%			\DisplayProof
%			\qquad
%			\text{and}
%			\qquad
%			\AxiomC{$\tm_1 \tostratind{m-1} \tmfour_1$}
%			\UnaryInfC{$\tm = \tm_0\tm_1 \tostratind{m} \tm_0\tmfour_1 = \tmfour$}
%			\DisplayProof
%			\,;
%			\end{align*}		
%%			analogous to the previous sub-case.
%			\item $\tmtwo = (\la{\var}{\tmtwo_0})\tmtwo_1 \tostratind{0} \tmtwo_0\isub{\var}{\tmtwo_1} = \tmthree$ with $m = 0$; 
%			as $n > 0$ then, according to the definition of $\tm \partostratind{n} \tmtwo$,
%				\begin{align*}
%				\AxiomC{$\tm_0 \partostratind{n_0} \tmtwo_0$}
%				\UnaryInfC{$\la{\var}\tm_0 \partostratind{n_0} \la{\var}\tmtwo_0$}
%				\AxiomC{$\tm_1 \partostratind{n_1} \tmtwo_1$}
%				\BinaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \partostratind{n} (\la{\var}{\tmtwo_0})\tmtwo_1 = \tmtwo$}
%				\DisplayProof
%				\end{align*}
%				where $n = \min\{n_0, n_1+1\}$; therefore (as $\partostratind{k} \,\subseteq\, \partobv$)
%				\begin{align*}
%				\AxiomC{$\tm_0 \partobv \tmtwo_0$}
%				\AxiomC{$\tm_1 \partobv \tmtwo_1$}
%				\BinaryInfC{$\tm = (\la{\var}{\tm_0})\tm_1 \partobv \tmtwo_0\isub{\var}{\tmtwo_1} = \tmthree$}
%				\DisplayProof
%				\shortintertext{and}
%				\AxiomC{}
%				\UnaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \tostratind{0} \tm_0\isub{\var}{\tm_1} = \tmfour$}
%				\DisplayProof
%				\,;
%				\end{align*}
%		\end{enumerate}
%	\end{itemize}
	\begin{enumerate}
	\item By induction on the definition of $\tm \partostratind{n} \tmtwo$.
	Cases:
	\begin{itemize}
		\item \emph{Variable}: $\tm = \var \partostratind{\infty} \var = \tmtwo$. 
		Then, there is no $\tmthree$ such that $\tmtwo \tostratind{m} \tmthree$ for any $m \in \nat$.
		
		\item \emph{Abstraction}: $\tm = \la \var\tm' \partostratind{n}  \la \var \tmtwo' = \tmtwo$ because $\tm' \partostratind{n} \tmtwo'$. 
		According to the definition of $\tmtwo \tostratind{m} \tmthree$, by necessity $\tmthree = \la{\var}{\tmthree'}$ with $\tmtwo' \tostratind{m} \tmthree'$.
		By \ih, $\tm' \partobv \tmthree'$, thus 
		\begin{align*}
		\AxiomC{$\tm' \partobv \tmthree'$}
		\UnaryInfC{$\tm = \la{\var}{\tm'} \partobv \la{\var}{\tmthree'} = \tmthree$}
		\DisplayProof
		\,.
		\end{align*}
		
		\item \emph{Application}:
		\begin{align*}
		\AxiomC{$\tm_0 \partostratind{n_0} \tmtwo_0$}	
		\AxiomC{$\tm_1 \partostratind{n_1} \tmtwo_1$}
		\BinaryInfC{$\tm = \tm_0 \tm_1 \partostratind{n} \tmtwo_0 \tmtwo_1 = \tmtwo$}
		\DisplayProof 
		\end{align*}
		where $n = \min\{n_0,n_1+1\}$.
		According to the definition of $\tmtwo \tostratind{m} \tmthree$, there are the following sub-cases:
		\begin{enumerate}
			\item $\tmtwo = \tmtwo_0\tmtwo_1 \tostratind{m} \tmthree_0\tmtwo_1 = \tmthree$ with $\tmtwo_0 \tostratind{m} \tmthree_0$; 
			since $m < n \leq n_0$, %here it is important to take the min in the for the index application case of the definition of \partostratind{n}
			by \ih applied to $\tm_0 \partostratind{n_0} \tmtwo_0 \tostratind{m} \tmthree_0$, we have $\tm_0 \partobv \tmthree_0$, and so (as $\partostratind{n_1} \,\subseteq\, \partobv$)
			\begin{align*}
			\AxiomC{$\tm_0 \partobv \tmthree_0$}
			\AxiomC{$\tm_1 \partobv \tmtwo_1$}
			\BinaryInfC{$\tm = \tm_0\tm_1 \partobv \tmthree_0\tmtwo_1 = \tmthree$}
			\DisplayProof
			\,;
			\end{align*}
			\item $\tmtwo = \tmtwo_0\tmtwo_1 \tostratind{m} \tmthree_0\tmtwo_1 = \tmthree$ with $\tmtwo_1 \tostratind{m-1} \tmthree_1$; 
			since $m-1 < n-1 \leq n_1$,
			by \ih applied to $\tm_1 \partostratind{n_1} \tmtwo_1 \tostratind{m-1} \tmthree_1$, we have $\tm_1 \partobv \tmthree_1$, and so (as $\tm_0 \partostratind{n_0} \,\subseteq\, \partobv$)
			\begin{align*}
			\AxiomC{$\tm_0 \partobv \tmtwo_0$}
			\AxiomC{$\tm_1 \partobv \tmthree_1$}
			\BinaryInfC{$\tm = \tm_0\tm_1 \partobv \tmtwo_0\tmthree_1 = \tmthree$}
			\DisplayProof
			\,;
			\end{align*}		
			%			analogous to the previous sub-case.
			\item $\tmtwo = (\la{\var}{\tmtwo_0})\tmtwo_1 \tostratind{0} \tmtwo_0\isub{\var}{\tmtwo_1} = \tmthree$ with $m = 0$; 
			as $n > 0$ then, according to the definition of $\tm \partostratind{n} \tmtwo$,
			\begin{align*}
			\AxiomC{$\tm_0 \partostratind{n_0} \tmtwo_0$}
			\UnaryInfC{$\la{\var}\tm_0 \partostratind{n_0} \la{\var}\tmtwo_0$}
			\AxiomC{$\tm_1 \partostratind{n_1} \tmtwo_1$}
			\BinaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \partostratind{n} (\la{\var}{\tmtwo_0})\tmtwo_1 = \tmtwo$}
			\DisplayProof
			\end{align*}
			where $n = \min\{n_0, n_1+1\}$; therefore (as $\partostratind{k} \,\subseteq\, \partobv$)
			\begin{align*}
			\AxiomC{$\tm_0 \partobv \tmtwo_0$}
			\AxiomC{$\tm_1 \partobv \tmtwo_1$}
			\BinaryInfC{$\tm = (\la{\var}{\tm_0})\tm_1 \partobv \tmtwo_0\isub{\var}{\tmtwo_1} = \tmthree$}
			\DisplayProof
			\,.
			\end{align*}
		\end{enumerate}
	\end{itemize}

	\item As $\tm \partonotstrat \tmtwo \tostrat \tmthree$, then $\tm \partostratind{n} \tmtwo \tostratind{m} \tmthree$ for some $n \in \nat \cup \{\infty\}$ and $m \in \nat$ such that $n > \Deg{\tm}$ and  $m = \Deg{\tmtwo}$.
	By persistence (\reflemma{perpetuity-strat}),  $\Deg{\tm} \geq \Deg{\tmtwo}$.
	Hence, $n > m$ and we can then merge (by \refpropp{i-e-merge-strat}{ind}) to $\tm \partob \tmthree$.
	\qedhere
	\end{enumerate}
\end{proof}

%\begin{lemma}
%	If $\tm \partob \tmtwo$ then $\tm \partostratind{m} \tmtwo$ for some $m \in \nat \cup \{\infty\}$.
%\end{lemma}
%
%\begin{proof}
%	By hypothesis, $\tm \partobind{n} \tmtwo$ for some $n \in \nat$.
%	The statement by straightforward induction on the definition of $\tm \partobind{n} \tmtwo$. 
%\end{proof}


%\begin{lemma}[Decomposition of parallel $\beta$-steps]
%\label{l:decomp-strat}
%If $\tm \partobind{n} \tmtwo$ with $n > 0$, then there are a term $\tmthree$ and $m \in \nat$ such that $\tm \tostratind{m} \tmthree \partobindlong{n-1} \tmtwo$ and $\tm \partostratind{m} \tmtwo$.	
%\end{lemma}
%
%\begin{proof}
%By induction on the definition of $\tm \partobind{n} \tmtwo$. 
%Cases:
%\begin{itemize}
%	\item \emph{Variable}: $\tm = \var \partobind{0} \var = \tmtwo$.
%	This is impossible because $n > 0$ by hypothesis.
%	
%	\item \emph{Abstraction}: $\tm = \la \var\tm' \partobind{n}  \la \var \tmtwo' = \tmtwo$ because $\tm' \partobind{n} \tmtwo'$. 
%	By \ih,   $\tm' \tostratind{m} \tmthree'$ for some term $\tmthree'$ and some $m \in \nat$ such that $\tmthree' \partobindlong{n-1} \tmtwo'$ and $\tm' \partostratind{m} \tmtwo'$, so 
%	\begin{align*}
%	\AxiomC{$\tm' \tostratind{m} \tmthree'$}
%	\UnaryInfC{$\tm = \la{\var}{\tm'} \tostratind{m} \la{\var}{\tmthree'} = \tmthree$}
%	\DisplayProof&
%	\qquad
%	\text{and}
%	\qquad
%	\AxiomC{$\tmthree' \partobind{n-1} \tmtwo'$}
%	\UnaryInfC{$\tmthree = \la{\var}{\tmthree'} \partobind{n-1} \la{\var}{\tmtwo'} = \tmtwo$}
%	\DisplayProof
%	\shortintertext{and}
%	\AxiomC{$\tm' \partostratind{m} \tmtwo'$}
%	\UnaryInfC{$\tm = \la{\var}{\tm'} \partostratind{m} \la{\var}{\tmtwo'} = \tmtwo$}
%	\DisplayProof
%	\,.
%	\end{align*}
%	
%	\item \emph{Application}:
%	\begin{align*}
%	\AxiomC{$\tm_0 \partobind{n_0} \tmtwo_0$}	
%	\AxiomC{$\tm_1 \partobind{n_1} \tmtwo_1$}
%	\BinaryInfC{$\tm = \tm_0 \tm_1 \partobind{n} \tmtwo_0 \tmtwo_1 = \tmtwo$}
%	\DisplayProof 
%	\end{align*}
%	where $n = n_0 +  n_1$.
%	By \ih, $\tm_0 \tostratind{m_0} \tmthree_0$ and $\tm_1 \tostratind{m_1} \tmthree_1$ for some terms $\tmthree_0, \tmthree_1$ and some $m_0, m_1 \in \nat$ such that $\tmthree_0 \partobindlong{n_0-1} \tmtwo_0$ and $\tmthree_1 \partobindlong{n_1-1} \tmtwo_1$ and $\tm_0 \partostratind{m_0} \tmthree_0$ and $\tm_1 \partostratind{m_1} \tmthree_1$.
%	Therefore,
%	\begin{align*}
%	\AxiomC{$\tm_0 \partostratind{m_0} \tmtwo_0$}
%	\AxiomC{$\tm_1 \partostratind{m_1} \tmtwo_1$}
%	\BinaryInfC{$\tm = \tm_0\tm_1 \partostratind{m} \tmtwo_0\tmtwo_1 = \tmtwo$}
%	\DisplayProof			
%	\end{align*}
%	where $m = \min\{m_0, m_1+1\}$.
%	There are two possibilities:
%	\begin{enumerate}
%		\item $m = m_0$; then 
%		\begin{align*}
%		\AxiomC{$\tm_0 \tostratind{m} \tmthree_0$}
%		\UnaryInfC{$\tm = \tm_0\tm_1 \tostratind{m} \tmthree_0\tm_1 = \tmthree$}
%		\DisplayProof
%		\qquad
%		\text{and}
%		\qquad
%		&
%		\AxiomC{$\tmthree_0 \partobind{n_0-1} \tmtwo_0$}
%		\AxiomC{$\tm_1 \partobind{n_1} \tmtwo_1$}
%		\BinaryInfC{$\tmthree = \tmthree_0\tm_1 \partobind{n-1} \tmtwo_0\tmtwo_1 = \tmtwo$}
%		\DisplayProof		
%		\,;
%		\end{align*}
%	
%		\item $m = m_1+1$; then 
%		\begin{align*}
%		\AxiomC{$\tm_1 \tostratind{m-1} \tmthree_1$}
%		\UnaryInfC{$\tm = \tm_0\tm_1 \tostratind{m} \tm_0\tmthree_1 = \tmthree$}
%		\DisplayProof
%		\qquad
%		\text{and}
%		\qquad
%		\AxiomC{$\tmthree_0 \partobind{n_0} \tmtwo_0$}
%		\AxiomC{$\tm_1 \partobind{n_1-1} \tmtwo_1$}
%		\BinaryInfC{$\tmthree = \tm_0\tmthree_1 \partobind{n-1} \tmtwo_0\tmtwo_1 = \tmtwo$}
%		\DisplayProof
%		\,.
%		\end{align*}
%	\end{enumerate}
%	
%	\item \emph{$\beta$-step}:
%	\begin{align*}
%	\AxiomC{$\tm_0 \partobind{n_0} \tm_0'$}
%	\AxiomC{$\tm_1 \partobind{n_1} \tm_1'$}
%	\BinaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \partobind{n} \tm_0' \isub{\var}{\tm_1'} = \tmtwo$}
%	\DisplayProof
%	\end{align*}
%	where $n = n_0 + \sizep{\tm_0}{\var}n_1 + 1 > 0$.
%	By \ih, $\tm_0 \partostratind{m_0} \tmtwo_0$ and $\tm_1 \partostratind{m_1} \tmtwo_1$ for some $m_0, m_1 \in \nat$.
%	Thus,
%	\begin{align*}
%	\AxiomC{$\tm_0 \partostratind{m_0} \tm_0'$}
%	\AxiomC{$\tm_1 \partostratind{m_1} \tm_1'$}
%	\BinaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \partostratind{0} \tm_0' \isub{\var}{\tm_1'} = \tmtwo$}
%	\DisplayProof
%	\,.
%	\end{align*}	
%	Let $\tmthree = \tm_0\isub{\var}{\tm_1}$.
%	By \reflemma{tob-subs}, $\tmthree = \tm_0\isub{\var}{\tm_1} \partobindlong{n_0 + \sizep{\tm_0}{\var} n_1} \tm_0'\isub{\var}{\tm_1'} = \tmtwo$ where $n_0 + \sizep{\tm_0}{\var} n_1 = n - 1$.
%	Clearly,
%	\begin{align*}
%	\AxiomC{}
%	\UnaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \tostratind{0} \tm_0 \isub{\var}{\tm_1} = \tmthree$}
%	\DisplayProof
%	\,.
%	\end{align*}
%	According to substitutivity (\reflemma{tob-subs}), $\tmthree = \tm_0\isub{\var}{\tm_1} \partostratind{j} \tm_0'\isub{\var}{\tm_1'} = \tmtwo$ for some $j \in \nat \cup \{\infty\}$, in particular $j \geq 0$.
%	\qedhere
%\end{itemize}
%\end{proof}
\begin{lemma}[Decomposition of parallel $\beta$-steps]
\label{l:decomp-strat}
If $\tm \partobind{n} \tmtwo$ then $\tm \partostratind{m} \tmtwo$ for some $m \in \nat \cup \{\infty\}$.
If moreover $n > 0$ then $m \neq \infty$ and $\tm \tostratind{m} \tmthree$ for some term $\tmthree$ such that $\tmthree \partobindlong{n-1} \tmtwo$ and $\tmthree \partostratind{j} \tmtwo$ with $j \geq m	$ (possibly $j = \infty$).	
\end{lemma}

\begin{proof}
By induction $(n,k) \in \nat \times \nat$ with the lexicographical order, where $k$ is the length of the derivation of $\tm \partobind{n} \tmtwo$. 
Cases:
\begin{itemize}
	\item \emph{Variable}: $\tm = \var \partobind{0} \var = \tmtwo$ where $n = 0$. 
	Then,
	\begin{align*}
	\AxiomC{}
	\UnaryInfC{$\tm = \var \partostratind{\infty} \var = \tmtwo$}
	\DisplayProof
	\,.
	\end{align*}
	
	\item \emph{Abstraction}: $\tm = \la \var\tm' \partobind{n}  \la \var \tmtwo' = \tmtwo$ because $\tm' \partobind{n} \tmtwo'$. 
	By \ih, $\tm' \partostratind{m} \tmtwo'$ for some $m \in \nat \cup \{\infty\}$.
	Then,
	\begin{align*}
	\AxiomC{$\tm' \partostratind{m} \tmtwo'$}
	\UnaryInfC{$\tm = \la{\var}{\tmthree'} \partostratind{m} \la{\var}{\tmtwo'} = \tmtwo$}
	\DisplayProof
	\,.
	\end{align*}
	If moreover $n > 0$, then by \ih, $m \neq \infty$ and $\tm' \tostratind{m} \tmthree'$ for some term $\tmthree'$ such that $\tmthree' \partobindlong{n-1} \tmtwo'$ and $\tmthree' \partostratind{j} \tmtwo'$ with $j \geq m$ (possibly $j = \infty$), so 
	\begin{align*}
	\AxiomC{$\tm' \tostratind{m} \tmthree'$}
	\UnaryInfC{$\tm = \la{\var}{\tm'} \tostratind{m} \la{\var}{\tmthree'} = \tmthree$}
	\DisplayProof
	\qquad
	\text{and}
	\qquad
	&
	\AxiomC{$\tmthree' \partostratind{j} \tmtwo'$}
	\UnaryInfC{$\tmthree = \la{\var}{\tmthree'} \partostratind{j} \la{\var}{\tmtwo'} = \tmtwo$}
	\DisplayProof
	\shortintertext{and}
	\AxiomC{$\tmthree' \partobind{n-1} \tmtwo'$}
	\UnaryInfC{$\tmthree = \la{\var}{\tmthree'} \partobind{n-1} \la{\var}{\tmtwo'} = \tmtwo$}
	\DisplayProof
	\,.
	\end{align*}
	
	\item \emph{Application}:
	\begin{align*}
	\AxiomC{$\tm_0 \partobind{n_0} \tmtwo_0$}	
	\AxiomC{$\tm_1 \partobind{n_1} \tmtwo_1$}
	\BinaryInfC{$\tm = \tm_0 \tm_1 \partobind{n} \tmtwo_0 \tmtwo_1 = \tmtwo$}
	\DisplayProof 
	\end{align*}
	where $n = n_0 + n_1$.
	By \ih, $\tm_0 \partostratind{m_0} \tmtwo_0$ and $\tm_1 \partostratind{m_1} \tmtwo_1$ for some $m_0, m_1 \in \nat \cup \{\infty\}$.
	Thus,
	\begin{align*}
	\AxiomC{$\tm_0 \partostratind{m_0} \tmtwo_0$}	
	\AxiomC{$\tm_1 \partostratind{m_1} \tmtwo_1$}
	\BinaryInfC{$\tm = \tm_0 \tm_1 \partostratind{m} \tmtwo_0 \tmtwo_1 = \tmtwo$}
	\DisplayProof 
	\end{align*}
	where $m = \min\{m_0,m_1+1\}$.
	If moreover $n > 0$, then by \ih, $m_0, m_1 \neq \infty$ and $\tm_0 \tostratind{m_0} \tmthree_0$ and $\tm_1 \tostratind{n_1} \tmthree_1$ for some terms $\tmthree_0, \tmthree_1$ such that $\tmthree_0 \partobindlong{n_0-1} \tmtwo_0$ and $\tmthree_1 \partobindlong{n_1-1} \tmtwo_1$ and $\tmthree_0 \partostratind{j_0} \tmtwo_0$ and $\tmthree_1 \partostratind{j_1} \tmtwo_1$ with $j_0 \geq m_0$, $j_1 \geq m_1$ (possibly $j_0,j_1 = \infty$).
	There are two possibilities:
	\begin{enumerate}
		\item $m = m_0$; then, $m_0 \leq m_1+1$ and 
		\begin{align*}
		\AxiomC{$\tm_0 \tostratind{m} \tmthree_0$}
		\UnaryInfC{$\tm = \tm_0\tm_1 \tostratind{m} \tmthree_0\tm_1 = \tmthree$}
		\DisplayProof
		\qquad
		\text{and}
		\qquad
		&
		\AxiomC{$\tmthree_0 \partobind{n_0-1} \tmtwo_0$}
		\AxiomC{$\tm_1 \partobind{n_1} \tmtwo_1$}
		\BinaryInfC{$\tmthree = \tmthree_0\tm_1 \partobind{n-1} \tmtwo_0\tmtwo_1 = \tmtwo$}
		\DisplayProof		
		\shortintertext{and}
		\AxiomC{$\tmthree_0 \partostratind{j_0} \tmtwo_0$}
		\AxiomC{$\tm_1 \partostratind{m_1} \tmtwo_1$}
		\BinaryInfC{$\tmthree = \tmthree_0\tm_1 \partostratind{j} \tmtwo_0\tmtwo_1 = \tmtwo$}
		\DisplayProof
		\end{align*}
		where $j = \min\{j_0, m_1+1\} \geq m_0 = m$; 
		\item $m = m_1+1$; then, $m_1 + 1 \leq m_0$ and  
		\begin{align*}
		\AxiomC{$\tm_1 \tostratind{m-1} \tmthree_1$}
		\UnaryInfC{$\tm = \tm_0\tm_1 \tostratind{m} \tm_0\tmthree_1 = \tmthree$}
		\DisplayProof
		\qquad
		\text{and}
		\qquad
		&
		\AxiomC{$\tmthree_0 \partobind{n_0} \tmtwo_0$}
		\AxiomC{$\tm_1 \partobind{n_1-1} \tmtwo_1$}
		\BinaryInfC{$\tmthree = \tm_0\tmthree_1 \partobind{n-1} \tmtwo_0\tmtwo_1 = \tmtwo$}
		\DisplayProof
		\shortintertext{and}
		\AxiomC{$\tmthree_0 \partostratind{m_0} \tmtwo_0$}
		\AxiomC{$\tm_1 \partostratind{j_1} \tmtwo_1$}
		\BinaryInfC{$\tmthree = \tm_0\tmthree_1 \partostratind{j} \tmtwo_0\tmtwo_1 = \tmtwo$}
		\DisplayProof
		\end{align*}
		where $j = \min\{m_0, j_1+1\} \geq m_1+1 = m$.
	\end{enumerate}
	
	\item \emph{$\beta$-step}:
	\begin{align*}
	\AxiomC{$\tm_0 \partobind{n_0} \tm_0'$}
	\AxiomC{$\tm_1 \partobind{n_1} \tm_1'$}
	\BinaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \partobind{n} \tm_0' \isub{\var}{\tm_1'} = \tmtwo$}
	\DisplayProof
	\end{align*}
	where $n = n_0 + \sizep{\tm_0}{\var}n_1 + 1 > 0$.
	By \ih, $\tm_0 \partostratind{m_0} \tmtwo_0$ and $\tm_1 \partostratind{m_1} \tmtwo_1$ for some $m_0, m_1 \in \nat$.
	Thus,
	\begin{align*}
	\AxiomC{$\tm_0 \partostratind{m_0} \tm_0'$}
	\AxiomC{$\tm_1 \partostratind{m_1} \tm_1'$}
	\BinaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \partostratind{0} \tm_0' \isub{\var}{\tm_1'} = \tmtwo$}
	\DisplayProof
	\,.
	\end{align*}	
	Let $\tmthree = \tm_0\isub{\var}{\tm_1}$.
	By \reflemma{partobind-subs}, $\tmthree = \tm_0\isub{\var}{\tm_1} \partobindlong{n_0 + \sizep{\tm_0}{\var} n_1} \tm_0'\isub{\var}{\tm_1'} = \tmtwo$ where $n_0 + \sizep{\tm_0}{\var} n_1 = n - 1$.
	Clearly,
	\begin{align*}
	\AxiomC{}
	\UnaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \tostratind{0} \tm_0 \isub{\var}{\tm_1} = \tmthree$}
	\DisplayProof
	\,.
	\end{align*}
	By \ih (since $n_0 + \sizep{\tm_0}{\var} n_1 = n -1$), $\tmthree = \tm_0\isub{\var}{\tm_1} \partostratind{j} \tm_0'\isub{\var}{\tm_1'} = \tmtwo$ for some $j \in \nat \cup \{\infty\}$, in particular $j \geq 0$.
	\qedhere
\end{itemize}
\end{proof}

%\setcounter{propositionAppendix}{\value{prop:quant-out-in-split-strat}}
\begin{propositionAppendix}[Stratified indexed split]
	\label{propappendix:quant-out-in-split-strat}
	\NoteState{prop:quant-out-in-split-strat}
	If $\tm \partobind n \tmtwo$ then either $\tm \partonotstrat\tmtwo$ or $n>0$ and there exists $\tmthree$ such that $\tm \tostrat \tmthree \partobindlong {n-1} \tmtwo$.
\end{propositionAppendix}

\begin{proof}
	If $n = 0$, then $\tm = \tmtwo$ (because $\partobind{0}$ is the identity relation) and so $\tm \partostratind{\infty} \tmtwo$ (because $\partostratind{\infty}$ is the identity relation), hence $\tm \partonotstrat \tmtwo$. %It requires that $\partonotstrat$ contains the infinite index and that $\partobind{0}$ is the identity relation (not only reflexive).
	
	Otherwise $n > 0$ and then, by \reflemma{decomp-strat}, $\tm \partostratind{k} \tmtwo$ and $\tm \tostratind{k} \tmthree$ for some $k \in \nat$ and some term $\tmthree$ such that $\tmthree \partobind{n-1} \tmtwo$.
	There are two cases:
	\begin{enumerate}
		\item either $k > \Deg{\tm}$ and then $\tm \partonotstrat \tmtwo$ (since $\tm \partostratind{k} \tmtwo$);
		\item or $k = \Deg{\tm}$  and so $\tm \tostrat \tmthree \partobindlong{n-1} \tmtwo$.
		\qedhere
	\end{enumerate}
\end{proof}

%\setcounter{corollaryAppendix}{\value{coro:e-i-split-strat}}
\begin{corollaryAppendix}[Stratified split]
	\label{coroappendix:e-i-split-strat}
	\NoteState{coro:e-i-split-strat}
	If $\tm \partob \tmtwo$ then $\tm \tostrat^* \tmthree \partonotstrat \tmtwo$ for some $\tmthree$.
\end{corollaryAppendix}

%\begin{proof}
%	By hypothesis, $\tm \partobind{n} \tmtwo$ for some $n \in \nat$.
%	We prove the statement by induction on $n \in \nat$.
%	
%	According to the indexed splitting (\refprop{quant-out-in-split-strat}), there are two cases:
%	\begin{itemize}
%		\item either $\tm \partonotstrat \tmtwo$ and we can then conclude taking $\tmthree = \tm$ (in particular, this is the case for $n = 0$, because $\partobind{0}$ is the identity relation);
%		\item or $n > 0$  and $\tm \tostrat \tmfour \partobind{n-1} \tmtwo$; 
%		by \ih applied to $\tmfour \partobind{n-1} \tmtwo$, there is a term $\tmthree$ such that $\tmfour \tostrat^* \tmthree \partonotstrat \tmtwo$;
%		therefore, $\tm \tostrat \tmfour \tostrat^* \tmthree \partonotstrat \tmtwo$.
%		\qedhere
%	\end{itemize}
%\end{proof}
\begin{proof}
	By hypothesis, $\tm \partobind{n} \tmtwo$ for some $n \in \nat$.
	We prove the statement by induction on $n \in \nat$.
	
	If $n = 0$, then $\tm = \tmtwo$ (because $\partobind{0}$ is the identity relation) and so $\tm \partostratind{\infty} \tmtwo$ (because $\partostratind{\infty}$ is the identity relation), hence $\tm \partonotstrat \tmtwo$.
	
	Otherwise $n > 0$ and then, by \reflemma{decomp-strat}, $\tm \partostratind{k} \tmtwo$ and $\tm \tostratind{k} \tmthree$ for some $k \in \nat$ and some term $\tmthree$ such that $\tmthree \partobind{n-1} \tmtwo$.
	There are two cases:
	\begin{enumerate}
		\item either $k > \Deg{\tm}$ and then $\tm \partonotstrat \tmtwo$ (as $\tm \partostratind{k} \tmtwo$), so we conclude taking $\tmthree = \tm$;
		\item or $k = \Deg{\tm}$  and then $\tm \tostrat \tmfour \partobindlong{n-1} \tmtwo$;
		by \ih applied to $\tmfour \partobind{n-1} \tmtwo$, there is a term $\tmthree$ such that $\tmfour \tostrat^* \tmthree \partonotstrat \tmtwo$;
		therefore, $\tm \tostrat \tmfour \tostrat^* \tmthree \partonotstrat \tmtwo$.
		\qedhere
	\end{enumerate}
\end{proof}

Note that the last proof uses only \reflemma{decomp-strat}, not \refprop{quant-out-in-split-strat}!


==> proofs/proofs-stratified-cbn.tex <==
% !TEX root = ../main.tex
\subsection{Omitted proofs and lemmas of \refsect{stratified-cbn}}

\begin{lemma}[Persistence]
\label{l:perpetuity-strat}
	If $\tm \partostratind{n} \tmtwo$ and $\tm \tostratind{m} \tmthree$ with $m < n$, then there exists a term $\tmfour$ such that $\tmtwo \tostratind{m} \tmfour$. 
\end{lemma}

\begin{proof}
	By induction on the definition of $\tm \partostratind{n} \tmtwo$.
	Cases:
	\begin{itemize}
		\item \emph{Variable}: $\tm = \var \partostratind{\infty} \var = \tmtwo$. 
		This is impossible because there is no $\tmthree$ such that $\tm \tostratind{m} \tmthree$ for any $m \in \nat$.
		
		\item \emph{Abstraction}: $\tm = \la \var\tm' \partostratind{n}  \la \var \tmtwo' = \tmtwo$ because $\tm' \partostratind{n} \tmtwo'$.
		By definition of $\tm \tostratind{m} \tmthree$, by necessity $\tmthree = \la{\var}\tmthree'$ with $\tm' \tostratind{m} \tmthree'$
		By \ih, $\tmtwo' \tostratind{m} \tmfour'$ for some term $\tmfour'$.
		Therefore, 
		\begin{align*}
		\AxiomC{$\tmtwo' \tostratind{m} \tmfour'$}
		\UnaryInfC{$\tmtwo = \la{\var}{\tmtwo'} \tostratind{m} \la{\var}{\tmfour'} = \tmfour$}
		\DisplayProof
		\,.
		\end{align*}
		
		\item \emph{Application}:
		\begin{align*}
		\AxiomC{$\tm_0 \partostratind{n_0} \tmtwo_0$}	
		\AxiomC{$\tm_1 \partostratind{n_1} \tmtwo_1$}
		\BinaryInfC{$\tm = \tm_0 \tm_1 \partostratind{n} \tmtwo_0 \tmtwo_1 = \tmtwo$}
		\DisplayProof 
		\end{align*}
		where $n = \min\{n_0,n_1+1\}$.
		According to the definition of $\tm \tostratind{m} \tmthree$, there are the following sub-cases:
		\begin{enumerate}
			\item $\tm = \tm_0\tm_1 \tostratind{m} \tmthree_0\tm_1 = \tmthree$ with $\tm_0 \tostratind{m} \tmthree_0$; 
			since $m < n \leq n_0$, %here it is important to take the min in the for the index application case of the definition of \partostratind{n}
			by \ih applied to $\tm_0$, we have $\tmtwo_0 \tostratind{m} \tmfour_0$  for some term $\tmfour_0$, and so 
			\begin{align*}
			\AxiomC{$\tmtwo_0 \tostratind{m} \tmfour_0$}
			\UnaryInfC{$\tmtwo = \tmtwo_0\tmtwo_1 \tostratind{m} \tmfour_0\tmtwo_1 = \tmfour$}
			\DisplayProof
			\,;
			\end{align*}
			\item $\tm = \tm_0\tm_1 \tostratind{m} \tm_0\tmthree_1 = \tmthree$ with $\tm_1 \tostratind{m-1} \tmthree_1$; 
			since $m-1 < n-1 \leq n_1$,
			by \ih applied to $\tm_1$, we have $\tmtwo_1 \tostratind{m} \tmfour_1$ for some term $\tmfour_1$, and so 
			\begin{align*}
			\AxiomC{$\tmtwo_1 \tostratind{m-1} \tmfour_1$}
			\UnaryInfC{$\tmtwo = \tmtwo_0\tmtwo_1 \tostratind{m} \tmtwo_0\tmfour_1 = \tmfour$}
			\DisplayProof
			\,;
			\end{align*}		
			%			analogous to the previous sub-case.
			
			\item $\tm = (\la{\var}{\tm_0})\tm_1 \tostratind{0} \tm_0\isub{\var}{\tm_1} = \tmthree$ with $m = 0 < n$. 
			According to the definition of $\tm \partostratind{n} \tmtwo$,
				\begin{align*}
				\AxiomC{$\tm_0 \partostratind{n_0} \tmtwo_0$}
				\UnaryInfC{$\la{\var}\tm_0 \partostratind{n_0} \la{\var}\tmtwo_0$}
				\AxiomC{$\tm_1 \partostratind{n_1} \tmtwo_1$}
				\BinaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \partostratind{n} (\la{\var}{\tmtwo_0})\tmtwo_1 = \tmtwo$}
				\DisplayProof
				\end{align*}
				where $n = \min\{n_0, n_1+1\}$; therefore
				\begin{align*}
				\AxiomC{}
				\UnaryInfC{$\tmtwo = (\la{\var}\tmtwo_0)\tmtwo_1 \tostratind{0} \tmtwo_0\isub{\var}{\tmtwo_1} = \tmfour$}
				\DisplayProof
				\,.
				\end{align*}
		\end{enumerate}
		
		\item \emph{$\beta$-step}: 
		\begin{align*}
		\AxiomC{}
		\UnaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \partostratind{0} \tm_0 \isub{\var}{\tm_1} = \tmtwo$}
		\DisplayProof
		\end{align*}
		where $n = 0$. This is impossible because there is no term $\tmthree$ such that $\tm \tostratind{m} \tmthree$ with $ m < 0$.
		\qedhere
	\end{itemize}
\end{proof}

%\begin{lemma}[Decomposition of parallel $n$-depth $\beta$-steps]
%	\label{l:decomp-strat}
%%	Let $\tm \partostratind{n} \tmtwo$ with $n \neq \infty$.
%%	\begin{enumerate}
%%		\item \label{p:decomp-strat-ind} Then, $\tm \tostratind{n} \tmthree \partostratind{j} \tmtwo$ for some term $\tmthree$ and some $j \geq n$ (possibly $j = \infty$).	
%%		
%%		\item\label{p:decomp-strat-notstrat} If moreover $\tm \partonotstrat \tmtwo$, then $n > 0 $ and $\tm \tostratind{k} \tmfour$ for some $\tmfour$ and some $k < n$.
%%	\end{enumerate}
%	If $\tm \partostratind{n} \tmtwo$ with $n \neq \infty$, then $\tm \tostratind{n} \tmthree \partostratind{j} \tmtwo$ for some term $\tmthree$ and some $j \geq n$ (possibly $j = \infty$).	
%\end{lemma}
%
%\begin{proof}
%	By induction on the definition of $\tm \partostratind{n} \tmtwo$. 
%		Cases:
%		\begin{itemize}
%			\item \emph{Variable}: $\tm = \var \partostratind{\infty} \var = \tmtwo$. 
%			This is impossible because $n \neq \infty$ by hypothesis.
%			
%			\item \emph{Abstraction}: $\tm = \la \var\tm' \partostratind{n}  \la \var \tmtwo' = \tmtwo$ because $\tm' \partostratind{n} \tmtwo'$. 
%			By \ih, $\tm' \tostratind{n} \tmthree' \partostratind{j} \tmtwo'$ for some term $\tmthree'$ and some $j \geq n$ (possibly $j = \infty$), so 
%			\begin{align*}
%			\AxiomC{$\tm' \tostratind{n} \tmthree'$}
%			\UnaryInfC{$\tm = \la{\var}{\tm'} \tostratind{n} \la{\var}{\tmthree'} = \tmthree$}
%			\DisplayProof
%			\qquad
%			\text{and}
%			\qquad
%			\AxiomC{$\tmthree' \partostratind{j} \tmtwo'$}
%			\UnaryInfC{$\tmthree = \la{\var}{\tmthree'} \partostratind{j} \la{\var}{\tmtwo'} = \tmtwo$}
%			\DisplayProof\,.
%			\end{align*}
%			
%			\item \emph{Application}:
%			\begin{align*}
%			\AxiomC{$\tm_0 \partostratind{n_0} \tmtwo_0$}	
%			\AxiomC{$\tm_1 \partostratind{n_1} \tmtwo_1$}
%			\BinaryInfC{$\tm = \tm_0 \tm_1 \partostratind{n} \tmtwo_0 \tmtwo_1 = \tmtwo$}
%			\DisplayProof 
%			\end{align*}
%			where $n = \min\{n_0,n_1+1\}$.
%			By \ih, $\tm_0 \tostratind{n_0} \tmthree_0 \partostratind{j_0} \tmthree_0$ and $\tm_1 \tostratind{n_1} \tmthree_1 \partostratind{j_1} \tmthree_1$ for some terms $\tmthree_0, \tmthree_1$ and some $j_0 \geq n_0$, $j_1 \geq n_1$ (possibly $j_0,j_1 = \infty$).
%			There are two possibilities:
%			\begin{enumerate}
%				\item $n = n_0$; then, $n_0 \leq n_1+1$ and 
%				\begin{align*}
%				\AxiomC{$\tm_0 \tostratind{n} \tmthree_0$}
%				\UnaryInfC{$\tm = \tm_0\tm_1 \tostratind{n} \tmthree_0\tm_1 = \tmthree$}
%				\DisplayProof
%				\qquad
%				\text{and}
%				\qquad
%				\AxiomC{$\tmthree_0 \partostratind{j_0} \tmtwo_0$}
%				\AxiomC{$\tm_1 \partostratind{n_1} \tmtwo_1$}
%				\BinaryInfC{$\tmthree = \tmthree_0\tm_1 \partostratind{j} \tmtwo_0\tmtwo_1 = \tmtwo$}
%				\DisplayProof
%				\end{align*}
%				where $j = \min\{j_0, n_1+1\} \geq n_0 = n$; 
%				\item $n = n_1+1$; then, $n_1 + 1 \leq n_0$ and  
%				\begin{align*}
%					\AxiomC{$\tm_1 \tostratind{n} \tmthree_1$}
%					\UnaryInfC{$\tm = \tm_0\tm_1 \tostratind{n} \tm_0\tmthree_1 = \tmthree$}
%					\DisplayProof
%					\qquad
%					\text{and}
%					\qquad
%					\AxiomC{$\tmthree_0 \partostratind{n_0} \tmtwo_0$}
%					\AxiomC{$\tm_1 \partostratind{j_1} \tmtwo_1$}
%					\BinaryInfC{$\tmthree = \tm_0\tmthree_1 \partostratind{j} \tmtwo_0\tmtwo_1 = \tmtwo$}
%					\DisplayProof
%				\end{align*}
%				where $j = \min\{n_0, j_1+1\} \geq n_1+1 = n$.
%			\end{enumerate}
%		
%			\item \emph{$\beta$-step}: 
%			\begin{align*}
%				\AxiomC{}
%				\UnaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \partostratind{0} \tm_0 \isub{\var}{\tm_1} = \tmtwo$}
%				\DisplayProof
%			\end{align*}
%			Let $\tmthree = \tmtwo$: then $\tmthree \partostratind{\infty} \tmtwo$ and
%			\begin{align*}
%				\AxiomC{}
%				\UnaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \tostratind{0} \tm_0 \isub{\var}{\tm_1} = \tmthree$}
%				\DisplayProof\,.
%			\end{align*}
%			\qedhere
%		\end{itemize}
%\end{proof}


\setcounter{propositionAppendix}{\value{prop:i-e-merge-strat}}
\begin{propositionAppendix}[Internal-external merge]
	\label{propappendix:i-e-merge-strat}
	\NoteState{prop:i-e-merge-strat}
	\begin{enumerate}
		\item If $\tm \partostratind{n}\tmtwo \tostratind{m} \tmthree$ with $n > m$, then $\tm \partob \tmthree$. %and $\tm \tostratind{m} \tmfour$ for some term $\tmfour$.
		\item If $\tm \partonotstrat \tmtwo \tostrat \tmthree$, then $\tm \partob \tmthree$.
	\end{enumerate}
\end{propositionAppendix}

\begin{proof}\hfill
%	\begin{enumerate}
%		\item By induction on the definition of $\tm \partostratind{n} \tmtwo$.
%	Cases:
%		\begin{itemize}
%		\item \emph{Variable}: $\tm = \var \partostratind{\infty} \var = \tmtwo$. 
%		Then, there is no $\tmthree$ such that $\tmtwo \tostratind{m} \tmthree$ for any $m \in \nat$.
%		
%		\item \emph{Abstraction}: $\tm = \la \var\tm' \partostratind{n}  \la \var \tmtwo' = \tmtwo$ because $\tm' \partostratind{n} \tmtwo'$. 
%		According to the definition of $\tmtwo \tostratind{m} \tmthree$, by necessity $\tmthree = \la{\var}{\tmthree'}$ with $\tmtwo' \tostratind{m} \tmthree'$.
%		By \ih, $\tm' \partobv \tmthree'$ and $\tm' \tostratind{m} \tmfour'$ for some term $\tmfour'$, thus 
%		\begin{align*}
%			\AxiomC{$\tm' \partobv \tmthree'$}
%			\UnaryInfC{$\tm = \la{\var}{\tm'} \partobv \la{\var}{\tmthree'} = \tmthree$}
%			\DisplayProof
%			\qquad
%			\text{and}
%			\qquad
%			\AxiomC{$\tm' \tostratind{m} \tmfour'$}
%			\UnaryInfC{$\tm = \la{\var}{\tm'} \tostratind{m} \la{\var}{\tmfour'} = \tmfour$}
%			\DisplayProof\,.
%		\end{align*}
%		
%		\item \emph{Application}:
%		\begin{align*}
%			\AxiomC{$\tm_0 \partostratind{n_0} \tmtwo_0$}	
%			\AxiomC{$\tm_1 \partostratind{n_1} \tmtwo_1$}
%			\BinaryInfC{$\tm = \tm_0 \tm_1 \partostratind{n} \tmtwo_0 \tmtwo_1 = \tmtwo$}
%			\DisplayProof 
%		\end{align*}
%		where $n = \min\{n_0,n_1+1\}$.
%		According to the definition of $\tmtwo \tostratind{m} \tmthree$, there are the following sub-cases:
%		\begin{enumerate}
%			\item $\tmtwo = \tmtwo_0\tmtwo_1 \tostratind{m} \tmthree_0\tmtwo_1 = \tmthree$ with $\tmtwo_0 \tostratind{m} \tmthree_0$; 
%			since $m < n \leq n_0$, %here it is important to take the min in the for the index application case of the definition of \partostratind{n}
%			by \ih applied to $\tm_0 \partostratind{n_0} \tmtwo_0 \tostratind{m} \tmthree_0$, we have $\tm_0 \partobv \tmthree_0$ and $\tm_0 \tostratind{m} \tmfour_0$ for some term $\tmfour_0$, and so (as $\partostratind{n_1} \,\subseteq\, \partobv$)
%			\begin{align*}
%			\AxiomC{$\tm_0 \partobv \tmthree_0$}
%			\AxiomC{$\tm_1 \partobv \tmtwo_1$}
%			\BinaryInfC{$\tm = \tm_0\tm_1 \partobv \tmthree_0\tmtwo_1 = \tmthree$}
%			\DisplayProof
%			\qquad
%			\text{and}
%			\qquad
%			\AxiomC{$\tm_0 \tostratind{m} \tmfour_0$}
%			\UnaryInfC{$\tm = \tm_0\tm_1 \tostratind{m} \tmfour_0\tm_1 = \tmfour$}
%			\DisplayProof
%			\,;
%			\end{align*}
%			\item $\tmtwo = \tmtwo_0\tmtwo_1 \tostratind{m} \tmthree_0\tmtwo_1 = \tmthree$ with $\tmtwo_1 \tostratind{m-1} \tmthree_1$; 
%			since $m-1 < n-1 \leq n_1$,
%			by \ih applied to $\tm_1 \partostratind{n_1} \tmtwo_1 \tostratind{m-1} \tmthree_1$, we have $\tm_1 \partobv \tmthree_1$ and $\tm_1 \tostratind{m-1} \tmfour_1$ for some term $\tmfour_1$, and so (as $\tm_0 \partostratind{n_0} \,\subseteq\, \partobv$)
%			\begin{align*}
%			\AxiomC{$\tm_0 \partobv \tmtwo_0$}
%			\AxiomC{$\tm_1 \partobv \tmthree_1$}
%			\BinaryInfC{$\tm = \tm_0\tm_1 \partobv \tmtwo_0\tmthree_1 = \tmthree$}
%			\DisplayProof
%			\qquad
%			\text{and}
%			\qquad
%			\AxiomC{$\tm_1 \tostratind{m-1} \tmfour_1$}
%			\UnaryInfC{$\tm = \tm_0\tm_1 \tostratind{m} \tm_0\tmfour_1 = \tmfour$}
%			\DisplayProof
%			\,;
%			\end{align*}		
%%			analogous to the previous sub-case.
%			\item $\tmtwo = (\la{\var}{\tmtwo_0})\tmtwo_1 \tostratind{0} \tmtwo_0\isub{\var}{\tmtwo_1} = \tmthree$ with $m = 0$; 
%			as $n > 0$ then, according to the definition of $\tm \partostratind{n} \tmtwo$,
%				\begin{align*}
%				\AxiomC{$\tm_0 \partostratind{n_0} \tmtwo_0$}
%				\UnaryInfC{$\la{\var}\tm_0 \partostratind{n_0} \la{\var}\tmtwo_0$}
%				\AxiomC{$\tm_1 \partostratind{n_1} \tmtwo_1$}
%				\BinaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \partostratind{n} (\la{\var}{\tmtwo_0})\tmtwo_1 = \tmtwo$}
%				\DisplayProof
%				\end{align*}
%				where $n = \min\{n_0, n_1+1\}$; therefore (as $\partostratind{k} \,\subseteq\, \partobv$)
%				\begin{align*}
%				\AxiomC{$\tm_0 \partobv \tmtwo_0$}
%				\AxiomC{$\tm_1 \partobv \tmtwo_1$}
%				\BinaryInfC{$\tm = (\la{\var}{\tm_0})\tm_1 \partobv \tmtwo_0\isub{\var}{\tmtwo_1} = \tmthree$}
%				\DisplayProof
%				\shortintertext{and}
%				\AxiomC{}
%				\UnaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \tostratind{0} \tm_0\isub{\var}{\tm_1} = \tmfour$}
%				\DisplayProof
%				\,;
%				\end{align*}
%		\end{enumerate}
%	\end{itemize}
	\begin{enumerate}
	\item By induction on the definition of $\tm \partostratind{n} \tmtwo$.
	Cases:
	\begin{itemize}
		\item \emph{Variable}: $\tm = \var \partostratind{\infty} \var = \tmtwo$. 
		Then, there is no $\tmthree$ such that $\tmtwo \tostratind{m} \tmthree$ for any $m \in \nat$.
		
		\item \emph{Abstraction}: $\tm = \la \var\tm' \partostratind{n}  \la \var \tmtwo' = \tmtwo$ because $\tm' \partostratind{n} \tmtwo'$. 
		According to the definition of $\tmtwo \tostratind{m} \tmthree$, by necessity $\tmthree = \la{\var}{\tmthree'}$ with $\tmtwo' \tostratind{m} \tmthree'$.
		By \ih, $\tm' \partobv \tmthree'$, thus 
		\begin{align*}
		\AxiomC{$\tm' \partobv \tmthree'$}
		\UnaryInfC{$\tm = \la{\var}{\tm'} \partobv \la{\var}{\tmthree'} = \tmthree$}
		\DisplayProof
		\,.
		\end{align*}
		
		\item \emph{Application}:
		\begin{align*}
		\AxiomC{$\tm_0 \partostratind{n_0} \tmtwo_0$}	
		\AxiomC{$\tm_1 \partostratind{n_1} \tmtwo_1$}
		\BinaryInfC{$\tm = \tm_0 \tm_1 \partostratind{n} \tmtwo_0 \tmtwo_1 = \tmtwo$}
		\DisplayProof 
		\end{align*}
		where $n = \min\{n_0,n_1+1\}$.
		According to the definition of $\tmtwo \tostratind{m} \tmthree$, there are the following sub-cases:
		\begin{enumerate}
			\item $\tmtwo = \tmtwo_0\tmtwo_1 \tostratind{m} \tmthree_0\tmtwo_1 = \tmthree$ with $\tmtwo_0 \tostratind{m} \tmthree_0$; 
			since $m < n \leq n_0$, %here it is important to take the min in the for the index application case of the definition of \partostratind{n}
			by \ih applied to $\tm_0 \partostratind{n_0} \tmtwo_0 \tostratind{m} \tmthree_0$, we have $\tm_0 \partobv \tmthree_0$, and so (as $\partostratind{n_1} \,\subseteq\, \partobv$)
			\begin{align*}
			\AxiomC{$\tm_0 \partobv \tmthree_0$}
			\AxiomC{$\tm_1 \partobv \tmtwo_1$}
			\BinaryInfC{$\tm = \tm_0\tm_1 \partobv \tmthree_0\tmtwo_1 = \tmthree$}
			\DisplayProof
			\,;
			\end{align*}
			\item $\tmtwo = \tmtwo_0\tmtwo_1 \tostratind{m} \tmthree_0\tmtwo_1 = \tmthree$ with $\tmtwo_1 \tostratind{m-1} \tmthree_1$; 
			since $m-1 < n-1 \leq n_1$,
			by \ih applied to $\tm_1 \partostratind{n_1} \tmtwo_1 \tostratind{m-1} \tmthree_1$, we have $\tm_1 \partobv \tmthree_1$, and so (as $\tm_0 \partostratind{n_0} \,\subseteq\, \partobv$)
			\begin{align*}
			\AxiomC{$\tm_0 \partobv \tmtwo_0$}
			\AxiomC{$\tm_1 \partobv \tmthree_1$}
			\BinaryInfC{$\tm = \tm_0\tm_1 \partobv \tmtwo_0\tmthree_1 = \tmthree$}
			\DisplayProof
			\,;
			\end{align*}		
			%			analogous to the previous sub-case.
			\item $\tmtwo = (\la{\var}{\tmtwo_0})\tmtwo_1 \tostratind{0} \tmtwo_0\isub{\var}{\tmtwo_1} = \tmthree$ with $m = 0$; 
			as $n > 0$ then, according to the definition of $\tm \partostratind{n} \tmtwo$,
			\begin{align*}
			\AxiomC{$\tm_0 \partostratind{n_0} \tmtwo_0$}
			\UnaryInfC{$\la{\var}\tm_0 \partostratind{n_0} \la{\var}\tmtwo_0$}
			\AxiomC{$\tm_1 \partostratind{n_1} \tmtwo_1$}
			\BinaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \partostratind{n} (\la{\var}{\tmtwo_0})\tmtwo_1 = \tmtwo$}
			\DisplayProof
			\end{align*}
			where $n = \min\{n_0, n_1+1\}$; therefore (as $\partostratind{k} \,\subseteq\, \partobv$)
			\begin{align*}
			\AxiomC{$\tm_0 \partobv \tmtwo_0$}
			\AxiomC{$\tm_1 \partobv \tmtwo_1$}
			\BinaryInfC{$\tm = (\la{\var}{\tm_0})\tm_1 \partobv \tmtwo_0\isub{\var}{\tmtwo_1} = \tmthree$}
			\DisplayProof
			\,.
			\end{align*}
		\end{enumerate}
	\end{itemize}

	\item As $\tm \partonotstrat \tmtwo \tostrat \tmthree$, then $\tm \partostratind{n} \tmtwo \tostratind{m} \tmthree$ for some $n \in \nat \cup \{\infty\}$ and $m \in \nat$, where (by definition of $\tostrat$) $m$ is minimal for $\tmtwo$, \ie if $\tmtwo \tostratind{m'} \tmthree'$ then $m'\geq m$, and (by definition of $\tm \partonotstrat \tmtwo$), $\tm \tostratind{k} \tmfour$ for term $\tmfour$ and some $k < n$.
	By perpetuity (\reflemma{perpetuity-strat}) there exists a term $\tmfour'$ such that $\tmtwo \tostratind{k} \tmfour'$, and $k \geq m$ by minimality of $m$.
	Hence, $n > m$ and we can then merge (by \refpropp{i-e-merge-strat}{ind}) to $\tm \partob \tmthree$.
	\qedhere
	\end{enumerate}
\end{proof}

\begin{lemma}[Substitutivity of $\partostratind{}$]
	\label{l:tostrat-subs} % \reflemmap{tob-subs}{ind-par}
	If $\tm \partostratind{n} \tm'$ and $\tmtwo \partostratind{m} \tmtwo'$ with $n,m \in \nat \cup \{\infty\}$, then $\tm \isub\var\tmtwo \partostratind{k} \tm' \isub\var{\tmtwo'}$ for some $k \in \nat \cup \{\infty\}$.
\end{lemma}

\begin{proof}
	By induction on the definition of $\tm \partostratind{n} \tmtwo$. 
		Cases:
		\begin{itemize}
			\item \emph{Variable}: $\tm = \vartwo \partostratind{\infty} \vartwo = \tm'$. 
			There are two sub-cases:
			\begin{enumerate}
				\item either $\vartwo = \var$ and then $\tm\isub{\var}{\tmtwo} = \tmtwo \partostratind{m} \tmtwo' = \tm'\isub{\var}{\tmtwo'}$;
				\item or $\vartwo \neq \var$ and then $\tm\isub{\var}{\tmtwo} = \vartwo \partostratind{\infty} \vartwo = \tm'\isub{\var}{\tmtwo'}$.
			\end{enumerate}
			
			\item \emph{Abstraction}: $\tm = \la \vartwo\tmthree \partostratind{n}  \la \vartwo \tmthree' = \tm'$ because $\tmthree \partostratind{n} \tmthree'$. 
			We can suppose without loss of generality that $\vartwo \notin \fv{\tmtwo} \cup \{\var\} \supseteq \fv{\tmtwo'} \cup \{\var\}$.
			By \ih, $\tmthree \partostratind{j} \tmthree'$ for some $j \in \nat \cup \{\infty\}$, so 
			\begin{align*}
			\AxiomC{$\tmthree \partostratind{j} \tmthree'$}
			\UnaryInfC{$\tm\isub{\var}{\tmtwo} = \la{\vartwo}{\tmthree\isub{\var}{\tmtwo}} \partostratind{j} \la{\vartwo}{\tmthree'\isub{\var}{\tmtwo'}} = \tm'\isub{\var}{\tmtwo'}$}
			\DisplayProof\,.
			\end{align*}
			
			\item \emph{Application}:
			\begin{align*}
			\AxiomC{$\tm_0 \partostratind{n_0} \tm'_0$}	
			\AxiomC{$\tm_1 \partostratind{n_1} \tm'_1$}
			\BinaryInfC{$\tm = \tm_0 \tm_1 \partostratind{n} \tm'_0 \tm'_1 = \tmtwo$}
			\DisplayProof 
			\end{align*}
			where $n = \min\{n_0,n_1+1\}$.
			By \ih, $\tm_0\isub{\var}{\tmtwo} \partostratind{j_0} \tm_0'\isub{\var}{\tmtwo}$ and $\tm_1\isub{\var}{\tmtwo} \partostratind{j_1} \tm_1'\isub{\var}{\tmtwo}$ for some  $j_0, j_1 \in \nat \cup \{\infty\}$.
			Therefore,
				\begin{align*}
				\AxiomC{$\tm_0\isub{\var}{\tmtwo} \partostratind{j_0} \tm_0'\isub{\var}{\tmtwo}$}
				\AxiomC{$\tm_1\isub{\var}{\tmtwo} \partostratind{j_1} \tm_1'\isub{\var}{\tmtwo}$}
				\BinaryInfC{$\tm\isub{\var}{\tmtwo} = \tm_0\isub{\var}{\tmtwo}\tm_1 \isub{\var}{\tmtwo} \partostratind{j} \tm_0'\isub{\var}{\tmtwo}\tm_1'\isub{\var}{\tmtwo} = \tm'$}
				\DisplayProof
				\end{align*}
				where $j = \min\{j_0, j_1+1\}$. 
		
			\item \emph{$\beta$-step}: 
			\begin{align*}
				\AxiomC{$\tm_0 \partostratind{n_0} \tm_0'$}
				\AxiomC{$\tm_1 \partostratind{n_1} \tm_1'$}
				\BinaryInfC{$\tm = (\la{\vartwo}\tm_0)\tm_1 \partostratind{0} \tm_0' \isub{\vartwo}{\tm_1'} = \tm'$}
				\DisplayProof
			\end{align*}
			We can suppose without loss of generality that $\vartwo \notin \fv{\tmtwo} \cup \{\var\} \supseteq \fv{\tmtwo} \cup \{\var\}$, hence $\tm'\isub{\var}{\tmtwo} = \tm_0'\isub{\vartwo}{\tm_1'}\isub{\var}{\tmtwo} = \tm_0'\isub{\var}{\tmtwo}\isub{\vartwo}{\tm_1'\isub{\var}{\tmtwo}}$.
			By \ih, $\tm_0\isub{\var}{\tmtwo} \partostratind{k_0} \tm_0'\isub{\var}{\tmtwo}$ and $\tm_1\isub{\var}{\tmtwo} \partostratind{k_1} \tm_1'\isub{\var}{\tmtwo}$ for some $k_1, k_2 \in \nat \cup \{\infty\}$.
			Therefore,
			\begin{align*}
				\AxiomC{$\tm_0\isub{\var}{\tmtwo} \partostratind{k_0} \tm_0'\isub{\var}{\tmtwo}$}
				\AxiomC{$\tm_1\isub{\var}{\tmtwo} \partostratind{k_1} \tm_1'\isub{\var}{\tmtwo}$}
				\BinaryInfC{$\tm\isub{\var}{\tmtwo} = (\la{\vartwo}\tm_0\isub{\var}{\tmtwo})\tm_1\isub{\var}{\tmtwo} \partostratind{0} \tm_0'\isub{\var}{\tmtwo} \isub{\vartwo}{\tm_1'\isub{\var}{\tmtwo}} = \tm'\isub{\var}{\tmtwo}$}
				\DisplayProof\,.
			\end{align*}
			\qedhere
		\end{itemize}
\end{proof}


\begin{lemma}[Decomposition of parallel $\beta$-steps]
\label{l:decomp-strat}
If $\tm \partobind{n} \tmtwo$ then $\tm \partostratind{m} \tmtwo$ for some $m \in \nat \cup \{\infty\}$.
If moreover $n > 0$ then $m \neq \infty$ and $\tm \tostratind{m} \tmthree$ for some term $\tmthree$ such that $\tmthree \partobindlong{n-1} \tmtwo$ and $\tmthree \partostratind{j} \tmtwo$ with $j \geq m	$ (possibly $j = \infty$).	
\end{lemma}

\begin{proof}
By induction on the definition of $\tm \partobind{n} \tmtwo$. 
Cases:
\begin{itemize}
	\item \emph{Variable}: $\tm = \var \partobind{0} \var = \tmtwo$. 
	Then,
	\begin{align*}
		\AxiomC{}
		\UnaryInfC{$\tm = \var \partostratind{\infty} \var = \tmtwo$}
		\DisplayProof
		\,.
	\end{align*}
	
	\item \emph{Abstraction}: $\tm = \la \var\tm' \partobind{n}  \la \var \tmtwo' = \tmtwo$ because $\tm' \partobind{n} \tmtwo'$. 
	By \ih, $\tm' \partostratind{m} \tmtwo'$ for some $m \in \nat \cup \{\infty\}$.
	Then,
	\begin{align*}
		\AxiomC{$\tm' \partostratind{m} \tmtwo'$}
		\UnaryInfC{$\tm = \la{\var}{\tmthree'} \partostratind{m} \la{\var}{\tmtwo'} = \tmtwo$}
		\DisplayProof
		\,.
	\end{align*}
	If moreover $n > 0$, then by \ih, $m \neq \infty$ and $\tm' \tostratind{m} \tmthree'$ for some term $\tmthree'$ such that $\tmthree' \partobindlong{n-1} \tmtwo'$ and $\tmthree' \partostratind{j} \tmtwo'$ with $j \geq m$ (possibly $j = \infty$), so 
	\begin{align*}
	\AxiomC{$\tm' \tostratind{m} \tmthree'$}
	\UnaryInfC{$\tm = \la{\var}{\tm'} \tostratind{m} \la{\var}{\tmthree'} = \tmthree$}
	\DisplayProof&
	\qquad
	\text{and}
	\qquad
	\AxiomC{$\tmthree' \partostratind{j} \tmtwo'$}
	\UnaryInfC{$\tmthree = \la{\var}{\tmthree'} \partostratind{j} \la{\var}{\tmtwo'} = \tmtwo$}
	\DisplayProof
	\\
	\shortintertext{and}
	&\AxiomC{$\tmthree' \partobind{n-1} \tmtwo'$}
	\UnaryInfC{$\tmthree = \la{\var}{\tmthree'} \partobind{n-1} \la{\var}{\tmtwo'} = \tmtwo$}
	\DisplayProof
	\,.
	\end{align*}
	
	\item \emph{Application}:
	\begin{align*}
	\AxiomC{$\tm_0 \partobind{n_0} \tmtwo_0$}	
	\AxiomC{$\tm_1 \partobind{n_1} \tmtwo_1$}
	\BinaryInfC{$\tm = \tm_0 \tm_1 \partobind{n} \tmtwo_0 \tmtwo_1 = \tmtwo$}
	\DisplayProof 
	\end{align*}
	where $n = n_0 + \cdot n_1$.
	By \ih, $\tm_0 \partostratind{m_0} \tmtwo_0$ and $\tm_1 \partostratind{m_1} \tmtwo_1$ for some $m_0, m_1 \in \nat \cup \{\infty\}$.
	Thus,
	\begin{align*}
	\AxiomC{$\tm_0 \partostratind{m_0} \tmtwo_0$}	
	\AxiomC{$\tm_1 \partostratind{m_1} \tmtwo_1$}
	\BinaryInfC{$\tm = \tm_0 \tm_1 \partostratind{m} \tmtwo_0 \tmtwo_1 = \tmtwo$}
	\DisplayProof 
	\end{align*}
	where $m = \min\{m_0,m_1+1\}$.
	If moreover $n > 0$, then by \ih, $m_0, m_1 \neq \infty$ and $\tm_0 \tostratind{m_0} \tmthree_0$ and $\tm_1 \tostratind{n_1} \tmthree_1$ for some terms $\tmthree_0, \tmthree_1$ such that $\tmthree_0 \partobindlong{n_0-1} \tmtwo_0$ and $\tmthree_1 \partobindlong{n_1-1} \tmtwo_1$ and $\tmthree_0 \partostratind{j_0} \tmtwo_0$ and $\tmthree_1 \partostratind{j_1} \tmtwo_1$ with $j_0 \geq m_0$, $j_1 \geq m_1$ (possibly $j_0,j_1 = \infty$).
	There are two possibilities:
	\begin{enumerate}
		\item $m = m_0$; then, $m_0 \leq m_1+1$ and 
		\begin{align*}
		\AxiomC{$\tm_0 \tostratind{n} \tmthree_0$}
		\UnaryInfC{$\tm = \tm_0\tm_1 \tostratind{n} \tmthree_0\tm_1 = \tmthree$}
		\DisplayProof
		&
		\qquad
		\text{and}
		\qquad
		\AxiomC{$\tmthree_0 \partobind{n_0-1} \tmtwo_0$}
		\AxiomC{$\tm_1 \partobind{n_1} \tmtwo_1$}
		\BinaryInfC{$\tmthree = \tmthree_0\tm_1 \partobind{n-1} \tmtwo_0\tmtwo_1 = \tmtwo$}
		\DisplayProof		
		\shortintertext{and}
		&
		\AxiomC{$\tmthree_0 \partostratind{j_0} \tmtwo_0$}
		\AxiomC{$\tm_1 \partostratind{n_1} \tmtwo_1$}
		\BinaryInfC{$\tmthree = \tmthree_0\tm_1 \partostratind{j} \tmtwo_0\tmtwo_1 = \tmtwo$}
		\DisplayProof
		\end{align*}
		where $j = \min\{j_0, m_1+1\} \geq m_0 = m$; 
		\item $m = m_1+1$; then, $m_1 + 1 \leq m_0$ and  
		\begin{align*}
		\AxiomC{$\tm_1 \tostratind{m} \tmthree_1$}
		\UnaryInfC{$\tm = \tm_0\tm_1 \tostratind{m} \tm_0\tmthree_1 = \tmthree$}
		\DisplayProof
		&
		\qquad
		\text{and}
		\qquad
		\AxiomC{$\tmthree_0 \partobind{n_0} \tmtwo_0$}
		\AxiomC{$\tm_1 \partobind{n_1-1} \tmtwo_1$}
		\BinaryInfC{$\tmthree = \tm_0\tmthree_1 \partobind{n-1} \tmtwo_0\tmtwo_1 = \tmtwo$}
		\DisplayProof
		\\\
		\shortintertext{and}
		&
		\AxiomC{$\tmthree_0 \partostratind{m_0} \tmtwo_0$}
		\AxiomC{$\tm_1 \partostratind{j_1} \tmtwo_1$}
		\BinaryInfC{$\tmthree = \tm_0\tmthree_1 \partostratind{j} \tmtwo_0\tmtwo_1 = \tmtwo$}
		\DisplayProof
		\end{align*}
		where $j = \min\{m_0, j_1+1\} \geq m_1+1 = m$.
	\end{enumerate}
	
	\item \emph{$\beta$-step}:
	\begin{align*}
	\AxiomC{$\tm_0 \partobind{n_0} \tm_0'$}
	\AxiomC{$\tm_1 \partobind{n_1} \tm_1'$}
	\BinaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \partobind{n} \tm_0' \isub{\var}{\tm_1'} = \tmtwo$}
	\DisplayProof
	\end{align*}
	where $n = n_0 + \sizep{\tm_0}{\var}n_1 + 1 > 0$.
	By \ih, $\tm_0 \partostratind{m_0} \tmtwo_0$ and $\tm_1 \partostratind{m_1} \tmtwo_1$ for some $m_0, m_1 \in \nat$.
	Thus,
	\begin{align*}
	\AxiomC{$\tm_0 \partostratind{m_0} \tm_0'$}
	\AxiomC{$\tm_1 \partostratind{m_1} \tm_1'$}
	\BinaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \partostratind{0} \tm_0' \isub{\var}{\tm_1'} = \tmtwo$}
	\DisplayProof
	\,.
	\end{align*}	
	Let $\tmthree = \tm_0\isub{\var}{\tm_1}$.
	By \reflemma{tob-subs}, $\tmthree = \tm_0\isub{\var}{\tm_1} \partobindlong{n_0 + \sizep{\tm_0}{\var} n_1} \tm_0'\isub{\var}{\tm_1'} = \tmtwo$ where $n_0 + \sizep{\tm_0}{\var} n_1 = n - 1$.
	Clearly,
	\begin{align*}
	\AxiomC{}
	\UnaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \tostratind{0} \tm_0 \isub{\var}{\tm_1} = \tmthree$}
	\DisplayProof
	\,.
	\end{align*}
	According to substitutivity (\reflemma{tostrat-subs}), $\tmthree = \tm_0\isub{\var}{\tm_1} \partostratind{j} \tm_0'\isub{\var}{\tm_1'} = \tmtwo$ for some $j \in \nat \cup \{\infty\}$, in particular $j \geq 0$.
	\qedhere
\end{itemize}
\end{proof}


\setcounter{propositionAppendix}{\value{prop:quant-out-in-split-strat}}
\begin{propositionAppendix}[Indexed external-internal split]
	\label{propappendix:quant-out-in-split-strat}
	\NoteState{prop:quant-out-in-split-strat}
	If $\tm \partobind n \tmtwo$ then either $\tm \partonotstrat\tmtwo$ or $n>0$ and there exists $\tmthree$ such that $\tm \tostrat \tmthree \partobindlong {n-1} \tmtwo$.
\end{propositionAppendix}

\begin{proof}
	If $n = 0$, then $\tm = \tmtwo$ (because $\partobind{0}$ is the identity relation) and so $\tm \partostratind{\infty} \tmtwo$ (because $\partostratind{\infty}$ is the identity relation), hence $\tm \partonotstrat \tmtwo$. %It requires that $\partonotstrat$ contains the infinite index and that $\partobind{0}$ is the identity relation (not only reflexive).
	
	Otherwise $n > 0$ and then, by \reflemma{decomp-strat}, $\tm \partostratind{k} \tmtwo$ and $\tm \tostratind{k} \tmthree$ for some $k \in \nat$ and some term $\tmthree$ such that $\tmthree \partobind{n-1} \tmtwo$ and $\tmthree \partostratind{j} \tmtwo$ with $j \geq k$.
	There are two cases:
	\begin{enumerate}
		\item either $k$ is not minimal for $\tm$ (\ie $\tm \tostratind{k'} \tmthree'$ for some $\tmthree'$ and some $k' < k$), and then $\tm \partonotstrat \tmtwo$ (since $\tm \partostratind{k} \tmtwo$);
		\item or $k$ is minimal for $\tm$ (\ie if $\tm \tostratind{k'} \tmthree'$ for some $\tmthree'$ then $k' \geq k$), and so $\tm \tostrat \tmthree \partobind{n-1} \tmtwo$.
		\qedhere
	\end{enumerate}
\end{proof}


==> proofs/proofs-stratified-cbn2CF.tex <==
% !TEX root = ../main.tex
\subsection{Omitted proofs and lemmas of \refsect{stratified-cbn}}
\newcommand{\partonotst}{\partonotstrat}


 We show that $\partonotstrat$ does not increase the degree of a term. Hence in particular the same holds for $\tonst$.

\newcounter{l:perpetuity-strat}
\addtocounter{l:perpetuity-strat}{\value{lemma}}
\begin{lemma}[Persistence]
	\label{l:perpetuity-strat}
	\NoteProof{lappendix:perpetuity-strat}
	\begin{enumerate}
		\item If $\tm \parto \tmtwo$ then $\Deg{\tmtwo} \geq \Deg{\tm}$. 
		\item 	If $\tm \partonotstrat \tmtwo$ then $\Deg{\tmtwo} = \Deg{\tm}$. 
	\end{enumerate}
\end{lemma}

\begin{proof}
\textbf{1.} is easily proved by a straightfoward induction on $\parto$.

\textbf{2}. is proved by induction on $\tm$. 	By hypothesis, $\tm \partostratind{n} \tmtwo$ for some $n > \Deg{\tm}$.
We prove that $\Deg{\tmtwo} = \Deg{\tm}$.
Cases:
\begin{itemize}
	\item $\tm = \var \parto \var = \tmtwo$. 
	Then, $\Deg{\tm}  = \Deg{\tmtwo}$.
	
	\item $\tm = \la \var\tm' \partostratind{n}  \la \var \tmtwo' = \tmtwo$ with  $\tm' \partostratind{n} \tmtwo'$. 
	Since $n > \Deg{\tm} = \Deg{\tm'}$, by \ih we have  $\Deg{\tmtwo} = \Deg{\tmtwo'} = \Deg{\tm'} = \Deg{\tm}$.
	
	\item $\tm$ is an \emph{application}. We consider two case, according to the definition of $\Deg{\tm}$
	
\begin{itemize}
	
	\item 	Assume $\tm=(\la{\var}\tm_0)\tm_1$. We have  $\Deg{\tm}=0$ and since $\tm \partostratind{n} \tmtwo$ with $n > 0$,
	the only possible derivation is the following.
	
	\begin{align*}
	\AxiomC{$\tm_0 \parto \tmtwo_0$}
	\UnaryInfC{$\la{\var}\tm_0 \parto \la{\var}\tmtwo_0$}
	\AxiomC{$\tm_1 \parto \tmtwo_1$}
	\BinaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \parto (\la{\var}{\tmtwo_0})\tmtwo_1 = \tmtwo$}
	\DisplayProof
	\end{align*}
	Therefore,  $\Deg{\tmtwo} = 0 = \Deg{\tm}$.
	
	
\item  Assume $\tm=\tm_0\tm_1$, where $\tm_0$ is not an abstraction. We have
\begin{align*}
\AxiomC{$\tm_0 \partostratind{n_0} \tmtwo_0$}	
\AxiomC{$\tm_1 \partostratind{n_1} \tmtwo_1$}
\BinaryInfC{$\tm = \tm_0 \tm_1 \partostratind{n} \tmtwo_0 \tmtwo_1 = \tmtwo$}
\DisplayProof 
\end{align*}
where $n = \min\{n_0,n_1+1\}$ and $ \deg{\tm} =\min \{\deg {\tm_0}, \deg {\tm_1} +1)\}$. 
\begin{enumerate}
	\item  If $\deg {\tm_0}$ is  minimal, then 
	$n_0\geq n > \deg {\tm_0} $. Therefore $\tm_0 \partonotstrat \tmtwo_0$ and by the \ih, $\deg{\tm_0}=\deg{\tms_0}$.
	We also know (by point 1.) that $\deg {\tms_1}\geq \deg {\tm_1}$, hence $ \deg{\tms} =\min \{\deg {\tms_0}, \deg {\tms_1} +1)
	= \deg {\tms_0}= \deg {\tm_0} = \deg{\tm}$.
	
	\item If $\deg {\tm_1} +1$ is minimal, then $n_1+1 \geq n> \deg {\tm_1+1}$, hence $n_1 > \deg{\tm_1}$.  Therefore $\tm_1 \partonotstrat \tmtwo_1$ and by the \ih, $\deg{\tm_1}=\deg{\tms_1}.$, and we conclude similarly to the previous case.
\end{enumerate}

	
\end{itemize}
\end{itemize}
	
\end{proof}

\setcounter{lemmaAppendix}{\value{l:perpetuity-strat}}
\begin{lemmaAppendix}[Persistence]
\label{lappendix:perpetuity-strat}
\NoteState{l:perpetuity-strat}
	If $\tm \partonotstrat \tmtwo$ then $\Deg{\tmtwo} \leq \Deg{\tm}$. 
\end{lemmaAppendix}

\begin{proof}
	By hypothesis, $\tm \partostratind{n} \tmtwo$ for some $n > \Deg{\tm}$.
	We prove that $\Deg{\tmtwo} \leq \Deg{\tm}$ by induction on the definition of $\tm \partostratind{n} \tmtwo$.
	Cases:
	\begin{itemize}
		\item \emph{Variable}: $\tm = \var \partostratind{\infty} \var = \tmtwo$. 
		Then, $\Deg{\tm} = \infty = \Deg{\tmtwo}$.
		
		\item \emph{Abstraction}: $\tm = \la \var\tm' \partostratind{n}  \la \var \tmtwo' = \tmtwo$ because $\tm' \partostratind{n} \tmtwo'$.
		As $n > \Deg{\tm} = \Deg{\tm'}$, then $\Deg{\tmtwo} = \Deg{\tmtwo'} \leq \Deg{\tm'} = \Deg{\tm}$ by \ih
		
		\item \emph{Application}:
		\begin{align*}
		\AxiomC{$\tm_0 \partostratind{n_0} \tmtwo_0$}	
		\AxiomC{$\tm_1 \partostratind{n_1} \tmtwo_1$}
		\BinaryInfC{$\tm = \tm_0 \tm_1 \partostratind{n} \tmtwo_0 \tmtwo_1 = \tmtwo$}
		\DisplayProof 
		\end{align*}
		where $n = \min\{n_0,n_1+1\}$.
		According to the definition of $\Deg{\tm}$, there are the following sub-cases:
		\begin{enumerate}
			\item $\Deg{\tm} = \Deg{\tm_0} \leq \Deg{\tm_1} + 1$ and $\tm_0$ is not an abstraction; 
			%here it is important to take the min in the for the index application case of the definition of \partostratind{n}
			by \ih applied to $\tm_0$ (since $\Deg{\tm_0} = \Deg{\tm} < n \leq n_0$), we have $\Deg{\tmtwo_0} \leq \Deg{\tm_0}$, and so (as $\Deg{\tm_0} \leq \Deg{\tm_1} + 1$) $\Deg{\tmtwo} = \min \{\Deg{\tmtwo_0}, \Deg{\tmtwo_1} + 1\} \leq \min\{\Deg{\tm_0}, \Deg{\tm_1} + 1\} = \Deg{\tm}$.
			
			\item $\Deg{\tm} = \Deg{\tm_1} + 1 \leq \Deg{\tm_0}$ and $\tm_0$ is not an abstraction; 
			%here it is important to take the min in the for the index application case of the definition of \partostratind{n}
			by \ih applied to $\tm_1$ (since $\Deg{\tm_1} + 1 = \Deg{\tm} < n \leq n_1+1$ and hence $\Deg{\tm_1} < n_1$), we have $\Deg{\tmtwo_1} \leq \Deg{\tm_1}$, and so (as $\Deg{\tm_1} + 1 \leq \Deg{\tm_0}$) $\Deg{\tmtwo} = \min \{\Deg{\tmtwo_0}, \Deg{\tmtwo_1} + 1\} \leq \min\{\Deg{\tm_0}, \Deg{\tm_1} + 1\} = \Deg{\tm}$.
			
			\item $\Deg{\tm} = 0$ and $\tm_0$ is an abstraction. 
			According to the definition of $\tm \partostratind{n} \tmtwo$, since $n > 0$, we have
				\begin{align*}
				\AxiomC{$\tm_0 \partostratind{n_0} \tmtwo_0$}
				\UnaryInfC{$\la{\var}\tm_0 \partostratind{n_0} \la{\var}\tmtwo_0$}
				\AxiomC{$\tm_1 \partostratind{n_1} \tmtwo_1$}
				\BinaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \partostratind{n} (\la{\var}{\tmtwo_0})\tmtwo_1 = \tmtwo$}
				\DisplayProof
				\end{align*}
				where $n = \min\{n_0, n_1+1\}$; therefore $\Deg{\tmtwo} = 0 = \Deg{\tm}$.
		\end{enumerate}
		
		\item \emph{$\beta$-step}: 
		\begin{align*}
		\AxiomC{}
		\UnaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \partostratind{0} \tm_0 \isub{\var}{\tm_1} = \tmtwo$}
		\DisplayProof
		\end{align*}
		where $0 = n > \Deg{\tm}$, which is impossible.
		\qedhere
	\end{itemize}
\end{proof}

%\begin{lemma}[Decomposition of parallel $n$-depth $\beta$-steps]
%	\label{l:decomp-strat}
%%	Let $\tm \partostratind{n} \tmtwo$ with $n \neq \infty$.
%%	\begin{enumerate}
%%		\item \label{p:decomp-strat-ind} Then, $\tm \tostratind{n} \tmthree \partostratind{j} \tmtwo$ for some term $\tmthree$ and some $j \geq n$ (possibly $j = \infty$).	
%%		
%%		\item\label{p:decomp-strat-notstrat} If moreover $\tm \partonotstrat \tmtwo$, then $n > 0 $ and $\tm \tostratind{k} \tmfour$ for some $\tmfour$ and some $k < n$.
%%	\end{enumerate}
%	If $\tm \partostratind{n} \tmtwo$ with $n \neq \infty$, then $\tm \tostratind{n} \tmthree \partostratind{j} \tmtwo$ for some term $\tmthree$ and some $j \geq n$ (possibly $j = \infty$).	
%\end{lemma}
%
%\begin{proof}
%	By induction on the definition of $\tm \partostratind{n} \tmtwo$. 
%		Cases:
%		\begin{itemize}
%			\item \emph{Variable}: $\tm = \var \partostratind{\infty} \var = \tmtwo$. 
%			This is impossible because $n \neq \infty$ by hypothesis.
%			
%			\item \emph{Abstraction}: $\tm = \la \var\tm' \partostratind{n}  \la \var \tmtwo' = \tmtwo$ because $\tm' \partostratind{n} \tmtwo'$. 
%			By \ih, $\tm' \tostratind{n} \tmthree' \partostratind{j} \tmtwo'$ for some term $\tmthree'$ and some $j \geq n$ (possibly $j = \infty$), so 
%			\begin{align*}
%			\AxiomC{$\tm' \tostratind{n} \tmthree'$}
%			\UnaryInfC{$\tm = \la{\var}{\tm'} \tostratind{n} \la{\var}{\tmthree'} = \tmthree$}
%			\DisplayProof
%			\qquad
%			\text{and}
%			\qquad
%			\AxiomC{$\tmthree' \partostratind{j} \tmtwo'$}
%			\UnaryInfC{$\tmthree = \la{\var}{\tmthree'} \partostratind{j} \la{\var}{\tmtwo'} = \tmtwo$}
%			\DisplayProof\,.
%			\end{align*}
%			
%			\item \emph{Application}:
%			\begin{align*}
%			\AxiomC{$\tm_0 \partostratind{n_0} \tmtwo_0$}	
%			\AxiomC{$\tm_1 \partostratind{n_1} \tmtwo_1$}
%			\BinaryInfC{$\tm = \tm_0 \tm_1 \partostratind{n} \tmtwo_0 \tmtwo_1 = \tmtwo$}
%			\DisplayProof 
%			\end{align*}
%			where $n = \min\{n_0,n_1+1\}$.
%			By \ih, $\tm_0 \tostratind{n_0} \tmthree_0 \partostratind{j_0} \tmthree_0$ and $\tm_1 \tostratind{n_1} \tmthree_1 \partostratind{j_1} \tmthree_1$ for some terms $\tmthree_0, \tmthree_1$ and some $j_0 \geq n_0$, $j_1 \geq n_1$ (possibly $j_0,j_1 = \infty$).
%			There are two possibilities:
%			\begin{enumerate}
%				\item $n = n_0$; then, $n_0 \leq n_1+1$ and 
%				\begin{align*}
%				\AxiomC{$\tm_0 \tostratind{n} \tmthree_0$}
%				\UnaryInfC{$\tm = \tm_0\tm_1 \tostratind{n} \tmthree_0\tm_1 = \tmthree$}
%				\DisplayProof
%				\qquad
%				\text{and}
%				\qquad
%				\AxiomC{$\tmthree_0 \partostratind{j_0} \tmtwo_0$}
%				\AxiomC{$\tm_1 \partostratind{n_1} \tmtwo_1$}
%				\BinaryInfC{$\tmthree = \tmthree_0\tm_1 \partostratind{j} \tmtwo_0\tmtwo_1 = \tmtwo$}
%				\DisplayProof
%				\end{align*}
%				where $j = \min\{j_0, n_1+1\} \geq n_0 = n$; 
%				\item $n = n_1+1$; then, $n_1 + 1 \leq n_0$ and  
%				\begin{align*}
%					\AxiomC{$\tm_1 \tostratind{n} \tmthree_1$}
%					\UnaryInfC{$\tm = \tm_0\tm_1 \tostratind{n} \tm_0\tmthree_1 = \tmthree$}
%					\DisplayProof
%					\qquad
%					\text{and}
%					\qquad
%					\AxiomC{$\tmthree_0 \partostratind{n_0} \tmtwo_0$}
%					\AxiomC{$\tm_1 \partostratind{j_1} \tmtwo_1$}
%					\BinaryInfC{$\tmthree = \tm_0\tmthree_1 \partostratind{j} \tmtwo_0\tmtwo_1 = \tmtwo$}
%					\DisplayProof
%				\end{align*}
%				where $j = \min\{n_0, j_1+1\} \geq n_1+1 = n$.
%			\end{enumerate}
%		
%			\item \emph{$\beta$-step}: 
%			\begin{align*}
%				\AxiomC{}
%				\UnaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \partostratind{0} \tm_0 \isub{\var}{\tm_1} = \tmtwo$}
%				\DisplayProof
%			\end{align*}
%			Let $\tmthree = \tmtwo$: then $\tmthree \partostratind{\infty} \tmtwo$ and
%			\begin{align*}
%				\AxiomC{}
%				\UnaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \tostratind{0} \tm_0 \isub{\var}{\tm_1} = \tmthree$}
%				\DisplayProof\,.
%			\end{align*}
%			\qedhere
%		\end{itemize}
%\end{proof}


%%\setcounter{propositionAppendix}{\value{prop:i-e-merge-strat}}
%\begin{propositionAppendix}[Merge]
%	\label{propappendix:i-e-merge-strat}
%	\NoteState{prop:i-e-merge-strat}
%	\begin{enumerate}
%		\item If $\tm \partostratind{n}\tmtwo \tostratind{m} \tmthree$ with $n > m$, then $\tm \partob \tmthree$. %and $\tm \tostratind{m} \tmfour$ for some term $\tmfour$.
%		\item If $\tm \partonotstrat \tmtwo \tostrat \tmthree$, then $\tm \partob \tmthree$.
%	\end{enumerate}
%\end{propositionAppendix}

%\setcounter{propositionAppendix}{\value{prop:i-e-merge-strat}}
\begin{propositionAppendix}[Merge]
	\label{propappendix:i-e-merge-strat}
	\NoteState{prop:i-e-merge-strat}
	\ If $\tm \partonotstrat \tmtwo \tostrat \tmthree$, then $\tm \partob \tmthree$.
\end{propositionAppendix}

\begin{proof}\hfill
	We first prove a stronger hypothesis, from which the claim  follows. 
	\begin{enumerate}
		
	\item We prove the following property 
	\begin{center}
	(\#) 	If $\tm \partostratind{n}\tmtwo \tostratind{m} \tmthree$ with $n > m$, then $\tm \partob \tmthree$. 
	\end{center}
	by induction on the definition of $\tm \partostratind{n} \tmtwo$.
	Cases:
	\begin{itemize}
		\item \emph{Variable}: $\tm = \var \partostratind{\infty} \var = \tmtwo$. 
		Then, there is no $\tmthree$ such that $\tmtwo \tostratind{m} \tmthree$ for any $m \in \nat$.
		
		\item \emph{Abstraction}: $\tm = \la \var\tm' \partostratind{n}  \la \var \tmtwo' = \tmtwo$ because $\tm' \partostratind{n} \tmtwo'$. 
		According to the definition of $\tmtwo \tostratind{m} \tmthree$, by necessity $\tmthree = \la{\var}{\tmthree'}$ with $\tmtwo' \tostratind{m} \tmthree'$.
		By \ih, $\tm' \partobv \tmthree'$, thus 
		\begin{align*}
		\AxiomC{$\tm' \partobv \tmthree'$}
		\UnaryInfC{$\tm = \la{\var}{\tm'} \partobv \la{\var}{\tmthree'} = \tmthree$}
		\DisplayProof
		\,.
		\end{align*}
		
		\item \emph{Application}:
		\begin{align*}
		\AxiomC{$\tm_0 \partostratind{n_0} \tmtwo_0$}	
		\AxiomC{$\tm_1 \partostratind{n_1} \tmtwo_1$}
		\BinaryInfC{$\tm = \tm_0 \tm_1 \partostratind{n} \tmtwo_0 \tmtwo_1 = \tmtwo$}
		\DisplayProof 
		\end{align*}
		where $n = \min\{n_0,n_1+1\}$.
		According to the definition of $\tmtwo \tostratind{m} \tmthree$, there are the following sub-cases:
		\begin{enumerate}
			\item $\tmtwo = \tmtwo_0\tmtwo_1 \tostratind{m} \tmthree_0\tmtwo_1 = \tmthree$ with $\tmtwo_0 \tostratind{m} \tmthree_0$; 
			since $m < n \leq n_0$, %here it is important to take the min in the for the index application case of the definition of \partostratind{n}
			by \ih applied to $\tm_0 \partostratind{n_0} \tmtwo_0 \tostratind{m} \tmthree_0$, we have $\tm_0 \partobv \tmthree_0$, and so (as $\partostratind{n_1} \,\subseteq\, \partobv$)
			\begin{align*}
			\AxiomC{$\tm_0 \partobv \tmthree_0$}
			\AxiomC{$\tm_1 \partobv \tmtwo_1$}
			\BinaryInfC{$\tm = \tm_0\tm_1 \partobv \tmthree_0\tmtwo_1 = \tmthree$}
			\DisplayProof
			\,;
			\end{align*}
			\item $\tmtwo = \tmtwo_0\tmtwo_1 \tostratind{m} \tmthree_0\tmtwo_1 = \tmthree$ with $\tmtwo_1 \tostratind{m-1} \tmthree_1$; 
			since $m-1 < n-1 \leq n_1$,
			by \ih applied to $\tm_1 \partostratind{n_1} \tmtwo_1 \tostratind{m-1} \tmthree_1$, we have $\tm_1 \partobv \tmthree_1$, and so (as $\tm_0 \partostratind{n_0} \,\subseteq\, \partobv$)
			\begin{align*}
			\AxiomC{$\tm_0 \partobv \tmtwo_0$}
			\AxiomC{$\tm_1 \partobv \tmthree_1$}
			\BinaryInfC{$\tm = \tm_0\tm_1 \partobv \tmtwo_0\tmthree_1 = \tmthree$}
			\DisplayProof
			\,;
			\end{align*}		
			%			analogous to the previous sub-case.
			\item $\tmtwo = (\la{\var}{\tmtwo_0})\tmtwo_1 \tostratind{0} \tmtwo_0\isub{\var}{\tmtwo_1} = \tmthree$ with $m = 0$; 
			as $n > 0$ then, according to the definition of $\tm \partostratind{n} \tmtwo$,
			\begin{align*}
			\AxiomC{$\tm_0 \partostratind{n_0} \tmtwo_0$}
			\UnaryInfC{$\la{\var}\tm_0 \partostratind{n_0} \la{\var}\tmtwo_0$}
			\AxiomC{$\tm_1 \partostratind{n_1} \tmtwo_1$}
			\BinaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \partostratind{n} (\la{\var}{\tmtwo_0})\tmtwo_1 = \tmtwo$}
			\DisplayProof
			\end{align*}
			where $n = \min\{n_0, n_1+1\}$; therefore (as $\partostratind{k} \,\subseteq\, \partobv$)
			\begin{align*}
			\AxiomC{$\tm_0 \partobv \tmtwo_0$}
			\AxiomC{$\tm_1 \partobv \tmtwo_1$}
			\BinaryInfC{$\tm = (\la{\var}{\tm_0})\tm_1 \partobv \tmtwo_0\isub{\var}{\tmtwo_1} = \tmthree$}
			\DisplayProof
			\,.
			\end{align*}
		\end{enumerate}
	\end{itemize}

	\item As $\tm \partonotstrat \tmtwo \tostrat \tmthree$, then $\tm \partostratind{n} \tmtwo \tostratind{m} \tmthree$ for some $n \in \nat \cup \{\infty\}$ and $m \in \nat$ such that $n > \Deg{\tm}$ and  $m = \Deg{\tmtwo}$.
	By (\reflemma{perpetuity-strat},  $\Deg{\tm} = \Deg{\tmtwo}$.
	Hence, $n > m$ and we can then merge (by \refpropp{i-e-merge-strat}{ind}) to $\tm \partob \tmthree$.
	\qedhere
	\end{enumerate}
\end{proof}

%\begin{lemma}
%	If $\tm \partob \tmtwo$ then $\tm \partostratind{m} \tmtwo$ for some $m \in \nat \cup \{\infty\}$.
%\end{lemma}
%
%\begin{proof}
%	By hypothesis, $\tm \partobind{n} \tmtwo$ for some $n \in \nat$.
%	The statement by straightforward induction on the definition of $\tm \partobind{n} \tmtwo$. 
%\end{proof}


%\begin{lemma}[Decomposition of parallel $\beta$-steps]
%\label{l:decomp-strat}
%If $\tm \partobind{n} \tmtwo$ with $n > 0$, then there are a term $\tmthree$ and $m \in \nat$ such that $\tm \tostratind{m} \tmthree \partobindlong{n-1} \tmtwo$ and $\tm \partostratind{m} \tmtwo$.	
%\end{lemma}
%
%\begin{proof}
%By induction on the definition of $\tm \partobind{n} \tmtwo$. 
%Cases:
%\begin{itemize}
%	\item \emph{Variable}: $\tm = \var \partobind{0} \var = \tmtwo$.
%	This is impossible because $n > 0$ by hypothesis.
%	
%	\item \emph{Abstraction}: $\tm = \la \var\tm' \partobind{n}  \la \var \tmtwo' = \tmtwo$ because $\tm' \partobind{n} \tmtwo'$. 
%	By \ih,   $\tm' \tostratind{m} \tmthree'$ for some term $\tmthree'$ and some $m \in \nat$ such that $\tmthree' \partobindlong{n-1} \tmtwo'$ and $\tm' \partostratind{m} \tmtwo'$, so 
%	\begin{align*}
%	\AxiomC{$\tm' \tostratind{m} \tmthree'$}
%	\UnaryInfC{$\tm = \la{\var}{\tm'} \tostratind{m} \la{\var}{\tmthree'} = \tmthree$}
%	\DisplayProof&
%	\qquad
%	\text{and}
%	\qquad
%	\AxiomC{$\tmthree' \partobind{n-1} \tmtwo'$}
%	\UnaryInfC{$\tmthree = \la{\var}{\tmthree'} \partobind{n-1} \la{\var}{\tmtwo'} = \tmtwo$}
%	\DisplayProof
%	\shortintertext{and}
%	\AxiomC{$\tm' \partostratind{m} \tmtwo'$}
%	\UnaryInfC{$\tm = \la{\var}{\tm'} \partostratind{m} \la{\var}{\tmtwo'} = \tmtwo$}
%	\DisplayProof
%	\,.
%	\end{align*}
%	
%	\item \emph{Application}:
%	\begin{align*}
%	\AxiomC{$\tm_0 \partobind{n_0} \tmtwo_0$}	
%	\AxiomC{$\tm_1 \partobind{n_1} \tmtwo_1$}
%	\BinaryInfC{$\tm = \tm_0 \tm_1 \partobind{n} \tmtwo_0 \tmtwo_1 = \tmtwo$}
%	\DisplayProof 
%	\end{align*}
%	where $n = n_0 +  n_1$.
%	By \ih, $\tm_0 \tostratind{m_0} \tmthree_0$ and $\tm_1 \tostratind{m_1} \tmthree_1$ for some terms $\tmthree_0, \tmthree_1$ and some $m_0, m_1 \in \nat$ such that $\tmthree_0 \partobindlong{n_0-1} \tmtwo_0$ and $\tmthree_1 \partobindlong{n_1-1} \tmtwo_1$ and $\tm_0 \partostratind{m_0} \tmthree_0$ and $\tm_1 \partostratind{m_1} \tmthree_1$.
%	Therefore,
%	\begin{align*}
%	\AxiomC{$\tm_0 \partostratind{m_0} \tmtwo_0$}
%	\AxiomC{$\tm_1 \partostratind{m_1} \tmtwo_1$}
%	\BinaryInfC{$\tm = \tm_0\tm_1 \partostratind{m} \tmtwo_0\tmtwo_1 = \tmtwo$}
%	\DisplayProof			
%	\end{align*}
%	where $m = \min\{m_0, m_1+1\}$.
%	There are two possibilities:
%	\begin{enumerate}
%		\item $m = m_0$; then 
%		\begin{align*}
%		\AxiomC{$\tm_0 \tostratind{m} \tmthree_0$}
%		\UnaryInfC{$\tm = \tm_0\tm_1 \tostratind{m} \tmthree_0\tm_1 = \tmthree$}
%		\DisplayProof
%		\qquad
%		\text{and}
%		\qquad
%		&
%		\AxiomC{$\tmthree_0 \partobind{n_0-1} \tmtwo_0$}
%		\AxiomC{$\tm_1 \partobind{n_1} \tmtwo_1$}
%		\BinaryInfC{$\tmthree = \tmthree_0\tm_1 \partobind{n-1} \tmtwo_0\tmtwo_1 = \tmtwo$}
%		\DisplayProof		
%		\,;
%		\end{align*}
%	
%		\item $m = m_1+1$; then 
%		\begin{align*}
%		\AxiomC{$\tm_1 \tostratind{m-1} \tmthree_1$}
%		\UnaryInfC{$\tm = \tm_0\tm_1 \tostratind{m} \tm_0\tmthree_1 = \tmthree$}
%		\DisplayProof
%		\qquad
%		\text{and}
%		\qquad
%		\AxiomC{$\tmthree_0 \partobind{n_0} \tmtwo_0$}
%		\AxiomC{$\tm_1 \partobind{n_1-1} \tmtwo_1$}
%		\BinaryInfC{$\tmthree = \tm_0\tmthree_1 \partobind{n-1} \tmtwo_0\tmtwo_1 = \tmtwo$}
%		\DisplayProof
%		\,.
%		\end{align*}
%	\end{enumerate}
%	
%	\item \emph{$\beta$-step}:
%	\begin{align*}
%	\AxiomC{$\tm_0 \partobind{n_0} \tm_0'$}
%	\AxiomC{$\tm_1 \partobind{n_1} \tm_1'$}
%	\BinaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \partobind{n} \tm_0' \isub{\var}{\tm_1'} = \tmtwo$}
%	\DisplayProof
%	\end{align*}
%	where $n = n_0 + \sizep{\tm_0}{\var}n_1 + 1 > 0$.
%	By \ih, $\tm_0 \partostratind{m_0} \tmtwo_0$ and $\tm_1 \partostratind{m_1} \tmtwo_1$ for some $m_0, m_1 \in \nat$.
%	Thus,
%	\begin{align*}
%	\AxiomC{$\tm_0 \partostratind{m_0} \tm_0'$}
%	\AxiomC{$\tm_1 \partostratind{m_1} \tm_1'$}
%	\BinaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \partostratind{0} \tm_0' \isub{\var}{\tm_1'} = \tmtwo$}
%	\DisplayProof
%	\,.
%	\end{align*}	
%	Let $\tmthree = \tm_0\isub{\var}{\tm_1}$.
%	By \reflemma{tob-subs}, $\tmthree = \tm_0\isub{\var}{\tm_1} \partobindlong{n_0 + \sizep{\tm_0}{\var} n_1} \tm_0'\isub{\var}{\tm_1'} = \tmtwo$ where $n_0 + \sizep{\tm_0}{\var} n_1 = n - 1$.
%	Clearly,
%	\begin{align*}
%	\AxiomC{}
%	\UnaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \tostratind{0} \tm_0 \isub{\var}{\tm_1} = \tmthree$}
%	\DisplayProof
%	\,.
%	\end{align*}
%	According to substitutivity (\reflemma{tob-subs}), $\tmthree = \tm_0\isub{\var}{\tm_1} \partostratind{j} \tm_0'\isub{\var}{\tm_1'} = \tmtwo$ for some $j \in \nat \cup \{\infty\}$, in particular $j \geq 0$.
%	\qedhere
%\end{itemize}
%\end{proof}
\begin{lemma}[Decomposition of parallel $\beta$-steps]
\label{l:decomp-strat}
If $\tm \partobind{n} \tmtwo$ then $\tm \partostratind{m} \tmtwo$ for some $m \in \nat \cup \{\infty\}$.
If moreover $n > 0$ then $m \neq \infty$ and $\tm \tostratind{m} \tmthree$ for some term $\tmthree$ such that $\tmthree \partobindlong{n-1} \tmtwo$ and $\tmthree \partostratind{j} \tmtwo$ with $j \geq m	$ (possibly $j = \infty$).	
\end{lemma}

\begin{proof}
By induction $(n,k) \in \nat \times \nat$ with the lexicographical order, where $k$ is the length of the derivation of $\tm \partobind{n} \tmtwo$. 
Cases:
\begin{itemize}
	\item \emph{Variable}: $\tm = \var \partobind{0} \var = \tmtwo$ where $n = 0$. 
	Then,
	\begin{align*}
	\AxiomC{}
	\UnaryInfC{$\tm = \var \partostratind{\infty} \var = \tmtwo$}
	\DisplayProof
	\,.
	\end{align*}
	
	\item \emph{Abstraction}: $\tm = \la \var\tm' \partobind{n}  \la \var \tmtwo' = \tmtwo$ because $\tm' \partobind{n} \tmtwo'$. 
	By \ih, $\tm' \partostratind{m} \tmtwo'$ for some $m \in \nat \cup \{\infty\}$.
	Then,
	\begin{align*}
	\AxiomC{$\tm' \partostratind{m} \tmtwo'$}
	\UnaryInfC{$\tm = \la{\var}{\tmthree'} \partostratind{m} \la{\var}{\tmtwo'} = \tmtwo$}
	\DisplayProof
	\,.
	\end{align*}
	If moreover $n > 0$, then by \ih, $m \neq \infty$ and $\tm' \tostratind{m} \tmthree'$ for some term $\tmthree'$ such that $\tmthree' \partobindlong{n-1} \tmtwo'$ and $\tmthree' \partostratind{j} \tmtwo'$ with $j \geq m$ (possibly $j = \infty$), so 
	\begin{align*}
	\AxiomC{$\tm' \tostratind{m} \tmthree'$}
	\UnaryInfC{$\tm = \la{\var}{\tm'} \tostratind{m} \la{\var}{\tmthree'} = \tmthree$}
	\DisplayProof
	\qquad
	\text{and}
	\qquad
	&
	\AxiomC{$\tmthree' \partostratind{j} \tmtwo'$}
	\UnaryInfC{$\tmthree = \la{\var}{\tmthree'} \partostratind{j} \la{\var}{\tmtwo'} = \tmtwo$}
	\DisplayProof
	\shortintertext{and}
	\AxiomC{$\tmthree' \partobind{n-1} \tmtwo'$}
	\UnaryInfC{$\tmthree = \la{\var}{\tmthree'} \partobind{n-1} \la{\var}{\tmtwo'} = \tmtwo$}
	\DisplayProof
	\,.
	\end{align*}
	
	\item \emph{Application}:
	\begin{align*}
	\AxiomC{$\tm_0 \partobind{n_0} \tmtwo_0$}	
	\AxiomC{$\tm_1 \partobind{n_1} \tmtwo_1$}
	\BinaryInfC{$\tm = \tm_0 \tm_1 \partobind{n} \tmtwo_0 \tmtwo_1 = \tmtwo$}
	\DisplayProof 
	\end{align*}
	where $n = n_0 + n_1$.
	By \ih, $\tm_0 \partostratind{m_0} \tmtwo_0$ and $\tm_1 \partostratind{m_1} \tmtwo_1$ for some $m_0, m_1 \in \nat \cup \{\infty\}$.
	Thus,
	\begin{align*}
	\AxiomC{$\tm_0 \partostratind{m_0} \tmtwo_0$}	
	\AxiomC{$\tm_1 \partostratind{m_1} \tmtwo_1$}
	\BinaryInfC{$\tm = \tm_0 \tm_1 \partostratind{m} \tmtwo_0 \tmtwo_1 = \tmtwo$}
	\DisplayProof 
	\end{align*}
	where $m = \min\{m_0,m_1+1\}$.
	If moreover $n > 0$, then by \ih, $m_0, m_1 \neq \infty$ and $\tm_0 \tostratind{m_0} \tmthree_0$ and $\tm_1 \tostratind{n_1} \tmthree_1$ for some terms $\tmthree_0, \tmthree_1$ such that $\tmthree_0 \partobindlong{n_0-1} \tmtwo_0$ and $\tmthree_1 \partobindlong{n_1-1} \tmtwo_1$ and $\tmthree_0 \partostratind{j_0} \tmtwo_0$ and $\tmthree_1 \partostratind{j_1} \tmtwo_1$ with $j_0 \geq m_0$, $j_1 \geq m_1$ (possibly $j_0,j_1 = \infty$).
	There are two possibilities:
	\begin{enumerate}
		\item $m = m_0$; then, $m_0 \leq m_1+1$ and 
		\begin{align*}
		\AxiomC{$\tm_0 \tostratind{m} \tmthree_0$}
		\UnaryInfC{$\tm = \tm_0\tm_1 \tostratind{m} \tmthree_0\tm_1 = \tmthree$}
		\DisplayProof
		\qquad
		\text{and}
		\qquad
		&
		\AxiomC{$\tmthree_0 \partobind{n_0-1} \tmtwo_0$}
		\AxiomC{$\tm_1 \partobind{n_1} \tmtwo_1$}
		\BinaryInfC{$\tmthree = \tmthree_0\tm_1 \partobind{n-1} \tmtwo_0\tmtwo_1 = \tmtwo$}
		\DisplayProof		
		\shortintertext{and}
		\AxiomC{$\tmthree_0 \partostratind{j_0} \tmtwo_0$}
		\AxiomC{$\tm_1 \partostratind{m_1} \tmtwo_1$}
		\BinaryInfC{$\tmthree = \tmthree_0\tm_1 \partostratind{j} \tmtwo_0\tmtwo_1 = \tmtwo$}
		\DisplayProof
		\end{align*}
		where $j = \min\{j_0, m_1+1\} \geq m_0 = m$; 
		\item $m = m_1+1$; then, $m_1 + 1 \leq m_0$ and  
		\begin{align*}
		\AxiomC{$\tm_1 \tostratind{m-1} \tmthree_1$}
		\UnaryInfC{$\tm = \tm_0\tm_1 \tostratind{m} \tm_0\tmthree_1 = \tmthree$}
		\DisplayProof
		\qquad
		\text{and}
		\qquad
		&
		\AxiomC{$\tmthree_0 \partobind{n_0} \tmtwo_0$}
		\AxiomC{$\tm_1 \partobind{n_1-1} \tmtwo_1$}
		\BinaryInfC{$\tmthree = \tm_0\tmthree_1 \partobind{n-1} \tmtwo_0\tmtwo_1 = \tmtwo$}
		\DisplayProof
		\shortintertext{and}
		\AxiomC{$\tmthree_0 \partostratind{m_0} \tmtwo_0$}
		\AxiomC{$\tm_1 \partostratind{j_1} \tmtwo_1$}
		\BinaryInfC{$\tmthree = \tm_0\tmthree_1 \partostratind{j} \tmtwo_0\tmtwo_1 = \tmtwo$}
		\DisplayProof
		\end{align*}
		where $j = \min\{m_0, j_1+1\} \geq m_1+1 = m$.
	\end{enumerate}
	
	\item \emph{$\beta$-step}:
	\begin{align*}
	\AxiomC{$\tm_0 \partobind{n_0} \tm_0'$}
	\AxiomC{$\tm_1 \partobind{n_1} \tm_1'$}
	\BinaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \partobind{n} \tm_0' \isub{\var}{\tm_1'} = \tmtwo$}
	\DisplayProof
	\end{align*}
	where $n = n_0 + \sizep{\tm_0}{\var}n_1 + 1 > 0$.
	By \ih, $\tm_0 \partostratind{m_0} \tmtwo_0$ and $\tm_1 \partostratind{m_1} \tmtwo_1$ for some $m_0, m_1 \in \nat$.
	Thus,
	\begin{align*}
	\AxiomC{$\tm_0 \partostratind{m_0} \tm_0'$}
	\AxiomC{$\tm_1 \partostratind{m_1} \tm_1'$}
	\BinaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \partostratind{0} \tm_0' \isub{\var}{\tm_1'} = \tmtwo$}
	\DisplayProof
	\,.
	\end{align*}	
	Let $\tmthree = \tm_0\isub{\var}{\tm_1}$.
	By \reflemma{partobind-subs}, $\tmthree = \tm_0\isub{\var}{\tm_1} \partobindlong{n_0 + \sizep{\tm_0}{\var} n_1} \tm_0'\isub{\var}{\tm_1'} = \tmtwo$ where $n_0 + \sizep{\tm_0}{\var} n_1 = n - 1$.
	Clearly,
	\begin{align*}
	\AxiomC{}
	\UnaryInfC{$\tm = (\la{\var}\tm_0)\tm_1 \tostratind{0} \tm_0 \isub{\var}{\tm_1} = \tmthree$}
	\DisplayProof
	\,.
	\end{align*}
	By \ih (since $n_0 + \sizep{\tm_0}{\var} n_1 = n -1$), $\tmthree = \tm_0\isub{\var}{\tm_1} \partostratind{j} \tm_0'\isub{\var}{\tm_1'} = \tmtwo$ for some $j \in \nat \cup \{\infty\}$, in particular $j \geq 0$.
	\qedhere
\end{itemize}
\end{proof}

%\setcounter{propositionAppendix}{\value{prop:quant-out-in-split-strat}}
\begin{propositionAppendix}[Stratified indexed split]
	\label{propappendix:quant-out-in-split-strat}
	\NoteState{prop:quant-out-in-split-strat}
	If $\tm \partobind n \tmtwo$ then either $\tm \partonotstrat\tmtwo$ or $n>0$ and there exists $\tmthree$ such that $\tm \tostrat \tmthree \partobindlong {n-1} \tmtwo$.
\end{propositionAppendix}

\begin{proof}
	If $n = 0$, then $\tm = \tmtwo$ (because $\partobind{0}$ is the identity relation) and so $\tm \partostratind{\infty} \tmtwo$ (because $\partostratind{\infty}$ is the identity relation), hence $\tm \partonotstrat \tmtwo$. %It requires that $\partonotstrat$ contains the infinite index and that $\partobind{0}$ is the identity relation (not only reflexive).
	
	Otherwise $n > 0$ and then, by \reflemma{decomp-strat}, $\tm \partostratind{k} \tmtwo$ and $\tm \tostratind{k} \tmthree$ for some $k \in \nat$ and some term $\tmthree$ such that $\tmthree \partobind{n-1} \tmtwo$.
	There are two cases:
	\begin{enumerate}
		\item either $k > \Deg{\tm}$ and then $\tm \partonotstrat \tmtwo$ (since $\tm \partostratind{k} \tmtwo$);
		\item or $k = \Deg{\tm}$  and so $\tm \tostrat \tmthree \partobindlong{n-1} \tmtwo$.
		\qedhere
	\end{enumerate}
\end{proof}

%\setcounter{corollaryAppendix}{\value{coro:e-i-split-strat}}
\begin{corollaryAppendix}[Stratified split]
	\label{coroappendix:e-i-split-strat}
	\NoteState{coro:e-i-split-strat}
	If $\tm \partob \tmtwo$ then $\tm \tostrat^* \tmthree \partonotstrat \tmtwo$ for some $\tmthree$.
\end{corollaryAppendix}

%\begin{proof}
%	By hypothesis, $\tm \partobind{n} \tmtwo$ for some $n \in \nat$.
%	We prove the statement by induction on $n \in \nat$.
%	
%	According to the indexed splitting (\refprop{quant-out-in-split-strat}), there are two cases:
%	\begin{itemize}
%		\item either $\tm \partonotstrat \tmtwo$ and we can then conclude taking $\tmthree = \tm$ (in particular, this is the case for $n = 0$, because $\partobind{0}$ is the identity relation);
%		\item or $n > 0$  and $\tm \tostrat \tmfour \partobind{n-1} \tmtwo$; 
%		by \ih applied to $\tmfour \partobind{n-1} \tmtwo$, there is a term $\tmthree$ such that $\tmfour \tostrat^* \tmthree \partonotstrat \tmtwo$;
%		therefore, $\tm \tostrat \tmfour \tostrat^* \tmthree \partonotstrat \tmtwo$.
%		\qedhere
%	\end{itemize}
%\end{proof}
\begin{proof}
	By hypothesis, $\tm \partobind{n} \tmtwo$ for some $n \in \nat$.
	We prove the statement by induction on $n \in \nat$.
	
	If $n = 0$, then $\tm = \tmtwo$ (because $\partobind{0}$ is the identity relation) and so $\tm \partostratind{\infty} \tmtwo$ (because $\partostratind{\infty}$ is the identity relation), hence $\tm \partonotstrat \tmtwo$.
	
	Otherwise $n > 0$ and then, by \reflemma{decomp-strat}, $\tm \partostratind{k} \tmtwo$ and $\tm \tostratind{k} \tmthree$ for some $k \in \nat$ and some term $\tmthree$ such that $\tmthree \partobind{n-1} \tmtwo$.
	There are two cases:
	\begin{enumerate}
		\item either $k > \Deg{\tm}$ and then $\tm \partonotstrat \tmtwo$ (as $\tm \partostratind{k} \tmtwo$), so we conclude taking $\tmthree = \tm$;
		\item or $k = \Deg{\tm}$  and then $\tm \tostrat \tmfour \partobindlong{n-1} \tmtwo$;
		by \ih applied to $\tmfour \partobind{n-1} \tmtwo$, there is a term $\tmthree$ such that $\tmfour \tostrat^* \tmthree \partonotstrat \tmtwo$;
		therefore, $\tm \tostrat \tmfour \tostrat^* \tmthree \partonotstrat \tmtwo$.
		\qedhere
	\end{enumerate}
\end{proof}

Note that the last proof uses only \reflemma{decomp-strat}, not \refprop{quant-out-in-split-strat}!


=========================

\subsection{STRATIFIED: Proposta di prova per Indexed Split e Split}
\newcommand{\tmpp}{\tmfive}
\CF{Scriverei la prova di Indexed Split esattamente come quella per Head. La prova sotto e' cut-and-paste dalla prova di Head;
	ho cambiato solo il caso applicazione.
	Non mi sembra di vedere difficolta' particolari; in un certo senso e' piu' facile, perche' non occorre distinguere se in  $rp$ il termine $r$
	 e' astrazione. \textbf{Ho segnalato in blu il punto chiave}.
	Cosa ne pensate?
 }




%
%\begin{lemma} Assume 	\[\AxiomC{$\tmr \partoat {d_{\tmr}} \tmr'$}
%	\AxiomC{$\tmpp \partoat{d_{\tmpp}} \tmpp'$}
%	\BinaryInfC{$\tm = \tmr \tmpp \partoat d \tmr' \tmpp' = \tmtwo$}
%	\DisplayProof\]
%If $d=\deg  {\tmr \tmpp}$	then either $\deg \tmr = d_{\tmr}$ or $\deg \tmpp = d_{\tmpp}$ .
%\end{lemma}
%\begin{proof} Observe that 
%	  $\deg  {\tmr \tmpp}\leq \deg  {\tmr } $ and $\deg  {\tmr \tmpp}\leq \deg  {\tmpp} $  hold in both cases defining $\deg{\tmr \tmpp}$.
%	  By definition, $d=\min\{ d_{\tmr}, d_{\tmpp}+1  \}$. If  $d=d_{\tmr}$, then $d=\deg  {\tmr \tmpp}\leq \deg \tmr \leq
%	  d_{\tmr}=d $, hence $\deg \tmr = 
%	  d_{\tmr}$.
%	   If  $d=d_{\tmpp}+1$, then $d=\deg  {\tmr \tmpp}\leq \deg \tmpp +1 \leq	  d_{\tmpp}+1 =d $, hence $\deg \tmpp = 
%	  d_{\tmpp}$. 
%\end{proof}

\begin{propositionAppendix}[Indexed split]
	\label{propappendix:quant-out-in-split-strat}
	\NoteState{prop:quant-out-in-split-strat}
	If $\tm \partobind n \tmtwo$ then either $\tm\partonotst \tms$ or $n>0$ and there exists $\tmthree$ such that $\tm \tostrat \tmu \partobindlong {n-1} \tms$.
\end{propositionAppendix}

\proof
By induction on $\tm \partobind n \tmtwo$. We freely use the fact that if $\tm \partobind n \tmtwo$ then $\tm \partob \tmtwo$. Cases:
\begin{itemize}
	\item \emph{Variable}: $\tm = \var \partobind 0 \var = \tmtwo$. Then $\tm = \var \partonotst\var = \tmtwo$.
	
	\item \emph{Abstraction}: $\tm = \la \var\tm' \partobind n  \la \var \tmtwo' = \tmtwo$ because $\tm' \partobind n \tmtwo'$. It follows by the \ih.
	
	\item \emph{Application}:
	\[\AxiomC{$\tmr \partobind {n_1} \tmr'$}
	\AxiomC{$\tmpp \partobind {n_2} \tmpp'$}
	\BinaryInfC{$\tm = \tmr \tmpp \partobindlong {n_1 + n_2} \tmr' \tmpp' = \tmtwo$}
	\DisplayProof\]
	(with $n = n_1 + n_2$). We examine the conclusion.	
	 If $\tmr \tmpp \partonotst \tmr' \tmpp' $ the claim holds.  	 
	 Otherwise, we have $\tmr \tmpp \partoat {d} \tmr' \tmpp'$ with   $d=\deg{\tmr \tmpp}$. Let us write explicitly all the depths:
	
		\[\AxiomC{$\tmr \partoat {d_{\tmr}} \tmr'$}
	\AxiomC{$\tmpp \partoat{d_{\tmpp}} \tmpp'$}
	\BinaryInfC{$\tm = \tmr \tmpp \partoat d \tmr' \tmpp' = \tmtwo$}
	\DisplayProof\]
We first \blue{prove that  if $d=\deg{\tmr \tmpp}$ then  either $\deg \tmr = d_{\tmr}$ or $\deg \tmpp = d_{\tmpp}$}. We then use the \ih\ on the opportune premiss.
\begin{itemize}
	\item Observe that 
	$\deg  {\tmr \tmpp}\leq \deg  {\tmr } $ and $\deg  {\tmr \tmpp}\leq \deg  {\tmpp}+1 $  hold in both cases defining $\deg{\tmr \tmpp}$.
	By definition, $d=\min\{ d_{\tmr}, d_{\tmpp}+1  \}$.
	\begin{enumerate}
		\item[(a.)]  If  $d=d_{\tmr}$, then $d=\deg  {\tmr \tmpp}\leq \deg \tmr \leq
	d_{\tmr}=d $, hence $\deg \tmr = 
	d_{\tmr}$.
\item[(b.)]	If  $d=d_{\tmpp}+1$, then $d=\deg  {\tmr \tmpp}\leq \deg \tmpp +1 \leq	  d_{\tmpp}+1 =d $, hence $\deg \tmpp = 
	d_{\tmpp}$. 	
	\end{enumerate}


	\item If (a.) holds, we apply the \ih\ to $\tmr \partobind {n_1} \tmr'$, and obtain that $n_1>0$ and $\tmr \tost \tmu_1 \partobind {n_1-1} \tmr'$, hence $n>0 $ and  $\tmr\tmpp  \tost \tmu_1\tmpp$ and $\tmu_1 \tmpp\partobind {n_1-1+n_2} \tmr'\tmpp'$.  If (b.) holds, we apply the \ih\ to $\tmpp \partobind {n_2} \tmpp'$.
\end{itemize}
	


	\item \emph{$\beta$ step}:
	\[\AxiomC{$\tmthree \partobind {n_1} \tmthree'$}
	\AxiomC{$\tmfour \partobind {n_2} \tmfour'$}		
	\BinaryInfC{$\tm = (\la\var \tmthree)\tmfour \partobindlong {n_1 + \sizep{\tmthree'}\var \cdot n_2 +1} \tmthree'\isub \var {\tmfour'} = \tmtwo$}
	\DisplayProof\]
	With $n = n_1 + \sizep{\tmthree'}\var \cdot n_2 +1 > 0$. We have $\tm = (\la\var \tmthree)\tmfour \tost \tmthree\isub\var\tmfour$ and by substitutivity of $\partobind n$ (\reflemma{partobind-subs}) $\tmthree\isub\var\tmfour \partobindlong{n_1 + \sizep{\tmthree'}\var \cdot n_2} \tmthree' \isub\var{\tmfour'} = \tmtwo$.
	\qedhere
\end{itemize}

\begin{corollary}[Split]
	If $\tm \partob \tmtwo$ then there exists $\tmthree$ such that $\tm \tost^* \tmthree \partonotst\tmtwo$.
\end{corollary}
\proof
If $\tm \partob \tmtwo$ then $\tm \partobind n \tmtwo$ for some $n$. We prove the statement by induction on $n$. By Indexed Split, there are two cases:
\begin{itemize}
	\item \emph{$\blue{\tmthree} \partonotst\tmtwo$}. This is an instance of the statement (take $\tmthree = \tm$).
	
	\item \emph{$n>0$ and there exists $\tmfour$ such that $\tm \tost \tmfour \partobind {n-1} \tmtwo$}. By \ih, there exists $\tmthree$ such that $\tmfour \tost^* \tmthree \partonotst \tmtwo$, and so $\tm \tost^* \tmthree \partonotst\tmtwo$.\qed
\end{itemize}  

\CF{%Anche qui, mi sembra che si possa usare la stessa prova che nel caso Head. Infatti, 
	la prova sopra e' cut-and-paste di \refcoro{e-i-split}.  Io direi semplicemente: \\
\blue{The proof is identical to that of \refcoro{e-i-split}, where  $\tost$ e $\partonotst$ respectively replace $\toh$ and $\partonoth$.}}

\newpage
\subsection{Domanda sulle altre prove di indexed split }
\CF{Mi domando se anche nelle altre prove di indexed split, non sia piu' semplice (mentalmente) usare per l'applicazione lo schema:
	\begin{enumerate}
		\item if $\tmr \tmpp \Rightarrow_{\neg e} \tmr'\tmpp'$ the claim holds
		\item otherwise, we use the \ih  
	\end{enumerate}
}

\subsubsection{Head: la prova seguente di  Indexed Split basta?}
\CF{E' corretto nell'applicazione sostituire i tre sottocasi con la parte blu seguente?}

\begin{proposition}[Indexed split]
%	\label{prop:quant-out-in-split}
	If $\tm \partobind n \tmtwo$ then $\tm \partonoth\tmtwo$, or $n>0$ and there exists $\tmthree$ such that $\tm \toh \tmthree \partobind {n-1} \tmtwo$.
\end{proposition}

\proof
By induction on $\tm \partobind n \tmtwo$. We use freely the fact that if $\tm \partobind n \tmtwo$ then $\tm \partob \tmtwo$. Cases:
\begin{itemize}
	\item \emph{Variable}: $\tm = \var \partobind 0 \var = \tmtwo$. Then $\tm = \var \partonoth\var = \tmtwo$.
	
	\item \emph{Abstraction}: $\tm = \la \var\tm' \partobind n  \la \var \tmtwo' = \tmtwo$ because $\tm' \partobind n \tmtwo'$. It follows by the \ih.
	
	\item \emph{Application}:
	\[\AxiomC{$\tmfour \partobind {n_1} \tmfour'$}
	\AxiomC{$\tmfive \partobind {n_2} \tmfive'$}
	\BinaryInfC{$\tm = \tmfour \tmfive \partobindlong {n_1 + n_2} \tmfour' \tmfive' = \tmtwo$}
	\DisplayProof\]
	With $n = n_1 + n_2$. \blue{We examine the conclusion.
	\begin{itemize}
		\item 	If $\tmfour \tmfive \partonoth \tmfour' \tmfive'$, the claim is holds.
\item 	Otherwise, observe that the  left premiss is not of the form $\tmfour \partonoth \tmfour'$ (otherwise,  $\tmfour \tmfive \partonoth \tmfour' \tmfive'$ ). By the \ih,
	\emph{$n_1>0$ and there exists $\tmfour''$ such that $\tmfour \toh \tmfour'' \partobind {n_1-1} \tmfour'$}. Then $\tm = \tmfour \tmfive \toh \tmfour'' \tmfive$ and 
	\[\AxiomC{$\tmfour'' \partobindlong {n_1-1} \tmfour'$}			
	\AxiomC{$\tmfive \partobind {n_2} \tmfive'$}	
	\BinaryInfC{$\tmfour'' \tmfive \partobindlong {n_1-1 + n_2} \tmfour' \tmfive' = \tmtwo$}
	\DisplayProof\]
	\end{itemize}
	}
	

	\item \emph{$\beta$ step}:
	\[\AxiomC{$\tmthree \partobind {n_1} \tmthree'$}
	\AxiomC{$\tmfour \partobind {n_2} \tmfour''$}		
	\BinaryInfC{$\tm = (\la\var \tmthree)\tmfour \partobindlong {n_1 + \sizep{\tmthree'}\var \cdot n_2 +1} \tmthree'\isub \var {\tmfour'} = \tmtwo$}
	\DisplayProof\]
	With $n = n_1 + \sizep{\tmthree'}\var \cdot n_2 +1 > 0$. We have $\tm = (\la\var \tmthree)\tmfour \toh \tmthree\isub\var\tmfour$ and by substitutivity of $\partobind n$ (\reflemma{partobind-subs}) $\tmthree\isub\var\tmfour \partobindlong{n_1 + \sizep{\tmthree'}\var \cdot n_2} \tmthree' \isub\var{\tmfour'} = \tmtwo$.
	\qedhere
\end{itemize}

\subsubsection{Leftmost: indexed split}
\CF{Tento di implementare anche  nel caso della leftmost, ma qui vado per puro pattern-matching, perche' LO e' una riduzione che io non capisco}

\begin{proposition}[Indexed split]
	\label{prop:quant-out-in-split-left}
	If $\tm \partobind n \tmtwo$ then $\tm \partonotlo \tmtwo$ or $n>0$ and there exists $\tmthree$ such that $\tm \tolo \tmthree \partobind {n-1} \tmtwo$.
\end{proposition}

\begin{proof}
	By induction on $\tm \partobind n \tmtwo$. We use freely the fact that if $\tm \partobind n \tmtwo$ then $\tm \partob \tmtwo$. Cases:
	\begin{itemize}
		\item \emph{Variable}: $\tm = \var \partobind 0 \var = \tmtwo$. Then $\tm = \var \partonotlo \var = \tmtwo$.
		
		\item \emph{Abstraction}: $\tm = \la \var\tm' \partobind n  \la \var \tmtwo' = \tmtwo$ because $\tm' \partobind n \tmtwo'$. It follows by the \ih.
		
		\item \emph{Application}:
		\[\AxiomC{$\tmfour \partobind {n_1} \tmfour'$}
		\AxiomC{$\tmfive \partobind {n_2} \tmfive'$}
		\BinaryInfC{$\tm = \tmfour \tmfive \partobindlong {n_1 + n_2} \tmfour' \tmfive' = \tmtwo$}
		\DisplayProof\]
		With $n = n_1 + n_2$.\blue{We examine the conclusion.
		\begin{itemize}
			\item  If $\tmfour \tmfive \partonotlo \tmfour' \tmfive'$, the claim holds.
			\item  Otherwise, observe that $\tmfour$ is not neutral (otherwise $\tmfour \tmfive \partonotlo \tmfour' \tmfive'$ by  the 5th rule) and the left premiss is not of the form 
		$\tmfour \partonotlo \tmfour'$ (otherwise $\tmfour \tmfive \partonotlo \tmfour' \tmfive'$ by the 2nd rule). By the \ih, 
		\emph{$n_1>0$ and there exists $\tmfour''$ such that $\tmfour \tolo \tmfour'' \partobind {n_1-1} \tmfour'$}. Then $\tm = \tmfour \tmfive \tolo \tmfour'' \tmfive$ and 
		\[\AxiomC{$\tmfour'' \partobindlong {n_1-1} \tmfour'$}			
		\AxiomC{$\tmfive \partobind {n_2} \tmfive'$}	
		\BinaryInfC{$\tmfour'' \tmfive \partobindlong {n_1-1 + n_2} \tmfour' \tmfive' = \tmtwo$}
		\DisplayProof\]
		\end{itemize}
		}
	
		
		\item \emph{$\beta$ step}:
		\[\AxiomC{$\tmthree \partobind {n_1} \tmthree'$}
		\AxiomC{$\tmfour \partobind {n_2} \tmfour''$}		
		\BinaryInfC{$\tm = (\la\var \tmthree)\tmfour \partobindlong {n_1 + \sizep{\tmtwo}\var \cdot n_2 +1} \tmthree'\isub \var {\tmfour'} = \tmtwo$}
		\DisplayProof\]
		With $n = n_1 + \sizep\tmtwo\var \cdot n_2 +1 > 0$. We have $\tm = (\la\var \tmthree)\tmfour \tolo \tmthree\isub\var\tmfour$ and by substitutivity of $\partobind n$ (\reflemmap{partobind-subs}{ind-par}) $\tmthree\isub\var\tmfour \partobindlong{n_1 + \sizep\tmtwo\var \cdot n_2} \tmthree' \isub\var{\tmfour'} = \tmtwo$.
	\end{itemize}
\end{proof}



%
%
%\subsection{Qualche  idea di  titolo}
%\begin{itemize}
%	\item Factor out the difficulties of normalization
%	
%	\item Factor your way to normalization
%\end{itemize}


==> proofs/proofs-weak-cbvBIS.tex <==
% !TEX root = ../main.tex
\subsection{Omitted proofs  of \refsect{cbv-calculus} (\cbv $\l$-calculus)}
\setcounter{lemmaAppendix}{\value{l:tobv-subs}}
\begin{lemmaAppendix}[Substitutivity of $\partobvind n$]
	\label{lappendix:tobv-subs} % \reflemmap{tob-subs}{ind-par}
	\NoteState{l:tobv-subs}
 If $\tm \partobvind n \tm'$ and $\val \partobvind m \val'$ then $\tm \isub\var\val \partobvindlong {n + \sizep{\tm'}\var\cdot m} \tm' \isub\var{\val'}$.
\end{lemmaAppendix}

\begin{proof}
By induction on $\tm \partobind n \tm'$. It follows the exact same pattern of the proof of substitutivity of $\partobind n$. Cases:
\begin{itemize}
	\item \emph{Variable}: two sub-cases
	\begin{itemize}
	\item $\tm = \var$: then $\tm = \var \partobvind 0 \var = \tm'$ then $\tm \isub\var\val = \var\isub\var\val = \val \partobvind m \val' = \var \isub\var{\val'} = \tm' \isub\var{\val'}$ that satisfies the statement because $n + \sizep{\tm'}\var\cdot m = 0+1\cdot m = m$. 
	 \item $\tm = \vartwo$: then $\tm = \vartwo \partobvind 0 \vartwo = \tm'$ then $\tm \isub\var\val = \vartwo\isub\var\val = \vartwo \partobvind 0 \vartwo = \vartwo \isub\var{\val'} = \tm' \isub\var{\val'}$ that satisfies the statement because $n + \sizep{\tm'}\var\cdot m = n +0\cdot m=n$.
	 \end{itemize}
	
	\item \emph{Abstraction}, \ie $\tm = \la{\vartwo}{\tmthree} \partobvind{n} \la{\vartwo}{\tmthree'} = \tm'$ because $\tmthree \partobvind{n} \tmthree'$; we can suppose without loss of generality that $\vartwo \neq \var$, hence $\sizep{\tmthree'}{\var} = \sizep{\tm'}{\var}$ and $\tm\isub{\var}{\val} = \la{\vartwo}(\tmthree\isub{\var}{\val})$ and $\tm'\isub{\var}{\val'} = \la{\vartwo}(\tmthree'\isub{\var}{\val'})$.
		By \ih, $\tmthree\isub{\var}{\val} \partobvindlong{n +  \sizep{\tmthree'}{\var} \cdot m} \tmthree'\isub{\var}{\val'}$, thus
		\begin{align*}
		\AxiomC{$\tmthree\isub{\var}{\val} \partobvindlong{n +  \sizep{\tmthree'}{\var} \cdot m} \tmthree'\isub{\var}{\val'}$}
		%%\RightLabel{$\parRew{\l}$}
		\UnaryInfC{$\tm\isub{\var}{\val} = \la {\vartwo}\tmthree\isub{\var}{\val} \partobvindlong{n +  \sizep{\tm'}{\var} \cdot m} \la{\vartwo}\tmthree'\isub{\var}{\val'} = \tm'\isub{\var}{\val'}$}
		\DisplayProof\,.
		\end{align*}		
		
	
	\item \emph{Application}, \ie	
	\[\AxiomC{$\tmthree \partobvind {n_\tmthree} \tmthree'$}
	\AxiomC{$\tmfour \partobvind {n_\tmfour} \tmfour'$}
	%\RightLabel{$\parRew{@}$}
	\BinaryInfC{$\tm = \tmthree \tmfour \partobvindlong {n_\tmthree + n_\tmfour} \tmthree' \tmfour'= \tm'$}
	\DisplayProof\]
	with $n = n_\tmthree + n_\tmfour$. By \ih, $\tmthree\isub\var\val \partobvindlong {n_\tmthree +\sizep{\tmthree'}\var \cdot m} \tmthree'\isub\var{\val'}$ and $\tmfour\isub\var\val \partobvindlong {n_\tmfour +\sizep{\tmfour'}\var \cdot m} \tmfour'\isub\var{\val'}$. Then 
	\[\AxiomC{$\tmthree\isub\var\val \partobvindlong {n_\tmthree +\sizep{\tmthree'}\var \cdot m} \tmthree'\isub\var{\val'}$}
	\AxiomC{$\tmfour\isub\var\val \partobvindlong {n_\tmfour +\sizep{\tmfour'}\var \cdot m} \tmfour'\isub\var{\val'}$}
	%\RightLabel{$\parRew{@}$}
	\BinaryInfC{$\tm\isub\var\val = \tmthree\isub\var\val \tmfour\isub\var\val \partobvindlong {n_\tmthree +\sizep{\tmthree'}\var \cdot m +n_\tmfour +\sizep{\tmfour'}\var \cdot m} \tmthree'\isub\var{\val'} \tmfour'\isub\var{\val'}= \tm'\isub\var{\val'}$}
	\DisplayProof\]
that proves the statement because $$n_\tmthree +\sizep{\tmthree'}\var \cdot m +n_\tmfour +\sizep{\tmfour'}\var \cdot m = n + (\sizep{\tmthree'}\var + \sizep{\tmfour'}\var)\cdot m = n + \sizep{\tm'}\var \cdot m$$

\item $\beta$, \ie
	\[\AxiomC{$\tmthree \partobvind {n_\tmthree} \tmthree'$}
	\AxiomC{$\valthree \partobvind {n_{\valthree}} \valfour$}
%\RightLabel{$\parRew{\beta}$}
\BinaryInfC{$\tm = (\la\vartwo \tmthree)\valthree \partobvindlong {n_\tmthree + \sizep{\tmthree'}\vartwo \cdot n_{\valthree} +1} \tmthree'\isub \vartwo {\valfour} = \tm'$}
\DisplayProof\]
with $n = n_\tmthree + \sizep{\tmthree'}\vartwo \cdot n_{\valthree} +1$. We can assume without loss of generality that $\vartwo\neq \var$, 
		hence, $\sizep{\tm'}{\var} = \sizep{\tmthree'\isub\vartwo {\valfour}}\var = \sizep{\tmthree'}{\var} + \sizep{\tmthree'}{\vartwo}\cdot\sizep{\valfour}{\var} $ and $\tm\isub\var\val = (\la\vartwo\tmthree\isub\var\val) (\valthree\isub\var\val)$ and $\tm'\isub\var{\val'} = \tmthree'\isub\var{\val'} \isub\vartwo{\valfour\isub\var{\val'}}$.
		
		By \ih, $\tmthree\isub\var\val \partobvindlong {n_\tmthree +\sizep{\tmthree'}\var \cdot m} \tmthree'\isub\var{\val'}$ and $\valthree\isub\var\val \partobvindlong {n_{\valthree} +\sizep{\valfour}\var \cdot m} \valfour\isub\var{\val'}$. Then 
	\[\AxiomC{$\tmthree\isub\var\val \partobvindlong {n_\tmthree +\sizep{\tmthree'}\var \cdot m} \tmthree'\isub\var{\val'}$}
	\AxiomC{$\valthree\isub\var\val \partobvindlong {n_{\valthree} +\sizep{\valfour}\var \cdot m} \valfour\isub\var{\val'}$}
	%\RightLabel{$\parRew{\beta}$}
	\BinaryInfC{$\tm\isub\var\val = (\la\vartwo\tmthree\isub\var\val) (\valthree\isub\var\val) \partobvindlong {n_\tmthree +\sizep{\tmthree'}\var \cdot m +\sizep{\tmthree'}\vartwo\cdot(n_{\valthree} +\sizep{\valfour}\var \cdot m)+1} \tmthree'\isub\var{\val'} \isub\vartwo{\valfour\isub\var{\val'}}= \tm'\isub\var{\val'}$}
\DisplayProof\]

The number on the $\partobv$ arrow satisfies
$$n_\tmthree +\sizep{\tmthree'}\var \cdot m +\sizep{\tmthree'}\vartwo\cdot(n_{\valthree} +\sizep{\valfour}\var \cdot m)+1 
=
\underbrace{n_\tmthree + \sizep{\tmthree'}\vartwo\cdot n_{\valthree} + 1}_n + \underbrace{\sizep{\tmthree'}\var \cdot m + \sizep{\tmthree'}\vartwo\cdot \sizep{\valfour}\var \cdot m}_{\sizep{\tm'}\var\cdot m}$$
\end{itemize}
\end{proof}


\subsection{Omitted proofs  of \refsect{weak-cbv} (weak \cbv)}

\setcounter{propositionAppendix}{\value{prop:macro-cbv}} 
\begin{propositionAppendix}[Weak \cbv macro-step system]
	\label{propappendix:macro-cbv}
	\NoteState{prop:macro-cbv}
\begin{enumerate}
 \item \label{pappendix:macro-cbv-merge} \emph{Merge}: if $\tm \partonotw\cdot \tow \tmthree$ then $\tm \partobv \tmthree$.
 \item \label{pappendix:macro-cbv-indexed-split} \emph{Indexed split}: if $\tm \partobvind n \tmtwo$ then $\tm \partonotw\tmtwo$, or $n>0$ and $\tm \tow \cdot \partobvind {n-1} \tmtwo$.
 \item \label{pappendix:macro-cbv-split} \emph{Split}: if $\tm \partobv \tmtwo$ then $\tm \tow^* \cdot \partonotw\tmtwo$.
\end{enumerate}
That is, $(\Lambda, \set{\tow, \tonotw})$ is a macro-step system with respect to $\partobv$ and $\partonotw$.
\end{propositionAppendix}


\begin{proof}
\hfill
\begin{enumerate}
 \item \emph{Merge}: by induction on $\tm \partonotw\tmtwo$. Note that the cases in which $\tmtwo=\var$ or $\tmtwo=\l x. \tms'$ are not possible.  Hence $ \tmtwo=\tmfour'\tmfive' $  and $\tm \partonotw\tmtwo$ is derived as follows
	\begin{align*}
	\AxiomC{$\tmfour \partonotw \tmfour'$}
	\AxiomC{$\tmfive \partonotw \tmfive'$}
	\BinaryInfC{$\tm = \tmfour\tmfive \partonotw \tmfour'\tmfive' =\tmtwo$}
	\DisplayProof
	\end{align*}
\begin{enumerate}
\item If $ \tmfour' \tow \tmfour''$ then $\tmtwo = \tmfour'' \tmfive'$. The \ih gives $\tmfour \partobv \tmfour''$, and $\tm \partobv \tmtwo$ is derived as follows (remember that $\partonotw \subseteq \partobv$):
\begin{align*}
	\AxiomC{$\tmfour \partobv \tmfour''$}
	\AxiomC{$\tmfive \partobv \tmfive'$}
	\BinaryInfC{$\tm = \tmfour\tmfive \partobv \tmfour''\tmfive' =\tmtwo$}
	\DisplayProof
	\end{align*}

	\item If $ \tmfive' \tow \tmfive''$ it is analogous to the previous case.

\item If 	$ \tmtwo \tow \tmthree$ by a top $\betav$ step then $\tmfour' = \la x \tmq'$. Now, by definition of $\partonotw$ the step $\tmfour \partonotw \tmfour'$ necessarily has the form $\tmfour = \la x \tmq \partonotw \la x \tmq' = \tmfour'$ for some $\tmq$ such that $\tmq\partobv \tmq'$. Then the hypothesis is $\tm = (\la x \tmq) \tmfive \partonotw (\la x \tmq') \tmfive' \tow \tmq'\isub{\var}{\tmfive'} = \tmthree$ and  $\tm \partobv \tmtwo$ is derived as follows (remember that $\partonotw \subseteq \partobv$):
\begin{align*}
\AxiomC{$\tmq\partob \tmq'$}
\AxiomC{$\tmfive \partob \tmfive'$}
\BinaryInfC{$\tm = (\la x \tmq) \tmfive \partob  \tmq'\isub{\var}{\tmfive'} =\tmtwo $}
\DisplayProof
\end{align*}
\end{enumerate}	


\item \emph{Indexed split}: by induction on the definition of $\tm \partobvind n \tmtwo$. 
	We freely use the fact that if $\tm \partobvind n \tmtwo$ then $\tm \partobv \tmtwo$. Cases:
	\begin{itemize}
		\item \emph{Variable}: $\tm = \var \partobvind 0 \var = \tmtwo$. 
		Then, $\tm = \var \partonotw\var = \tmtwo$.
		
		\item \emph{Abstraction}: $\tm = \la \var\tm' \partobvind n  \la \var \tmtwo' = \tmtwo$ because $\tm' \partobvind n \tmtwo'$. 
		Then, 
		\begin{align*}
		\AxiomC{$\tm' \partobv \tmtwo'$}
		\UnaryInfC{$\tm = \la{\var}\tm' \partonotw \la{\var}\tmtwo' = \tmtwo$}
		\DisplayProof
		\,.
		\end{align*}
		
%		\item \emph{Application}:
%		\[\AxiomC{$\tmfour \partobvind {n} \tmfour'$}
%		\AxiomC{$\tmfive \partobvind {m} \tmfive'$}
%		\BinaryInfC{$\tm = \tmfour \tmfive \partobvindlong {n + m} \tmfour' \tmfive' = \tmtwo$}
%		\DisplayProof\]
%		By \ih applied to $\tmfour \partobvind{n} \tmfour'$ and $\tmfive \partobvind{m} \tmfive'$, there are three sub-cases:
%		\begin{enumerate}
%			\item either $\tmfour \partonotw \tmfour'$ and $\tmfive \partonotw \tmfive'$, and then  
%			\[\AxiomC{$\tmfour \partonotw \tmfour'$}
%			\AxiomC{$\tmfive \partonotw \tmfive'$}
%			\BinaryInfC{$\tm = \tmfour \tmfive \partonotw \tmfour' \tmfive' = \tmtwo$}
%			\DisplayProof
%			\,;\]
%			\item or $n > 0$ and there exists $\tmfour''$ such that $\tmfour \tow \tmfour'' \partobvind {n-1} \tmfour'$;
%			then, $\tm = \tmfour \tmfive \tow \tmfour'' \tmfive \eqdef \tmthree$ and 
%			\[\AxiomC{$\tmfour'' \partobvindlong {n-1} \tmfour'$}			
%			\AxiomC{$\tmfive \partobvind {m} \tmfive'$}	
%			\BinaryInfC{$\tmthree = \tmfour'' \tmfive \partobvindlong {n-1 + m} \tmfour' \tmfive' = \tmtwo$}
%			\DisplayProof 
%			\,;\]
%			\item or $m > 0$ and there exists $\tmfive''$ such that $\tmfive \tow \tmfive'' \partobvind {m-1} \tmfive'$;
%			then, $\tm = \tmfour \tmfive \tow \tmfour \tmfive'' \eqdef \tmthree$ and 
%			\[\AxiomC{$\tmfour \partobvindlong {n} \tmfour'$}			
%			\AxiomC{$\tmfive'' \partobvind {m-1} \tmfive'$}	
%			\BinaryInfC{$\tmthree = \tmfour\tmfive'' \partobvindlong {n + m - 1} \tmfour' \tmfive' = \tmtwo$}
%			\DisplayProof 
%			\,.\]
%		\end{enumerate}
	\item \emph{Application}:
	\[\AxiomC{$\tmfour \partobvind {n_1} \tmfour'$}
	\AxiomC{$\tmfive \partobvind {n_2} \tmfive'$}
	\BinaryInfC{$\tm = \tmfour \tmfive \partobvindlong {n_1 + n_2} \tmfour' \tmfive' = \tmtwo$}
	\DisplayProof\]
	with $n = n_1 + n_2$. There are only two cases:
	\begin{itemize}
		\item either $\tmfour \tmfive \partonotw \tmfour' \tmfive'$, and then the claim holds.
		\item or $\tmfour \tmfive \not\partonotw \tmfour' \tmfive'$, and then $\tmfour \not\partonotw \tmfour'$ or $\tmfive \not\partonotw \tmfive'$ (otherwise $\tmfour \tmfive \partonotw \tmfour' \tmfive'$). 
		Suppose $\tmfour \not\partonotw \tmfour'$ (the other case is analogous). 
		By \ih applied to $\tmfour \partobvind{n_1} \tmfour'$,
		$n_1>0$ and there is $\tmfour''$ such that $\tmfour \tow \tmfour'' \partobvind {n_1-1} \tmfour'$. 
		So, $\tm = \tmfour \tmfive \tow \tmfour'' \tmfive$ and 
		\[\AxiomC{$\tmfour'' \partobvindlong {n_1-1} \tmfour'$}			
		\AxiomC{$\tmfive \partobvind {n_2} \tmfive'$}	
		\BinaryInfC{$\tmfour'' \tmfive \partobvindlong {n_1-1 + n_2} \tmfour' \tmfive' = \tmtwo$}
		\DisplayProof
		\ .
		\]
	\end{itemize}
		
		\item \emph{$\betav$ step}:
		\[\AxiomC{$\tmfive \partobvind {n_1} \tmfive'$}
		\AxiomC{$\tmfour$ is a value}
		\AxiomC{$\tmfour \partobvind {n_2} \tmfour'$}		
		\TrinaryInfC{$\tm = (\la\var \tmfive)\tmfour \partobvindlong {n_1 + \sizep{\tmfive'}\var \cdot n_2 +1} \tmfive'\isub \var {\tmfour'} = \tmtwo$}
		\DisplayProof\]
		with $n = n_1 + \sizep{\tmfive'}\var \cdot n_2 +1 > 0$. 
		We have $\tm = (\la\var \tmfive)\tmfour \tow \tmfive\isub\var\tmfour \eqdef \tmthree$ and substitutivity of $\partobvind n$ (\reflemma{tobv-subs}) gives $\tmthree = \tmfive\isub\var\tmfour \partobvindlong{n_1 + \sizep{\tmfive'}\var \cdot n_2} \tmfive' \isub\var{\tmfour'} = \tmtwo$.		
	\end{itemize}
	
	\item \emph{Split}: exactly as in the head case (\refpropp{macro-head}{split}), using the Indexed Split property for weak \cbv (\refpoint{macro-cbv-indexed-split} above).
	\qedhere
	\end{enumerate}
\end{proof}
\newpage
\setcounter{propositionAppendix}{\value{essential-weak}}
\begin{propositionAppendix}[Weak \cbv essential system]
	\label{propappendix:essential-weak}
	\NoteState{prop:essential-weak}
	\begin{enumerate}
		\item\label{pappendix:essential-weak-persistence} \emph{Persistence}: if $\tm \tow \tmtwo$ and $\tm \tonotw \tmthree$ then $\tmthree \tow \tmfour$ for some $\tmfour$.
		\item\label{pappendix:essential-weak-diamond} \emph{Diamond}: if $\tmtwo\ltow \tm \tow\tmthree$ with $\tmtwo \neq \tmthree$ then $\tmtwo \tow \tmfour \ltow \tmthree$ for some $\tmfour$.
	\end{enumerate}
	Then, $(\Lambda, \set{ \tow, \tonotw})$ is an essential system.
\end{propositionAppendix}
%%\setcounter{lemmaAppendix}{\value{l:persistence-cbv}}
%\begin{lemmaAppendix}[Persistence]
%	\label{lappendix:persistence-cbv}
%%	\NoteState{l:persistence-cbv}
%	If $\tm \tonotw \tmtwo$ and $\tm \tow \tmthree$, then $\tmtwo \tow \tmfour$ for some $\tmfour$. 
%\end{lemmaAppendix}


\blue{\begin{proof}We prove that if $\tm \tonotw \tms$ and $\tms$ is $\tow$-normal, then $\tm$ is $\tow$-normal, by induction on the term $\tms$. Cases. 
	\begin{enumerate}
		\item $\tms=x$ does not apply, because no $\tonotw$-step is possible.
		\item $\tms=\la x \tmr$. We have $\tm=\la x \tmr \tonotw \la x \tmr'=\tms$,
		and $\tmr \tonotw  \tmr'$,  with $\tmr'$ $\tow$-normal.  By the \ih, $\tmr $ is $\tow$-normal, hence  so is $\tm=\la x \tmr$.
	
	\item $\tms= \tmq\tmr$. Then $\tm=\tmq_1\tmr_1$, with either $\tmq_1\tonotw\tmq$ (and $\tmr_1=\tmr$),
	or  $\tmr_1\tonotw\tmr$ (and $\tmq_1=\tmq$). 
	\begin{enumerate}
		\item By the \ih., $\tmq_1$ and $\tmr_1$ are both $\tow$-normal.
		\item  The $\beta$-rule does not apply, because   if $ \tmq_1 $ is  an abstraction and $\tmr_1$ is  a value, then $ \tmq$ is  an abstraction and $\tmr$ is  a value,
		against the assumption that $\tms$ is $\tow$-normal. 
	\end{enumerate}
	Hence, no rule for $\tow$ applies, and   $\tmr=\tmq_1\tmr_1$ is $\tow$-normal

	\end{enumerate}
	
	

\end{proof}}

\begin{proof}\hfill
	\begin{enumerate}
		\item \emph{Persistence}: By induction on the definition of $\tm \tonotw \tmtwo$.
		Cases:
		\begin{itemize}
			\item \emph{Abstraction}: $\tm = \la\var\tmfive \tonotw \la\var\tmfive'$ because $\tmfive \tobv \tmfive'$. This case is impossible because $\tm$ is $\tow$ normal, against the hypothesis that $\tm \tow \tmthree$.
			
			\item \emph{Application left}: $\tm = \tmfive\tmsix \tonotw \tmfive_{\neg\wsym}\tmsix = \tmtwo$ because $\tmfive \tonotw \tmfive_{\neg\wsym}$.
			According to the definition of $\tow $, there are the following sub-cases:
			\begin{enumerate}
				\item $\tm = \tmfive\tmsix \tow \tmfive_\wsym\tmsix = \tmthree$ with $\tmfive \tow \tmfive_\wsym$; 
				by \ih applied to $\tmfive$, we have $\tmfive_{\neg\wsym} \tow \tmfour'$  for some term $\tmfour'$, and so 
				\begin{align*}
				\AxiomC{$\tmfive_{\neg\wsym} \tow \tmfour'$}
				\UnaryInfC{$\tmtwo = \tmfive_{\neg\wsym}\tmsix \tow \tmfour'\tmsix =: \tmfour$}
				\DisplayProof
				\,;
				\end{align*}
				\item $\tm = \tmfive\tmsix \tow \tmfive\tmsix' = \tmthree$ with  $\tmsix \tow \tmsix'$; 
				hence
				\begin{align*}
				\AxiomC{$\tmsix \tow \tmsix'$}
				\UnaryInfC{$\tmtwo = \tmfive_{\neg\wsym}\tmsix \tow \tmfive_{\neg\wsym}\tmsix' =`: \tmfour$}
				\DisplayProof
				\,;
				\end{align*}		
				%			analogous to the previous sub-case.
				
				\item $\tm = (\la{\var}{\tmfive'})\tmsix \tow \tmfive'\isub{\var}{\tmsix} = \tmthree$ where $\tmfive = \la{\var}{\tmfive'}$ and $\tmsix$ is a value. 
				According to the definition of $\tm \tonotw \tmtwo$,
				\begin{align*}
				\AxiomC{$\tmfive \tobv \tmfive_{\neg\wsym}$}
				\UnaryInfC{$\la{\var}\tmfive' \tonotw \la{\var}\tmfive_{\neg\wsym}'$}
				\UnaryInfC{$\tm = (\la{\var}\tmfive')\tmsix \tonotw (\la{\var}{\tmfive_{\neg\wsym}'})\tmsix = \tmtwo$}
				\DisplayProof
				\end{align*}
				where $\tmfive_{\neg\wsym} = \la{\var}{\tmfive_{\neg\wsym}'}$; therefore
				\begin{align*}
				\AxiomC{}
				\UnaryInfC{$\tmtwo = (\la{\var}\tmfive_{\neg\wsym}')\tmsix \tow \tmfive_{\neg\wsym}'\isub{\var}{\tmsix} =: \tmfour$}
				\DisplayProof
				\,.
				\end{align*}
			\end{enumerate}
			
			\item \emph{Application right}: analogous to the previous point.
		\end{itemize}
		
		\item \emph{Diamond}: 
		The idea of the proof is that, when $(\la{\var}\tm)\val \tow \tm\isub{\var}{\val}$, the $\betav$-redexes in $\val$ (which is a value) can be duplicated in $\tm\isub{\var}{\val}$ but they are under an abstraction and $\tow$ does not reduce  under abstractions.
		
		Formally, the proof is by induction on $\tm$.
		Note that $\tm$ is not a value, because values are $\tow$-normal, since $\tow$ does not reduce under abstractions.
		Therefore, $\tm = \tm_0\tm_1$.
		The case where $\tm_0 = \la{\var}{\tm'}$ and $\tm_1$ is a value is impossible, because $\tm_0$ and $\tm_1$ would be $\tow$-normal and so from $\tmtwo \ltow \tm \tow \tmthree$ it would follow $\tmtwo = \tm'\isub{\var}{\tm_1} = \tmthree$, which contradicts the hypothesis. 
		The remaining cases are:
		\begin{itemize}
			\item $\tmtwo = \tm_0\tmtwo_1 \ltow \tm = \tm_0\tm_1 \tow \tmthree_0\tm_1 = \tmthree$ with $\tm_0 \tow \tmthree_0$,  and $\tm_1 \tow  \tmtwo_1$. 
			Then, $\tmtwo \tow \tmthree_0\tmtwo_1 \ltow \tmthree$.
			
			\item $\tmtwo = \tmtwo_0 \tm_1 \ltow \tm = \tm_0\tm_1 \tow \tmthree_0\tm_1 = \tmthree$ with $\tmtwo_0 \ltow \tm_0 \tow \tmthree_0$. 
			By \ih, there is $\tmfour_0$ such that $\tmtwo_0 \tow \tmfour_0 \ltow \tmthree_0$.
			Thus, $\tmtwo \tow \tmfour_0\tm_1 \ltow \tmthree$.
			
			\item $\tmtwo = \tm_0\tmtwo_1  \ltow \tm = \tm_0\tm_1 \tow \tm_0\tmthree_0 = \tmthree$ with $\tmtwo_1 \ltow \tm_1 \tow \tmthree_1$. 
			Analogous to the previous case.
			\qedhere
		\end{itemize}
	\end{enumerate}
\end{proof}


==> proofs/proofs-weak-cbvCF.tex <==
% !TEX root = ../main.tex
\subsection{Omitted proofs  of \refsect{weak-cbv}}
\setcounter{lemmaAppendix}{\value{l:tobv-subs}}
\begin{lemmaAppendix}[Substitutivity of $\partobvind n$]
	\label{lappendix:tobv-subs} % \reflemmap{tob-subs}{ind-par}
	\NoteState{l:tobv-subs}
 If $\tm \partobvind n \tm'$ and $\tmtwo \partobvind m \tmtwo'$ where $\tmtwo$ is a value,  then $\tm \isub\var\tmtwo \partobvindlong {n + \sizep{\tm'}\var\cdot m} \tm' \isub\var{\tmtwo'}$.
\end{lemmaAppendix}
%\setcounter{lemmaAppendix}{\value{l:tobv-subs}}
%\begin{lemmaAppendix}[Basic properties of $\tobv$ and $\partobvind n$]
%	\label{lappendix:tobv-subs} % \reflemmap{tob-subs}{ind-par}
%	\NoteState{l:tobv-subs}
%	\hfill
%	\begin{enumerate}  
%		%    \item \label{p:tobv-subs-one} 
%		%    \emph{Left substitutivity of $\tobv$}:
%		%    if $\tm \tobv \tm'$ then $\tm\isub\var\tmtwo \tobv \tm'\isub\var\tmtwo$.
%		%    \item \label{p:tobv-subs-two}
%		%    \emph{Right substitutivity of $\tobv$}:
%		%    if $\tmtwo \tobv \tmtwo'$ then $\tm\isub\var\tmtwo \tobv^* \tm\isub\var{\tmtwo'}$.
%		%  
%		\item \label{pappendix:tobv-subs-refl}
%		\emph{Reflexivity of $\partobvind n$}: $\tm \partobvind 0 \tmtwo$ if and only if $\tm = \tmtwo$.
%		\item \label{pappendix:tobv-subs-ind-par}
%		\emph{Substitutivity of $\partobvind n$}: if $\tm \partobvind n \tm'$ and $\tmtwo \partobvind m \tmtwo'$ where $\tmtwo$ is a value,  then $\tm \isub\var\tmtwo \partobvindlong {n + \sizep{\tm'}\var\cdot m} \tm' \isub\var{\tmtwo'}$.
%		\item \label{pappendix:tobv-subs-sing-par}
%		\emph{Single-parallel $\beta$}: $\tobv \,=\, \partobvind 1$ and $\partobvind n \,\subsetneq\, \tobv^n$.
%	\end{enumerate}
%\end{lemmaAppendix}

\begin{proof}
%	\begin{enumerate}
	%	\item Trivial.
		
	%	\item 
		By induction on the definition of $\tm \partobvind{n} \tm'$. Cases:
	\begin{itemize}
		\item \emph{Variable}, \ie $\tm = \var \partobvind{0} \var = \tm'$. Then, $\sizep{\tm'}\var = 1$ and $\tm\isub{\var}{\tmtwo} = \tmtwo \partobvind{m} \tmtwo' = \tm'\isub{\var}{\tmtwo'}$, where $m = 0 + \sizep{\tm'}{\var} \cdot m$.
		\item \emph{Abstraction}, \ie $\tm = \la{\vartwo}{\tmthree} \partobvind{n} \la{\vartwo}{\tmthree'} = \tm'$ because $\tmthree \partobvind{n} \tmthree'$; we can suppose without loss of generality that $\vartwo \notin \fv{\tmtwo} \cup \{\var\} \supseteq \fv{\tmtwo'} \cup \{\var\}$, hence $\sizep{\tmthree'}{\var} = \sizep{\tm'}{\var}$ and $\tm\isub{\var}{\tmtwo} = \la{\vartwo}(\tmthree\isub{\var}{\tmtwo})$ and $\tm'\isub{\var}{\tmtwo'} = \la{\vartwo}(\tmthree'\isub{\var}{\tmtwo'})$.
		By \ih, $\tmthree\isub{\var}{\tmtwo} \partobvindlong{n +  \sizep{\tmthree'}{\var} \cdot m} \tmthree'\isub{\var}{\tmtwo'}$, thus
		\begin{align*}
		\AxiomC{$\tmthree\isub{\var}{\tmtwo} \partobvindlong{n +  \sizep{\tmthree'}{\var} \cdot m} \tmthree'\isub{\var}{\tmtwo'}$}
		%%\RightLabel{$\parRew{\l}$}
		\UnaryInfC{$\tm\isub{\var}{\tmtwo} = \la {\vartwo}\tmthree\isub{\var}{\tmtwo} \partobvindlong{n +  \sizep{\tm'}{\var} \cdot m} \la{\vartwo}\tmthree'\isub{\var}{\tmtwo'} = \tm'\isub{\var}{\tmtwo'}$}
		\DisplayProof\,.
		\end{align*}		
		\item \emph{Application}, \ie $\tm = {\tmthree}\tmfour \partobvind{n_1 + n_2} {\tmthree'}\tmfour' = \tm'$ because $\tmthree \partobvind{n_1} \tmthree'$ and $\tmfour \partobvind{n_2} \tmfour'$.
		By \ih, $\tmthree\isub{\var}{\tmtwo} \partobvindlong{n_1 +  \sizep{\tmthree'}{\var} \cdot m} \tmthree'\isub{\var}{\tmtwo'}$ and $\tmfour\isub{\var}{\tmtwo} \partobvindlong{n_2 +  \sizep{\tmfour'}{\var} \cdot m} \tmfour'\isub{\var}{\tmtwo'}$, hence
		\begin{align*}
		\AxiomC{$\tmthree\isub{\var}{\tmtwo} \partobvindlong{n_1 +  \sizep{\tmthree'}{\var} \cdot m} \tmthree'\isub{\var}{\tmtwo'}$}
		\AxiomC{$\tmfour\isub{\var}{\tmtwo} \partobvindlong{n_2 +  \sizep{\tmfour'}{\var} \cdot m} \tmfour'\isub{\var}{\tmtwo'}$}
		%%\RightLabel{$\parRew{\l}$}
		\BinaryInfC{$\tm\isub{\var}{\tmtwo} = \tmthree\isub{\var}{\tmtwo} \tmfour\isub{\var}{\tmtwo} \partobvindlong{n +  \sizep{\tm'}{\var} \cdot m} \tmthree'\isub{\var}{\tmtwo'} \tmfour'\isub{\var}{\tmtwo'} = \tm'\isub{\var}{\tmtwo'}$}
		\DisplayProof
		\end{align*}
		where $\sizep{\tm'}{\var} = \sizep{\tmthree'}{\var} + \sizep{\tmfour'}{\var}$ and $n = n_1 + n_2$.
		
		\item \emph{$\betav$ step}:
		\[\AxiomC{$\tmthree \partobvind {n_1} \tmthree'$}
		\AxiomC{$\tmfour$ is a value}
		\AxiomC{$\tmfour \partobvind {n_2} \tmfour'$}		
		\TrinaryInfC{$\tm = (\la\vartwo \tmthree)\tmfour \partobvind{n} \tmthree'\isub \vartwo {\tmfour'} = \tm'$}
		\DisplayProof\]
		where $n = n_1 + \sizep{\tmthree'}{\var} \cdot n_2 +1$.
		We can assume without loss of generality that $\vartwo \notin \fv{\tmtwo} \cup \{\var\} \supseteq \fv{\tmtwo'} \cup \{\var\}$;
		hence, $\sizep{\tm'}{\var} = \sizep{\tmthree'}{\var} + \sizep{\tmthree'}{\vartwo}\sizep{\tmfour'}{\var} $ and $\tm\isub{\var}{\tmfour} = (\la{\vartwo}{\tmthree}\isub{\var}{\tmtwo})\tmfour\isub{\var}{\tmtwo}$ and $\tm'\isub{\var}{\tmfour'} = {\tmthree'}\isub{\vartwo}{\tmfour'}\isub{\var}{\tmtwo'} = \tmthree'\isub{\vartwo}{\tmtwo'}\isub{\var}{\tmfour'\isub{\vartwo}{\tmtwo'}}$.
		By \ih, $\tmthree\isub{\var}{\tmtwo} \partobvindlong{n_1 + m \cdot \sizep{\tmthree'}{\var}} \tmthree'\isub{\var}{\tmtwo'}$ and $\tmfour\isub{\var}{\tmtwo} \allowbreak\partobvindlong{n_2 + m \cdot \sizep{\tmfour'}{\var}} \tmfour'\isub{\var}{\tmtwo'}$.
		Therefore, since $\tmfour\isub{\var}{\tmtwo}$ is a value,
		\[\AxiomC{$\tmthree\isub{\var}{\tmtwo} \partobvindlong{n_1 + m \cdot \sizep{\tmthree'}{\var}} \tmthree'\isub{\var}{\tmtwo'}$}
		\AxiomC{$\tmfour\isub{\var}{\tmfour} \partobvindlong{n_2 + m \cdot \sizep{\tmfour'}{\var}} \tmfour'\isub{\var}{\tmtwo'}$}		
		\BinaryInfC{$\tm \isub{\var}{\tmtwo} = (\la\vartwo \tmthree\isub{\var}{\tmtwo})\tmfour\isub{\var}{\tmtwo} \partobvindlong{n_1 + m \cdot \sizep{\tmthree'}{\var} + (n_2 + m \cdot \sizep{\tmfour'}{\var})\sizep{\tmthree'}{\vartwo} + 1} \tmthree'\isub \vartwo {\tmfour'}\isub{\var}{\tmtwo'} = \tm'\isub{\var}{\tmtwo'}$}
		\DisplayProof\]
		where $n_1 + m \cdot \sizep{\tmthree'}{\var} + (n_2 + m \cdot \sizep{\tmfour'}{\var})\sizep{\tmthree'}{\vartwo} + 1 = n + m(\sizep{\tmthree'}{\var} + \sizep{\tmthree'}{\vartwo}\cdot \sizep{\tmfour'}{\var}) = n + m \cdot \sizep{\tm'}{\var}$.
	\end{itemize}

%	\item Trivial.
%	\qedhere
%	\end{enumerate}
\end{proof}

\setcounter{propositionAppendix}{\value{prop:i-e-merge-cbv}}
\begin{propositionAppendix}[Merge]
\label{propappendix:i-e-merge-cbv}
\NoteState{prop:i-e-merge-cbv}
	If $\tm \partonotw\tmtwo \tow \tmthree$ then $\tm \partobv \tmthree$.
\end{propositionAppendix}

\begin{proof}
	By induction on the form of  $ \tmtwo $. 
	Cases $\tmtwo=\var$ or $\tmtwo=\l x. \tms'$ are not possible.  Hence $ \tmtwo=\tmfour'\tmfive' $  and $\tm \partonotw\tmtwo$ is derived as follows
	\begin{align*}
	\AxiomC{$\tmfour \partonotw \tmfour'$}
	\AxiomC{$\tmfive \partonotw \tmfive'$}
	\BinaryInfC{$\tm = \tmfour\tmfive \partonotw \tmfour'\tmfive' $}
	\DisplayProof
	\end{align*}
\begin{enumerate}
	\item If 	$ \tmtwo \tow \tmthree$ by a $\betav$-rule (let $r=\la \var \tmq'$, $\tmfive$ value) then $\tmtwo= (\la x \tmq') \tmfive' \tow \tmq'\isub{\var}{\tmfive'} $ and  we conclude by the following derivation 
\begin{align*}
\AxiomC{$\tmq\partob \tmq'$}
\AxiomC{$\tmfive \partob \tmfive'$}
\BinaryInfC{$  (\la x \tmq) \tmfive \partob  \tmq'\isub{\var}{\tmfive'}  $}
\DisplayProof
\end{align*}

\item Otherwise, either $ \tmfour' \tow \tmfour''$ or $\tmfive' \tow \tmfive''$, and  we apply the \ih\ to the concerned premiss, concluding by application rule.
\end{enumerate}	
%	Cases:
%	\begin{itemize}
%		\item \emph{Variable}: $\tm = \var \partonotw \var = \tmtwo$. 
%		Then, there is no $\tmthree$ such that $\tmtwo \tow \tmthree$.
%		
%		\item \emph{Abstraction}: $\tm = \la \var\tm' \partonotw  \la \var \tmtwo' = \tmtwo$ because $\tm' \partobv \tmtwo'$. 
%		Then, there is no $\tmthree$ such that $\tmtwo \tow \tmthree$.
%		\item \emph{Application}:
%		\begin{align*}
%		\AxiomC{$\tmfour \partonotw \tmfour'$}
%		\AxiomC{$\tmfive \partonotw \tmfive'$}
%		\BinaryInfC{$\tm = \tmfour\tmfive \partonotw \tmfour'\tmfive' = \tmtwo$}
%		\DisplayProof
%		\end{align*}
%		Sub-cases:
%		\begin{enumerate}
%			\item $\tmtwo = \tmfour'\tmfive' \tow \tmfour''\tmfive' = \tmthree$ with $\tmfour' \tow \tmfour''$; 
%			by \ih applied to $\tmfour \partonotw \tmfour' \tow \tmfour''$, we have $\tmfour \partobv \tmfour''$, and so (as $\tmfive \partonotw \tmfive'$ implies $\tmfive \partobv \tmfive'$ by \reflemmap{prop-partobvint}{partobv})
%			\begin{align*}
%			\AxiomC{$\tmfour \partobv \tmfour''$}
%			\AxiomC{$\tmfive \partobv \tmfive'$}
%			\BinaryInfC{$\tm = \tmfour\tmfive \partobv \tmfour''\tmfive' = \tmthree$}
%			\DisplayProof\,;
%			\end{align*}
%			\item $\tmtwo = \tmfour'\tmfive' \tow \tmfour'\tmfive'' = \tmthree$ with $\tmfive' \tow \tmfive''$; 
%			analogous to the previous sub-case.
%			%			by \ih applied to $\tmfive \partonotw \tmfive' \tow \tmfive''$, we have $\tmfive \partobv \tmfive''$, and so (as $\tmfour \partonotw \tmfour'$ implies $\tmfour \partobv \tmfour'$ by \reflemmap{prop-partobvint}{partobv})
%			%			\begin{align*}
%			%			\AxiomC{$\tmfour \partobv \tmfour''$}
%			%			\AxiomC{$\tmfive \partobv \tmfive'$}
%			%			\BinaryInfC{$\tm = \tmfour\tmfive \partobv \tmfour''\tmfive' = \tmthree$}
%			%			\DisplayProof\,.
%			%			\text{\qedhere}
%			%			\end{align*}
%			\qedhere
%		\end{enumerate}
%	\end{itemize}
\end{proof}

\setcounter{propositionAppendix}{\value{prop:quant-out-in-split-cbv}}
\begin{propositionAppendix}[Indexed split]
	\label{propappendix:quant-out-in-split-cbv}
	\NoteState{propappendix:quant-out-in-split-cbv}
	If $\tm \partobvind n \tmtwo$ then either $\tm \partonotw\tmtwo$ or $n>0$ and there exists $\tmthree$ such that $\tm \tow \tmthree \partobvind {n-1} \tmtwo$.
\end{propositionAppendix}

\begin{proof}
	By induction on the definition of $\tm \partobvind n \tmtwo$. 
	We use freely the fact that if $\tm \partobvind n \tmtwo$ then $\tm \partobv \tmtwo$. Cases:
	\begin{itemize}
		\item \emph{Variable}: $\tm = \var \partobvind 0 \var = \tmtwo$. Then $\tm = \var \partonotw\var = \tmtwo$.
		
		\item \emph{Abstraction}: $\tm = \la \var\tm' \partobvind n  \la \var \tmtwo' = \tmtwo$ because $\tm' \partobvind n \tmtwo'$. 
		Then, 
		\begin{align*}
		\AxiomC{$\tm' \partobv \tmtwo'$}
		\UnaryInfC{$\tm = \la{\var}\tm' \partonotw \la{\var}\tmtwo' = \tmtwo$}
		\DisplayProof
		\end{align*}
		
		\item \emph{Application}:
		\[\AxiomC{$\tmfour \partobvind {n} \tmfour'$}
		\AxiomC{$\tmfive \partobvind {m} \tmfive'$}
		\BinaryInfC{$\tm = \tmfour \tmfive \partobvindlong {n + m} \tmfour' \tmfive' = \tmtwo$}
		\DisplayProof\]
		By \ih applied to $\tmfour \partobvind{n} \tmfour'$ and $\tmfive \partobvind{m} \tmfive'$, there are three sub-cases:
		\begin{enumerate}
			\item either $\tmfour \partonotw \tmfour'$ and $\tmfive \partonotw \tmfive'$, and then  
			\[\AxiomC{$\tmfour \partonotw \tmfour'$}
			\AxiomC{$\tmfive \partonotw \tmfive'$}
			\BinaryInfC{$\tm = \tmfour \tmfive \partonotw \tmfour' \tmfive' = \tmtwo$}
			\DisplayProof\,;\]
			\item or $n > 0$ and there exists $\tmfour''$ such that $\tmfour \tow \tmfour'' \partobvind {n-1} \tmfour'$;
			then, $\tm = \tmfour \tmfive \tow \tmfour'' \tmfive \eqdef \tmthree$ and 
			\[\AxiomC{$\tmfour'' \partobvindlong {n-1} \tmfour'$}			
			\AxiomC{$\tmfive \partobvind {m} \tmfive'$}	
			\BinaryInfC{$\tmthree = \tmfour'' \tmfive \partobvindlong {n-1 + m} \tmfour' \tmfive' = \tmtwo$}
			\DisplayProof \,;\]
			\item or $m > 0$ and there exists $\tmfive''$ such that $\tmfive \tow \tmfive'' \partobvind {m-1} \tmfive'$;
			then, $\tm = \tmfour \tmfive \tow \tmfour \tmfive'' \eqdef \tmthree$ and 
			\[\AxiomC{$\tmfour \partobvindlong {n} \tmfour'$}			
			\AxiomC{$\tmfive'' \partobvind {m-1} \tmfive'$}	
			\BinaryInfC{$\tmthree = \tmfour\tmfive'' \partobvindlong {n + m - 1} \tmfour' \tmfive' = \tmtwo$}
			\DisplayProof \,.\]
		\end{enumerate}
		
		\item \emph{$\betav$ step}:
		\[\AxiomC{$\tmfive \partobvind {n_1} \tmfive'$}
		\AxiomC{$\tmfour$ is a value}
		\AxiomC{$\tmfour \partobvind {n_2} \tmfour'$}		
		\TrinaryInfC{$\tm = (\la\var \tmfive)\tmfour \partobvindlong {n_1 + \sizep{\tmfive'}\var \cdot n_2 +1} \tmfive'\isub \var {\tmfour'} = \tmtwo$}
		\DisplayProof\]
		with $n = n_1 + \sizep{\tmfive'}\var \cdot n_2 +1 > 0$. We have $\tm = (\la\var \tmfive)\tmfour \tow \tmfive\isub\var\tmfour \eqdef \tmthree$ and by \reflemmap{tobv-subs}{ind-par} $\tmthree = \tmfive\isub\var\tmfour \partobvindlong{n_1 + \sizep{\tmfive'}\var \cdot n_2} \tmfive' \isub\var{\tmfour'} = \tmtwo$.
		\qedhere
	\end{itemize}
\end{proof}

\blue{\paragraph{On the definition of Internal Parallel Step.}
	A parallel steps  is internal, written 
	$M\partonotw N$,  if 
	$M\parto N$ and $M\tonotw^* N$ (obviously,  $\partonotw \,\subseteq\, \parto$).  We give explicitly the inference rules. We prove that the inference rules characterize the definition of parallel internal step.
	
	
	
	
\begin{lemma}\label{l:basicpar}If $\tm \partobv \tms$ then $\tm \to^* \tms$. Moreover, if $\partobv$ is obtained via the $\parallel\betav$-rule, then $\tm \tobv^*\tm'\tobv \tms$ where  the last step is a $\betav$-rule.
\end{lemma}
\begin{proof}
	Induction on the derivation of $\tm \parto \tms$
\end{proof}

\begin{lemma} The following are equivalent:
	\begin{enumerate}
		\item $\tm \partobv \tms$ and $\tm \tonotw^*\tms$
		\item $\tm \partonotw\tms$
	\end{enumerate}
\end{lemma}


\begin{proof}
\begin{itemize}
	\item $1\rightarrow 2$ by induction on $\tm$. We observe that if $\tm=\tmr\tms$,  $\tm \partobv \tms$ can only be conclusion of a
	$\parallel$App-rule, and not of a $\parallel$$\betav$-rule, because $\tm \tonotw^*\tms$ and \reflemma{basicpar}.
	\item $2\rightarrow 1$ is immediate 
\end{itemize}
\end{proof}}

==> proofs/proofs.tex <==
% !TEX root = ../main.tex
\section{Technical appendix: omitted proofs and lemmas}
\label{sect:proofs}

The enumeration of propositions, theorems, lemmas already stated in the body of the article is unchanged.

%\input{\proofspath/proofs-abstract-rew}

\input{\proofspath/proofs-head}

\input{\proofspath/proofs-weak-cbv}

\input{\proofspath/proofs-leftmost}

\input{\proofspath/proofs-stratified-cbn2}


